Exploration in Structured Reinforcement Learning

We address reinforcement learning problems with finite state and action spaces where the underlying MDP has some known structure that could be potentially exploited to minimize the exploration rates of suboptimal (state, action) pairs. For any arbitrary structure, we derive problem-specific regret lower bounds satisfied by any learning algorithm. These lower bounds are made explicit for unstructured MDPs and for those whose transition probabilities and average reward functions are Lipschitz continuous w.r.t. the state and action. For Lipschitz MDPs, the bounds are shown not to scale with the sizes $S$ and $A$ of the state and action spaces, i.e., they are smaller than $c\log T$ where $T$ is the time horizon and the constant $c$ only depends on the Lipschitz structure, the span of the bias function, and the minimal action sub-optimality gap. This contrasts with unstructured MDPs where the regret lower bound typically scales as $SA\log T$. We devise DEL (Directed Exploration Learning), an algorithm that matches our regret lower bounds. We further simplify the algorithm for Lipschitz MDPs, and show that the simplified version is still able to efficiently exploit the structure.

==> discussion.tex <==
% !TEX root =  main.tex

\section{Discussion}

Sample complexity.

Discounted.

Communicating MDP.



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "./main"
%%% End: 


==> general.tex <==
% !TEX root =  main.tex

\section{The Fundamental Limit}

minimization problem for general structure.



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "./main"
%%% End: 


==> model_old.tex <==
% !TEX root =  main.tex

%\section{Reinforce}  \label{sec:model}
\section{Models and Objectives}

We consider an MDP $\phi=(p_\phi,q_\phi)$ with finite state and action spaces $\set{S}$ and $\set{A}$ of respective cardinalities $S$ and $A$. $p_\phi$ and $q_\phi$ are the transition and reward kernels of $\phi$. Specifically, when in state $x$, under action $a$, the system moves to state $y$ with probability $p_\phi(y|x,a)$, and a reward drawn from distribution $q_\phi(\cdot | x,a)$ of average $r_\phi(x,a)$ is collected. The rewards are bounded, w.l.o.g., in $[0,1]$. We assume that for any $(x,a)$, $q_\phi(\cdot |x,a)$ is absolutely continuous w.r.t. some measure $\lambda$ on $[0,1]$\footnote{$\lambda$ can be the Lebesgue measure; alternatively, if rewards take values in $\{0,1 \}$, $\lambda$ can be the sum of Dirac measures at 0 and 1.}. 
%We denote by $\set{P}(\set{S})$ and $\set{P}([0,1])$ the set of distributions on $\set{S}$ (resp. on $[0,1]$, absolutely continuous w.r.t. $\lambda$).

The random vector $Z_t:=(X_t, A_t, R_t)$ represents the state, the action, and the collected reward at step $t$. In each step $t$,  a policy $\pi$ selects an action, denoted by $\pi_t(x)$ when the system is in state $x$,  based on the history captured through $\set{H}_t^\pi$, the $\sigma$-algebra generated by $(Z_1,\ldots, Z_{t-1},X_t)$ observed under $\pi$: $\pi_t(x)$ is $\set{H}_t^\pi$-measurable. We denote by $\Pi$ the set of all such policies. 

{\bf Structured MDPs.} The MDP $\phi$ is initially unknown. However we assume that $\phi$ belongs to some well specified set $\Phi$. For any (state, action) pair $(x,a)$, $\Phi$ defines the set $\set{S}^+(x,a)$ of reachable states from $(x,a)$: $y\in \set{S}^+(x,a)$ if for any $\phi\in \Phi$, $p_\phi(y|x,a)>0$. The sets $\set{S}^+(x,a)$ are defined so that any $\phi\in \Phi$ is {\it ergodic}\footnote{$\phi$ is ergodic if under any stationary policy $f:\set{S}\to \set{A}$ (the action selected in state $x$ is $f(x)$), the resulting Markov chain $(X_t)_{t\ge 1}$ is irreducible.}. $\Phi$ may further encode a known structure of the MDP. The knowledge of $\Phi$ can be exploited to devise (more) efficient policies. The results derived in this paper are valid under {\it any} structure, but we give a particular attention to the cases of \\
(i) {\it Unstructured MPDs} where $\phi\in \Phi$ if for all $(x,a)$, $p_\phi(\cdot |x,a)\in \set{P}(\set{S}^+(x,a)), q_\phi(\cdot |x,a)\in  \set{P}([0,1])$\footnote{For any finite set $\set{U}$, $\set{P}(\set{U})$ is the set of distributions on $\set{U}$ and $\set{P}([0,1])$ is the set of distributions on $[0,1]$, absolutely continuous w.r.t. $\lambda$.};\\
(ii) {\it Lipschitz MDPs} where $\phi\in \Phi$ if $p_\phi(\cdot |x,a)\in \set{P}(\set{S}^+(x,a))$ and $r_\phi(x,a)$ are Lipschitz-continuous w.r.t. $x$ and $a$ (we provide a precise definition in the next section). 


{\bf The learning problem.} The expected cumulative reward up to step $T$ of a policy $\pi\in \Pi$ when the system starts in state $x$ is $V_T^\pi(x) := \EXP_x^\pi[\sum_{t=1}^T R_t],$ where $\EXP_x^\pi [\cdot ]$ denotes the expectation under policy $\pi$ given that $X_1=x$. Now assume that the system starts in state $x$ and evolves according to the initially unknown MDP $\phi\in \Phi$ for given structure $\Phi$, the objective is to devise a policy $\pi\in \Pi$ maximizing  $V_T^\pi(x)$ or equivalently, minimizing the regret $R_T^\pi(x)$ up to step $T$ defined as the difference between the cumulative reward of an optimal policy and that obtained under $\pi$:
\begin{align*}
R_T^\pi(x) = V^\star_T(x) - V^\pi_T(x)
\end{align*}
where $V^\star_T(x) := \sup_{ \pi \in \Pi} V^\pi_T (x)$.

{\bf Notations and preliminaries.} Let $\Pi_{D}$ be the set of stationary policies, i.e. when in state $X_t=x$, $f\in \Pi_{D}$ selects an action $f(x)$ (independent of $t$). For any $\phi\in \Phi$ and any policy $\pi\in \Pi_D$, we denote by $g^\pi$ its {\it gain} (or long-term average reward): $g_\phi^\pi:=\lim_{T\to\infty}{1\over T}V_T^\pi(x)$ (the limit is independent of $x$ since $\phi$ is irreducible). We denote by $\Pi^\star(\phi)$ the set of stationary policies with maximal gain: $\Pi^\star(\phi):=\{ f \in \Pi_{D}: g_\phi^f= g_\phi^\star\}$, where $g_\phi^\star:=\max_{\pi \in \Pi} g_\phi^\pi$. The {\it bias function} $h_\phi^f$ of $f\in \Pi_D$ is defined by $h_\phi^f(x):=\TN{{\em C}-}\lim_{T\to\infty} \EXP_x^f[\sum_{t = 1}^\infty (R_t  - g_\phi^f(X_t))]$; $h_\phi^f(x)$ quantifies the advantage of starting in state $x$. We denote by $\mathbf{B}^a_\phi$ and $\mathbf{B}^*_\phi$ the Bellman operator of choosing action $a$ and the optimal Bellman operator under $\phi$, respectively, by for any $h: \set{S} \mapsto \mathbb{R}$ and $x \in \set{S}$,
\begin{align*}
(\mathbf{B}^a_\phi h)(x) :=  r_\phi(x,a) + \sum_{y \in \set{S}} p_\phi(y| x,a) h(y) \quad \text{and} \quad
(\mathbf{B}^*_\phi h)(x) := \max_{a \in \set{A}} (\mathbf{B}^a_\phi h)(x) .
\end{align*}
Then for any $f \in \Pi_{D}$, $g_\phi^f$ and $h_\phi^f$ satisfy the {\it evaluation equation}: for all state $x\in\set{S}$, $g_\phi^f+ h_\phi^f(x) = (\mathbf{B}^{f(x)}_\phi  h_\phi^f) (x)$. Furthermore, $f \in \Pi_{D}\in \Phi^\star(\phi)$ if and only if 
$g_\phi^f$ and $h_\phi^f$ verify the {\it optimality equation}: 
\begin{align*}
g_\phi^f + h_\phi^f(x) = (\mathbf{B}^{*}_\phi  h_\phi^{f}) (x).
\end{align*}
We denote by $h_\phi^\star$ the bias function of optimal stationary policies, and by $H$ its span: $H:=\max_{x,y}h_\phi^\star(x)-h_\phi^\star(y)$. For $x\in \set{S}$, $h: \set{S} \mapsto \mathbb{R}$, and $\phi\in\Phi$, let $\set{O}(x;h, \phi) = \{a \in \set{A}: (\mathbf{B}^\star_\phi h)(x) =(\mathbf{B}^a_\phi h)(x) \}$. The set of optimal actions in state $x$ under $\phi$ is hence $\set{O}(x; \phi) := \set{O}(x; h^\star, \phi)$, and $\Pi^*(\phi) = \{f \in \Pi_D : f(x) \in \set{O}(x;\phi) ~\forall x \in \set{S}\}$. Finally, we define for any state $x$ and action $a$, the action sub-optimality gap  $\delta^*(x,a;\phi) =  (\mathbf{B}_\phi^\star h_\phi^\star)(x) - (\mathbf{B}_\phi^a h_\phi^\star)(x)$. $\delta^*(x,a;\phi)$ is interpreted as the gap in long-term reward by initially selecting action $a$ in state $x$ (and then applying an optimal stationary policy) rather then any optimal action. The minimum action sub-optimality gap is defined as $\delta_{\min}:= \min_{(x,a): \delta^*(x,a)>0}\delta^*(x,a;\phi)$.

For two distributions $p_1$ and $p_2$ on $\set{S}$ (resp. on $[0,1]$ and absolutely continuous w.r.t. $\lambda$), we denote by $\| p_1-p_2\|_1\:=\sum_{y\in\set{S}} |p_1(y)-p_2(y)|$ (resp. $\int |p_1(r)-p_2(r)|\lambda(dr)$).




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "./main"
%%% End: 


==> modelnew.tex <==
% !TEX root =  main.tex

\section{Latent learning: Objective and Sampling}

We consider a Markov Decision Process (MDP) with finite state space $\mathcal{S}$, action space $\mathcal{A}$. The dynamics and instantaneous rewards are defined as follows. When the system is in state $s$ and the action $a$ is selected, the system evolves to state $s'$ with probability $p(s'|s,a)$ and the reward $r(s,a,s')$ is collected. The rewards are bounded, i.e., $r(s,a,s')\in [-R_{\max},R_{\max}]$. We observe the system dynamics under a stationary behavior policy $\pi_b$: when in state $s$, action $a$ is selected with probability $\pi_b(s,a)$. Under $\pi_b$, the system evolves as a Markov chain, assumed to admit a unique stationary distribution, and $\mu(s,a)$ denotes the stationary probability of being in state $s$ and selecting action $a$ under $\pi_b$. We also denote by $(s_n,a_n)_{n\ge 0}$ the trajectory of the system observed under $\pi_b$. The objective is to identify, from this trajectory, an optimal policy $\pi^\star: \mathcal{S}\to\mathcal{A}$ maximizing the cumulative discounted reward. 

When starting in state $s$, the expected cumulative discounted reward of a given randomized policy $\pi$ is $\mathbb{E}[\sum_{n=0}^\infty \lambda^n r(s_n^\pi,a_n^\pi,s_{n+1}^\pi) | s_0^\pi=s]$, where $s_n^\pi$ and $a_n^\pi$ denote the state and the action selected under $\pi$ at step $n$, respectively, and where $\lambda\in (0,1)$ is the discount factor. This cumulative reward can be evaluated through the {\it action-value} function $Q^\pi$ of policy $\pi$, defined so that $Q^\pi(s,a)$ represents the cumulative discounted reward given that the system starts in state $s$, that the first selected action is $a$, and that after the first step, actions are chosen according to $\pi$. Indeed, the cumulative reward under $\pi$ is then $\sum_a \pi(s,a)Q(s,a)$. $Q^\pi$ is a fixed point of the Bellman operator of $\pi$, i.e., $Q^\pi = \bold{B}^\pi Q^\pi$ where for any $q: \mathcal{S}\times \mathcal{A} \to \mathbb{R}$,
\begin{align} 
&(\bold{B}^\pi q)(s,a) \nonumber \\
&=\sum_{s' \in \mathcal{S} } \left[r(s, a, s') + \sum_{a' \in \mathcal{A} } \lambda q (s', a') \pi(s,a') \right] p(s'|s,a).
\label{eq:bellman-operator} 
\end{align}
Now for a given function $q:\mathcal{S}\times \mathcal{A} \to \mathbb{R}$, we define the greedy policy $\pi_q$ w.r.t. $q$ as the deterministic policy selecting in state $s$ an action maximizing $q(s,a)$ over $a$ (ties are broken arbitrarily). We further introduce the Bellman operator, defined as $B^\star q = B^{\pi_q}q$ for any $q:\mathcal{S}\times \mathcal{A} \to \mathbb{R}$. It is well known that the action-value function $Q^\star$ of $\pi^\star$ is the fixed point of $B^\star$, and it can be identified for example by applying the $Q$-learning algorithm to the observed trajectory $(s_n,a_n)_{n\ge 0}$. 

\subsection{Linear function approximation}

When the state and action spaces are large, direct methods to identify $Q^\star$ converge very slowly, and we may instead aim at identifying a function that approximates $Q^\star$ well. In this paper, we restrict our attention to searching for such a function within the set $\mathcal{Q}$ of functions parametrized by $\theta\in \mathbb{R}^d$: $\mathcal{Q}=\{ Q_\theta: Q_\theta=\theta^\top \phi,  \theta\in \mathbb{R}^d \}$, where the function $\phi=(\phi_1,\ldots,\phi_d): \mathcal{S}\times \mathcal{A}\to \mathbb{R}^d$ is well chosen. This choice may depend on the system, but is always made so that $\phi$ has linearly independent components. {\tt Additional assumption son $\phi$ should go here}.

\medskip
{\tt Questions to Jungseul: \\
1. Did people directly look at the problem of finding the $\theta$ such that the greedy policy w.r.t. $Q_\theta$ has maximal reward? Here of course you have to rederive Bellman equation since we know that the Bellman operator goes outside $\mathcal{Q}$\\ 
2. Why do we have to have $\mu$ in our objective? It does not make sense if we just want to identify the best Q function approximation.
}

Identifying the parameter $\theta^\star$ such that the greedy policy w.r.t.  $Q_{\theta^\star}$ has maximum cumulative reward among all greedy policies constructed from functions in ${\cal Q}$ is challenging. This is mainly due to the fact that in general, the set ${\cal Q}$ is not stable by Bellman operator, and hence algorithms aiming at minimizing the mean-square Bellman error $\| Q_\theta - B^\star Q_\theta\|^2$ (for some norm) may diverge \citet{baird1995residual}. To circumvent this difficulty, we rather aim at minimizing the so-called mean-square projected Bellman error, MSPBE, see e.g. \cite{maei2010toward}: 



\iffalse


where $s_n \in \mathcal{S}$, $a_n \in \mathcal{A}$, and $r_{n+1} \in (-R_{\max}, R_{\max})$
are the $n$-th state, action, and reward, respectively.
%Let $\mathcal{H}_n = (s_0, a_0, r_1, ..., s_n)$ be the history up to the $n$-th state.
Let $P$ be the joint distribution kernel of next state and reward, depending on only the current state and action,
i.e., $(s_{n+1}, r_{n+1}) \sim P(\cdot, \cdot~; s, a)$ given $(s_n, a_n) = (s,a)$.
%, independently of $\mathcal{H}_n$ given $(s_n, a_n)$.
We assume that a stationary policy $\pi_b$, often called {\it behavior policy}, generates sequence of transitions
with selecting $a_n = a$ with probability $\pi_b(s, a)$ at state $s_n = s$.
Then, the sequence of pairs of state and action is 
a Markov process. % with $\mathcal{S} \times \mathcal{A}$.
Through out this paper, we further assume that the Markov process has 
a unique\footnote{It is sufficient to assume irreducible Markov process with finite state space for the uniqueness of stationary distribution.} stationary distribution $\mu$ over $\mathcal{S} \times \mathcal{A}$. 


We address the {\it off-policy} control problem of the MDP $(\mathcal{S}, \mathcal{A}, P)$, which
finds an optimal policy $\pi^*$ with maximum value from samples generated by another policy $\pi_b$. 
%as
%$Q^\pi(s,a) = \EXP [ \sum_{n = 0}^\infty \lambda^n r(s, a, s')]$
A classic approach is studying action-value function $Q^\pi$ of policy $\pi$, which verifies 
a recursion $Q^\pi = \bold{B}^\pi Q^\pi$.
Here $\bold{B}^\pi$ is the Bellman operator of $\pi$ such that
for any $q: \mathcal{S}\times \mathcal{A} \to \mathbb{R}$,
\begin{align} 
&(\bold{B}^\pi q)(s,a) \nonumber \\
&=\sum_{s' \in \mathcal{S} } \left[r(s, a, s') + \sum_{a' \in \mathcal{A} } \lambda q (s', a') \pi(s,a') \right] P_a (s, s')
\label{eq:bellman-operator} \;,
\end{align}
%where $r(s, a, s')$ is the expected reward of selecting action $a$ at state $s$,
%and $P_a(s, s')$ is the probability of transition to state $s'$ from state $s$ chosen action $a$.
where $\lambda  \in [0,1)$ is discount factor, and 
$r(s, a, s')$ and $P_a(s, s')$ are the expected reward and the probability of transition to state $s'$ from acting $a$ at state $s$, respectively.
Denote $\pi_Q$ be a greedy policy\footnote{We break tie arbitrarily.} of $Q$, which selects actions maximizing $Q(s, \cdot)$ at each state $s$.
It is well known that 
the optimal policy $\pi^*$ is the greedy policy of the optimal action-value function $Q^*$ such that 
$Q^* = \bold{B}^{*}Q^*$ where $\bold{B}^{*}$ is Bellman operator of greedy policy, i.e., $\bold{B}^{*}q = \bold{B}^{\pi_q}$. $Q$-learning is the famous algorithm for solving such a fixed point problem \cite{watkins1992q}. 
















More formally, we want to find $\pi^*$ that maximizes the value function $V^\pi$:
\begin{align*}
V^\pi ( s) &:= \EXP \left[ \lim_{n\to\infty}\sum_{k=0}^{n} \lambda^{k} r(s^\pi_k, a^\pi_k, s^\pi_{k+1}) \mid s^\pi_0 = s \right] \;. % \; \text{and}\\
\end{align*}
Note that it is an {\it off-policy} learning scenario
where we learn about a policy, so called {\it target policy}, from observations collected by another policy, so called {\it behavior policy}.
It is well known that a greedy policy of the optimal action-value function $Q^*$ is the optimal policy,
where $Q^*$ is the fixed point of the Bellman operator $\bold{B}$.

\begin{compactenum}
\item {\bf Define Bellman operator $\bold{B}^\pi$}

The value of $\pi$ is denoted by function $V^\pi:\mathcal{S} \to \mathbb{R}$,
where $V^\pi (s)$ is the expected discounted reward started from state $s$ under $\pi$.

where $\lambda \in [0,1)$ is discount factor,
and the expectation is taken with respect to the generation of 
$s^\pi_{n+1} \sim P_{\mathcal{S}}(\cdot \mid s^\pi_n, a^\pi_n )$ and $a^\pi_n \sim \pi(\cdot \mid s^\pi_n)$
given $s^\pi_0 = s$ according to target policy $\pi$ for all $n \ge 0$. 
Similarly, the action-value of $\pi$ is 
denoted by $Q^\pi: \mathcal{S} \times \mathcal{A} \to \mathbb{R}$,
where $Q^\pi (s, a)$ is the expected discounted reward starting from $(s,a) \in \mathcal{S} \times \mathcal{A}$,
and following policy $\pi$ afterward, i.e.,
\begin{align*}
Q^\pi (s, a) 
&:= \sum_{s' \in \mathcal{S}} \left[r(s, a, s') + \lambda V^\pi (s') \right] P_{\mathcal{S}} (s' \mid s, a) \\
&= \sum_{s' \in \mathcal{S}} \left[r(s, a, s') + \sum_{a' \in \mathcal{A}}\lambda Q^\pi (s', a') \pi(a' \mid s') \right] P_{\mathcal{S}}(s' \mid s, a) \;.
\end{align*}
We note that the action-value function is a fixed point of the Bellman operator $\bold{B}^\pi$ of $\pi$,
$\bold{B}^\pi Q^\pi = Q^\pi$,
where for any $q: \mathcal{S}\times \mathcal{A} \to \mathbb{R}$,
\begin{align} \label{eq:bellman-operator}
(\bold{B}^\pi q)(s,a)
&: = \sum_{s' \in \mathcal{S}} \left[R(s, a, s') + \sum_{a' \in \mathcal{A}}\lambda q (s', a') \pi(a' \mid s) \right] P_a (s, s')\;.
\end{align}

\end{compactenum}



\fi 

\iffalse



In particular, it is the most interest of to find an optimal policy $\pi^*$ maximizing 
the value function, i.e., 
\begin{align*}
\pi^* := \argmax_{\pi} V^\pi(s) \;.
\end{align*}
In order to find the optimal policy, one can use $Q$-function $Q^\pi (s, a)$ defined as 
the expected cumulated rewards where the first state and action are $s$ and $a$:
\begin{align*}
Q^\pi (s, a) 
&:= \sum_{s' \in \mathcal{S}} \left[R(s, a, s') + \lambda V^\pi (s') \right] P_a (s, s') \\
&= \sum_{s' \in \mathcal{S}} \left[R(s, a, s') + \sum_{b \in \mathcal{A}}\lambda Q^\pi (s', b) \pi(s, b) \right] P_a (s, s') \;,
\end{align*}
where $\pi(s, a)$ is the probability that policy $\pi$ selects action $a$ at state $s$.
Define $\bold{B}^\pi$
and $\bold{B}^*$, called the Bellman operator of policy $\pi$
and the Bellman optimal operator as follows:
\begin{align*}
(\bold{B}^\pi Q)(s,a)\;,
&: = \sum_{s' \in \mathcal{S}} \left[R(s, a, s') + \sum_{b \in \mathcal{A}}\lambda Q (s', b) \pi(s, b) \right] P_a (s, s')\;, \\
(\bold{B}^* Q)(s,a)\;,
&: = \sum_{s' \in \mathcal{S}} \left[R(s, a, s') + \max_{b \in \mathcal{A}}\lambda Q (s', b) \right] P_a (s, s')\;.
\end{align*}
Let $V^*:= V^{\pi^*}$ and $Q^*:= Q^{\pi^*}$. 
Then, $Q^\pi$ and $Q^*$ are fixed points of $\bold{B}^\pi$ and $\bold{B}^*$, respectively.
Note the following recursive relation of $Q^*$ (or $Q^\pi$):
\begin{align}
Q^* (s,a) &= (\bold{B}^* Q^*)(s,a) \label{eq:recursive-Bellman-operator} \\
& = 
\sum_{s' \in \mathcal{S}} \left[R(s, a, s') + \lambda  V^*(s') \right] P_a (s, s')  \;. \nonumber
%\\
%&= 
%\sum_{s' \in \mathcal{S}} \left[R(s, a, s') + \lambda \max_{b \in \mathcal{A}} Q^*(s', b) \right] P_a (s, s')\;,
\end{align}



We denote by $V^\pi$ and $Q^\pi$ 
the value and action-value of target policy $\pi$ with discount factor $\lambda \in [0, 1)$,
which are the expected discounted reward started at state $s$ following $\pi$ from the start
or following $\pi$ after selecting action $a$, respectively. 
More formally, we define
\begin{align*}
V^\pi ( s) &:= \EXP \left[ \sum_{n=0}^{\infty} \lambda^{n} r(s_n, a^\pi_n, s_{n+1}) \mid s_0 = s \right] \;, \\ 
Q^\pi (s, a) 
&:= \sum_{s' \in \mathcal{S}} \left[r(s, a, s') + \lambda V^\pi (s') \right] P_a (s, s') \\
&= \sum_{s' \in \mathcal{S}} \left[r(s, a, s') + \sum_{b \in \mathcal{A}}\lambda Q^\pi (s', b) \pi(s, b) \right] P_a (s, s') \;.
\end{align*}
where $r(s, a, s')$ is the expected immediate reward at transition $(s, a, s')$,
$a^\pi_n \sim \pi(\cdot \mid s_n)$.

\fi

%which is the expectation of accumulated reward starting from state $s$ with discount factor $\lambda$.
%Once we In particular, it is the most interest of to find an optimal policy $\pi^*$ maximizing 
%the value function, i.e., 
%\begin{align*}
%\pi^* := \argmax_{\pi} V^\pi(s) \;.
%\end{align*}
%In order to find the optimal policy, one can use $Q$-function $Q^\pi (s, a)$ defined as 
%the expected cumulated rewards where the first state and action are $s$ and $a$:
%where $\pi(s, a)$ is the probability that policy $\pi$ selects action $a$ at state $s$.


%For any $Q: \mathcal{S} \times \mathcal{A} \to \mathbb{R}$,
%we define 
%the Bellman operator $\bold{B}^\pi$ of $\pi$
%and Bellman optimal operator $\bold{B}^*$ as follows:
%\begin{align*}
%(\bold{B}^\pi Q)(s,a)
%&: = \sum_{s' \in \mathcal{S}} \left[R(s, a, s') + \sum_{b \in \mathcal{A}}\lambda Q (s', b) \pi(s, b) \right] P_a (s, s')\;, \\
%(\bold{B}^* Q)(s,a)
%&: = \sum_{s' \in \mathcal{S}} \left[R(s, a, s') + \max_{b \in \mathcal{A}}\lambda Q (s', b) \right] P_a (s, s')\;.
%\end{align*}




%In particular, it is the most interest of estimating $Q$-function of optimal policy $\pi^*$
%that maximizes the value, i.e., $\pi^* := \argmax_{\pi} V^\pi(s)$ for all $s \in \mathcal{S}$.
%
%to find an optimal policy $\pi^*$ maximizing 
%the value, i.e., 
%
%Let $V^*:= V^{\pi^*}$ and $Q^*:= Q^{\pi^*}$. 
%Then, $Q^\pi$ and $Q^*$ are fixed points of $\bold{B}^\pi$ and $\bold{B}^*$, respectively.
%Note the following recursive relation of $Q^*$ (or $Q^\pi$):
%\begin{align}
%Q^* (s,a) &= (\bold{B}^* Q^*)(s,a) \label{eq:recursive-Bellman-operator} \\
%& = 
%\sum_{s' \in \mathcal{S}} \left[R(s, a, s') + \lambda  V^*(s') \right] P_a (s, s')  \;. \nonumber
%%\\
%%&= 
%%\sum_{s' \in \mathcal{S}} \left[R(s, a, s') + \lambda \max_{b \in \mathcal{A}} Q^*(s', b) \right] P_a (s, s')\;,
%\end{align}
%%where the last equality is from the optimality of $V^*(s)$.
%Hence selecting action $\argmax_{a \in \mathcal{A}} Q^*(s, a)$
%is the optimal policy in a sense that the corresponding control process $\{A_n\}$ such that $ A_n = \argmax_{a \in \mathcal{A}} Q^*(S_n, a)$
%achieves the optimal value function $V^*$.
%Therefore, the problem to find an optimal policy is solved once the function $Q^*$ is obtained for all $(s, a) \in \mathcal{S} \times \mathcal{A}$.



\subsection{Objective Function}
%{\note Alexandre, can you replace $\theta'$ denoting parameter that defines policy with $\vartheta$?...}
Such a scalability issue of $Q$-learning algorithm
is addressed by approximating action-value function with few parameters.
We use a linear approximation $Q_\theta (s,a) = \theta^\top \phi(s,a)$
with the parameter vector $\theta \in \mathbb{R}^d$ and the feature vector $\phi(s,a) = [\phi_1(s,a), ..., \phi_d (s,a)]^\top$.
 %$\{\varphi_i \in \mathbb{R}^{|\mathcal{S} \times \mathcal{A}|} : j = 1,.., d\}$ of feature functions
Recalling that the optimal state-action function $Q^*$ without approximation 
is the fixed point of $Q^* = \bold{B}^{*} Q^*$,
it is natural to find $\theta^*$ verifying $Q_{\theta^*} = \bold{T} \bold{B}^{*} Q_{\theta^*}$.
%Here, $\pi_{\theta} := \pi_{Q_{\theta}}$ is the greedy policy of $Q_\theta$,
Here $\bold{T}$ is the projection operator onto $\mathcal{Q} := \{Q_\theta : \theta \in \mathbb{R}^d\}$ such that
for any $q: \mathcal{S} \times \mathcal{A} \to \mathbb{R}$,
\begin{align*}
\bold{T} q  = 
\argmin_{Q_\theta \in \mathcal{Q} } \|Q_\theta - q\|^2_{\mu} \;,
%Q_\theta \quad \text{where}~\theta = \argmin_{\theta \in \mathbb{R}^d } \|Q_\theta - q\|^2 \;
\end{align*}
where we define $\|q\|^2_{\mu} := \sum q^2 (s,a) \mu(s,a)$ as the expectation of $q^2(s, a)$
over stationary distribution $\mu$.
%with respect to $s \sim \mu(\cdot)$ and $a \sim \pi_b(s, \cdot)$.
%\begin{align}
%\|q\|^2_{\mathcal{H}} &:= 
%\sum_{s \in \mathcal{S}} q^2(s, a) \mu(s) \pi_b(a \mid s)
%= \lim_{n \to \infty} \EXP\left[ \frac{1}{n} \sum_{k = 0}^n q^2(s_k, a_k) \right]  
% \;. \label{eq:norm}
%\end{align}



% transient from another time-scale separation between temporal learning and gain matrix.
%and 
To find the fixed point of $\bold{T} \bold{B}^{*}$,
we consider a constraint minimization of mean square projected Bellman error (MSPBE) with two sets of parameters $\theta, \theta' \in \mathbb{R}^d$:
\begin{align}  \label{eq:double-object}
\mathcal{E}(\theta, \theta') :=  \| Q_\theta - \bold{T} \bold{B}^{{\theta'}} Q_\theta \|^2_{\mu} \;,
%\textnormal{subject to }&~~ \vartheta = \theta \in \mathbb{R}^d
%\;. \nonumber
\end{align}
where $\bold{B}^{{\theta'}}$ is Bellman operator of greedy policy $\pi_{\theta'} := \pi_{Q_{\theta'}}$ with respect to $Q_{\theta'}$.
Here once we fix $\theta'$, the minimization problem of $\mathcal{E}(\theta, \theta')$ 
corresponds to the policy {\it evaluation} problem for target policy $\pi_{\theta'}$
to find $Q^{\pi_{\theta}}$.
Hence,  we are particularly interested in a constrained minimization of \eqref{eq:double-object} such that $\theta = \theta'$.
A fixed point $\theta^*$ of $\bold{T}\bold{B}^{*}$
minimizes \eqref{eq:double-object} with $\mathcal{E}(\theta^*, \theta^*) = 0$
if it exists.


From the calculation in \cite{sutton2009fast},
we have
\begin{align} 
\mathcal{E}(\theta, \theta') 
= \EXP_\mu [ \delta (\theta, \theta') {\varphi}]^\top
\EXP_\mu [ \varphi {\varphi}^\top]^{-1}
\EXP_\mu [ \delta (\theta, \theta') {\varphi}] \;,  \nonumber \footnotemark
% \label{eq:MSPBE-calc}
\end{align}
where the expectation is taken with respect to random transition
$(\hat{s}, \hat{a}, \hat{r}, \hat{s}')$ such that
$(\hat{s}, \hat{a}) \sim \mu(\cdot, \cdot)$
and $(\hat{s}', \hat{r}) \sim P(\cdot, \cdot ; \hat{s}, \hat{a})$,
and $\delta (\theta, \theta')$ is the temporal error, defined by
\begin{align} \label{eq:def-delta}
\delta (\theta, \theta') := \hat{r} + \lambda \theta^\top \varphi'(\theta')  - \theta^\top \varphi 
\end{align}
with 
$\varphi := \phi(\hat{s},\hat{a})$ and $\varphi'(\theta') :=  \sum_{a'} \phi(\hat{s}', a') \pi_{\theta'}(\hat{s}', a' ).$
Hence, the minimizer of $\mathcal{E}(\theta, \theta)$ in \eqref{eq:double-object} 
can be interpreted as $\theta^*$ such that $\mathcal{D}(\theta^*, \theta^*) = 0$ where we define
expected 
\begin{align} \label{eq:td-error}
\mathcal{D}(\theta, \theta') := \EXP_\mu [ \delta(\theta, \theta')  \varphi ]\;.
\end{align}






\subsection{Derivation of \alg}


To find $\theta^*$ in \eqref{eq:optimal-theta},
there have been proposed variety of algorithms.
We can classify them into two groups: direct and indirect ones.
First, direct approaches update target policy and its evaluation at each given sample, e.g.,
Greedy-GQ \cite{maei2010toward} and ZAP-Q \cite{devraj2017zap}.
Such dramatic updates sometimes reduce convergence time.
However, due to discontinuity of target policy $\pi_\theta$ in $\theta$,
a single random sample often causes unbounded behavior
(see Section~\ref{sec:numerical} for numerical examples).
For this reason, convergence guarantee requires somewhat unnatural assumptions such as
explicitly restricting frequency of target policy change \cite{devraj2017zap}.
%However, $\mathcal{E}(\theta, \theta)$ is non-differentiable with respect to $\theta$ , while it is piecewise quadratic.
%Based on the sub-gradient of $\mathcal{E}(\theta, \theta)$,
%one can develop algorithms, which evaluates and greedily improves target policy $\pi_\theta$ at the same time,
%e.g., $Q$-learning \cite{watkins1992q}, 
%However, 
%%It is worthy to mention that the instability is not a matter of 

To bypass the sub-gradient issue and to secure stability,
indirect approaches separate the policy evaluation and improvement, e.g., 
{\note LSPI? Some related works are in our dropbox folder (reading-9policy-iter).}...
DQN \cite{mnih2013playing}.


{\note Some notes on synchronization duration $\tau$...}


Although these approaches provide more stability compared to direct ones,
they are often criticized as the slow convergence.
Hence, we propose an indirect algorithm, named \alg, which employs
several techniques to improve convergence speed: batch sample and
gain matrix.


{\note At some point, place the following introduction on sampling...}
Hence, from stochastic gradient method minimizing \eqref{eq:double-object},
%to minimize $\mathcal{E} (\vartheta, \theta)$ under constraint of $\vartheta =  \theta$,
we develop \alg (Algorithm~\ref{alg:ours}) 
of which $n$-th update uses a batch of
sampled transitions $\xi_n = (\hat{s}_{n,i}, \hat{a}_{n,i}, \hat{r}_{n,i}, \hat{s}'_{n,i})_{i = 1, ..., B}$. In particular, we consider two sampling schemes: 

{\textbf{\textit{ Random sampling}}}: At the $n$-th iteration, it generates 
$B$ independent  transitions $\xi_n^{\iid} := (\hat{s}_{n,i}, \hat{a}_{n,i}, \hat{r}_{n,i}, \hat{s}'_{n,i})_{i = 1, ..., B}$,
where
$\hat{s}_{n,i} \stackrel{\text{iid}}{\sim} \mu$, $\hat{a}_{n,i} \stackrel{\text{iid}}{\sim} \pi_b(\hat{s}_{n, i}, \cdot)$,
$\hat{s}'_{n,i} \stackrel{\text{iid}}{\sim} P_{\hat{a}_{n,i}}(\hat{s}_{n,i}, \cdot)$, and $\hat{r}_{n,i}$ is the corresponding random reward.
%variable conditionally independent of $n$ given $\hat{s}_n, \hat{a}_n, \hat{s}'_n$ where $\EXP [\hat{r}_n \mid \hat{s}_n, \hat{a}_n, \hat{s}'_n] = r(\hat{s}_n, \hat{a}_n, \hat{s}'_n)$.
% each of which starts at a state independently drawn from stationary distribution $\mu$.
%it first draws $B$ states from stationary distribution $\mu$ independently, and then
%obtains $B$ transitions started at 
%correspondingly selects the action, the next state and the reward, i.e.,

{\textbf{\textit{ Experience replay}}}: 
This scheme is given a stream of transitions $(s_n, a_n, r_n, s'_n)_{n \ge 0}$ generated by the behavior policy $\pi_b$,
where we denote $s'_n := s_{n+1}$. 
At the $n$-th iteration, it stores the $W$ most recent transitions from the $(n+W-1)$-th transition to window $W_n = ({s}_{n+k}, {a}_{n+k}, {r}_{n+k}, {s}'_{n+k})_{0 \le k < W} $ of size $W$, and draws $B$ transitions $\xi_n^{\textnormal{ER}} := (\hat{s}_{n,i}, \hat{a}_{n,i}, \hat{r}_{n,i}, \hat{s}'_{n,i})_{i = 1, ..., B}$ independently uniformly at random from $W_n$.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{
\begin{algorithm}[tb]
   \caption{\alg}
   \label{alg:ours}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:}    sequences of step sizes $\alpha_n, \beta_n$
    and sample batches $\xi_n = (\hat{s}_{n,i}, \hat{a}_{n,i}, \hat{r}_{n,i}, \hat{s}'_{n,i})_{i = 1,..., B}$, and duration $\tau$.
    
      \STATE Initialize $\theta_0, \theta'_0 \in \mathbb{R}^d$, $\Gamma_0 \in \mathbb{R}^{d \times d}$, $n = m =  0$.
%\STATE {\bf repeat}%
   \REPEAT
  \STATE
   Process sample $\xi_n$ based on $\theta'_m$
   for $A_{n} :=\frac{1}{B} \sum_{i = 1}^B  A_{n,i}(\theta'_{m})$ and $b_{n} :=\frac{1}{B} \sum_{i = 1}^B  b_{n,i}$, where
   \begin{align*}
  \varphi_{n, i} &:= \phi(\hat{s}_{n,i}, \hat{a}_{n,i}) \;,\\
 \varphi'_{n, i}(\theta'_m) &:=   \sum_{a' \in \mathcal{A}} \phi(\hat{s}'_{n,i}, a') \pi_{\theta^-_m} (\hat{s}'_{n,i}, a')\;, \\
A_{n, i} (\theta'_{m}) &:= 
\varphi_{n,i} (\lambda \varphi'_{n,i}(\theta'_{m}) - \varphi_{n,i})^\top \;,
\\
b_{n, i} &:= 
 \hat{r}_{n,i} \varphi_{n,i}  \;.
\end{align*}
\STATE Update $\theta_{n+1}$, $\hat{A}_{n+1}$ as follows:
\begin{align}
%\!\!\!\!\!\!\!\! \theta_{n+1} &= \theta_n + \alpha_n (\vartheta_{n+1}- \theta_n) \;, \label{eq:update-policy} \\
\!\!\!\!\!\!\!\! \theta_{n+1} 
&= \theta_n + \alpha_n  \Gamma_{n+1} (A_{n} \theta_n + b_{n})
\label{eq:update-temporal} \;,  \\
\!\!\!\!\!\!\!\!
\hat{A}_{n+1} &= \hat{A}_n  + \beta_n (A_{n} - \hat{A}_n) \label{eq:update-gain}
 \;,
\end{align}
where  $\Gamma_{n+1} : = - \hat{A}_{n+1}^{[+]}$.\footnotemark


%\STATE $\Gamma_{n+1} = \Gamma_n  + \gamma_n (\Gamma_{n} - \hat{G}_n)$
%%\STATE $\Gamma_{n+1} = \langle \hat{G}_{n+1} \rangle^{-1} $
%\STATE $\varrho_{n+1} = \varrho_n  + \beta_n \langle \Gamma_{n+1} \rangle^{-1} (G_{n+1} \varrho_n - \varrho_n)$
%\STATE $\theta_{n+1} = \theta_n  + \alpha_n (\vartheta_n - \theta_n)$ recalling $\varrho_n = [ w_n^\top , \vartheta_n^\top]^\top$

%   \FOR{$i=1$ {\bfseries to} $m-1$}
%   \IF{$x_i > x_{i+1}$}
%   \STATE Swap $x_i$ and $x_{i+1}$
%   \STATE $noChange = false$
%   \ENDIF
%   \ENDFOR
\STATE Increase $n$ to $n+1$, and $t_\alpha$ to $t_\alpha + \alpha_n $.
   \IF{$t_\alpha \ge \tau$}
\STATE Update ${\theta'_{m+1}} = {\theta_{n+1}}$, increase $m$ to $m+1$, and reset $t_\alpha$ to $0$ .
   \ENDIF
   \UNTIL{$\theta_n$ converges}
\end{algorithmic}
\end{algorithm}
\footnotetext{ We denote by $A^{[+]}$ a projected inverse (or pseudoinverse) of matrix $A$,
in which the projection ensures $\|A^{[+]}\| < b_{\Gamma}$ for some $b_{\Gamma}  > \max_{\theta} \|(A(\theta))^{-1}\|$
for all $A(\theta)$ defined in \eqref{eq:def-A}.
%  Moore-Penrose inverse of matrix $A$ .
%, we use $\langle \cdot \rangle$ is a projection to ensure boundedness of $\langle \cdot \rangle^{-1}$,  
}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Policy Evaluation}
For given $\theta'$, $\theta$ such that $\mathcal{D}(\theta,  \theta') = 0$ corresponds to
a solution of the following linear equation:
\begin{align*}
A(\theta') \theta + b  = 0 \;,
\end{align*}
where with the same $\varphi, \varphi'(\theta'), \hat{r}$ in \eqref{eq:def-delta},
\begin{align}
A(\theta') :=  \EXP_\mu \left[ \varphi  (\varphi - \lambda \varphi'(\theta')) ^\top \right]  ~~ and ~~
b := \EXP_\mu \left[ \hat{r} \varphi \right] \label{eq:def-A} \;.
\end{align}
%$C := \EXP_\mu \left[ \varphi \varphi^\top \right]$,
This proposes a linear recursion of $\theta_n$ \cite{sutton1988TD}:
\begin{align}  \label{eq:no-gain}
\theta_{n+1} = \theta_{n} + \alpha_n (A_{n+1}\theta_n + b_{n+1}) \;,
\end{align}
of which associated ODE is
\begin{align} \label{eq:ode-given}
\dot{\theta}(t) = A(\theta') \theta(t) + b
\end{align}
Even if $A(\theta') = \EXP_\mu (A_{n})$ is invertible, the above recursion can cause divergence of $\theta_n$.
Indeed, when $A(\theta')$ is invertible but is not Hurwitz, the system is diverging.
To fix such problem, \citet{sutton2009fast, sutton2009convergent} proposed
gradient based TD algorithms (GTD, GTD2, TDC) on minimizing $\mathcal{E}(\theta, \theta')$,
where for given $\theta'$, $\mathcal{E}(\theta, \theta')$ is differentiable 
with
\begin{align*}
&-\frac{1}{2}\nabla_{\theta'} \mathcal{E} (\theta, \theta') \\
&= 
\EXP_\mu \left[  (\varphi - \lambda \varphi'(\theta')) \varphi^\top \right]
\EXP_\mu \left[ \varphi \varphi^\top \right]^{-1}
 \EXP_\mu \left[\delta(\theta, \theta') \varphi \right] \;.
 \end{align*}
The gradient based algorithms use
auxiliary parameter vector $w \in \mathbb{R}^d$ to approximate $\EXP_\mu \left[ \varphi \varphi^\top \right]^{-1}
 \EXP_\mu \left[\delta(\vartheta, \theta) \varphi \right]$ or $\EXP_\mu \left[\delta(\vartheta, \theta) \varphi \right]$.
This yields a stable associated ODE, e.g., 
GTD \cite{sutton2009convergent} has 
$[\dot{w}(t)^\top, \dot{\theta}(t)^\top]^\top = G(\theta') [{w}(t)^\top, {\theta}(t)^\top]^\top + [b, 0]^\top$
with
\begin{align*}
G(\theta'):=
\begin{bmatrix}
-I & A(\theta')\\
-A(\theta')^\top & 0
\end{bmatrix} \;,
\end{align*}
which is Hurwitz if $A(\theta')$ is invertible, and thus the system is stable.


%\begin{align*}
%\begin{bmatrix}
%\dot{w}(t) \\
%\dot{\theta}(t)
%\end{bmatrix}
%=
%\begin{bmatrix}
%-I & A\\
%-A^\top & 0
%\end{bmatrix}
%\begin{bmatrix}
%{w}(t) \\
%{\theta}(t)
%\end{bmatrix}
%+ 
%\begin{bmatrix}
%b \\
%0
%\end{bmatrix} \;,
%\end{align*}
%in which $G =d$
%In particular, GTD2 \cite{sutton2009fast} uses the following update:
%\begin{align*}  
%\begin{bmatrix}
%w_{n+1}  \\
%\theta_{n+1} 
%\end{bmatrix}
%= 
%\begin{bmatrix}
%w_{n} \\
%\theta_{n}
%\end{bmatrix}
%+
%\alpha_n
%\left(
%\begin{bmatrix}
%- C_{n+1} & A_{n+1}\\
%A_{n+1} & 0
%\end{bmatrix}
%\begin{bmatrix}
%w_{n} \\
%\theta_{n}
%\end{bmatrix}
%+ \begin{bmatrix}
%b_{n+1} \\
%0
%\end{bmatrix}
%\right)
%%&= \theta_n + \alpha_n  (\varphi - \lambda \varphi'(\theta'))
%%\varphi^\top w_n \;, \\
%%w_{n+1} &=w_n + \alpha_n (\delta(\theta_n, \theta') - \varphi^\top w_n)
%%\varphi  \;.
%\end{align*} 
 
 
Instead of employing the auxiliary parameter $w$,
we address such issue by obtaining matrix inversion $\Gamma(\theta') \approx -A(\theta')^{-1}$ directly.
This results update  in \eqref{eq:update-temporal} and \eqref{eq:update-gain},
and the associated ODE of $\theta$ is 
\begin{align*}
\dot{\theta}(t)  = {\Gamma(\theta')A(\theta')} \theta(t) + \Gamma(\theta') b \;,
\end{align*}
where if 
$A(\theta')$ is invertible, $\Gamma(\theta')A(\theta')$ becomes $-I$ which is Hurwitz.
To make our algorithm general, we will take pseudoinverse if $A(\theta')$ is not invertible.
This approach is also known as Newton-Raphson, in which $\Gamma(\theta')$ is referred
to as gain matrix (see Chapter~4, Part~I of \cite{benveniste2012adaptive} for general discussion on gain matrix).
Some notes about optimality of our gain .. optimal for linear system solver. 
{\note
Since \citet{devraj2017zap} improves convergence speed.....
Although, gain matrix is not necessary for achieving optimal covariance (if $\alpha_n = \frac{1}{n+1}$ see Konda paper..), but improves the transient behavior as in ZAP Q learning.
}



\clearpage


%We have 
%\begin{align}
%%\!\!\!\!\!\!\!\! \theta_{n+1} &= \theta_n + \alpha_n (\vartheta_{n+1}- \theta_n) \;, \label{eq:update-policy} \\
% \theta_{n+1}  &= \theta_n + \alpha_n  \Gamma_{n+1} (A_{n+1} \theta_n + b_{n+1}) \\ 
%\hat{A}_{n+1} &= \hat{A}_n  + \beta_n (A_{n+1} - \hat{A}_n)
%\end{align}
%where  $\Gamma_{n+1} : = - \hat{A}_{n+1}^{[+]} \approx -A^{-1}$.

{\note A page of potentially useful garbage.

We update $\theta$ and $\vartheta$ of $\mathcal{E}(\vartheta, \theta)$
in two separate time-scales with choice of $\alpha_n  \ll \beta_n$.
Since $\theta'$ varies slower than $\theta$,
updating $\theta$ can be viewed as evaluating a fixed target policy $\pi_{\theta'}$ for short time,
while $\theta'$ slowly tracking $\theta$ eventually improves control $\pi_{\theta'}$.
Similar time-scale separation technique is used for deep $Q$-network (DQN) \cite{mnih2013playing}.
% target network vs current network...
% two time-scales corresponding to $(\alpha_n)_{n\ge 0}$ and $(\beta)_{n\ge 0}$
%such that $\alpha_n, \beta_n, \alpha_n / \beta_n  \to 0$
%and decompose minimization of MBPBE into two parts: (i) update $\theta$ with step size $\alpha_n$ (control learning)
%and (ii) update $\vartheta$ given $\theta$ with step size $\beta_n$ (temporal learning).
First, the simple recursion \eqref{eq:update-policy} lets $\theta_n$ slowly follow after $\vartheta_n$.
Then, the rest


Employing the same linear predictor $w_n \in \mathbb{R}^d$ of
$\EXP_\mu \left[ \varphi \varphi^\top \right]^{-1}
 \EXP_\mu \left[\delta(\vartheta, \theta) \varphi \right]$ proposed by \citet{sutton2009fast},
we first obtain a linear recursion of $\vartheta_n$ and $w_n$ to minimize $\mathcal{E}(\varepsilon, \theta)$ given $\theta$:
\begin{align*}  
\vartheta_{n+1} 
&= \vartheta_n + \beta_n  (\varphi - \lambda \varphi'(\theta))
\varphi^\top w_n \;, \\
w_{n+1} &=w_n + \beta_n (\delta(\vartheta_n, \theta) - \varphi^\top w_n)
\varphi  \;,
\end{align*}
with the same $\varphi$,$\varphi', \delta$ in \eqref{eq:def-delta}.
{\note Explain matrix form with $\varphi$: Further, $\vartheta_n$ and $w_n$ vector form, conclude 
the special case of \eqref{eq:update-temporal} plugging identity matrix in $\Gamma_{n+1}$.
}


{\note Why $w$ is necessary:
Since the gradient $\nabla_{\vartheta} \mathcal{E} (\vartheta, \theta)$ involves
multiplication of expectations, we cannot directly sample the entire gradient.
Hurwitz (GTD) , ZAP Q learning doesn't have this correction, while at the steady state, the gain matrix makes $\Gamma A = -I$ Hurwitz...
}





The constrained minimization of \eqref{eq:double-object} can be addressed
in various ways. First, one can directly consider minimization of $\mathcal{E}(\theta, \theta)$, e.g., Greedy-GQ \cite{maei2010toward} and ZAP-Q \cite{devraj2017zap}.
Unfortunately, $\mathcal{E}(\theta, \theta)$ is not differentiable due to discontinuity of $\pi_{\theta}$.
Hence, such direct approaches employ sub-gradient of $\mathcal{E}(\theta, \theta)$...
{\note
Oscillation since the sub-gradient allows a single random observation to change
direction of policy improvement $\pi_\theta$. (see Section~\ref{sec:numerical} for numerical examples)}
%Hence 
%there have been proposed variety of stochastic sub-gradient methods, e.g.,
%$Q$-learning \cite{watkins1992q}, 
%Greedy-GQ \cite{maei2010toward} and ZAP-Q \cite{devraj2017zap}.
%However, such algorithms often suffer from slow and unstable convergence due to unwanted cycle of updates between temporal and control learnings (see Section~\ref{sec:numerical} for numerical examples),
%although convergence guarantee is available even with correlated samples under mild assumptions, e.g., \cite{devraj2017zap}.




\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm*}[tb]
   \caption{\alg learning}
   \label{alg:ours}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} sequences of step sizes $\alpha_n, \beta_n, \gamma_n$ and sample batches $\xi_n = (\hat{s}_{n,i}, \hat{a}_{n,i}, \hat{r}_{n,i}, \hat{s}'_{n,i})_{i = 1,..., B}$
      \STATE Initialize $\theta_0 \in \mathbb{R}^d$, $\varrho_0 = [ w_0^\top , \vartheta_0^\top]^\top \in \mathbb{R}^{2d}$, $\hat{G}_0 \in \mathbb{R}^{2d \times 2d}$, $n = 0$.
   \REPEAT
   \STATE 
   Prepare  $G_{n+1} :=\frac{1}{B} \sum_{i = 1}^B  G_{n+1,i}$ and $g_{n+1} :=\frac{1}{B} \sum_{i = 1}^B  g_{n+1,i}$
   from sample batch $\xi_n$, where 
   $\varphi_{n, i} := \phi(\hat{s}_{n,i}, \hat{a}_{n,i})$,
   $ \varphi'_{n, i} := \sum_{a' \in \mathcal{A}} \phi(\hat{s}'_{n,i}, a') \pi_{\theta_n} (\hat{s}'_{n,i}, a')$,
   \begin{align*}
G_{n+1, i} := \begin{bmatrix}
- \varphi_{n,i} \varphi_{n,i}^\top
& \varphi_{n,i} (\lambda \varphi'_{n,i} - \varphi_{n,i})^\top
 \\ 
 (\varphi_{n,i} - \lambda \varphi'_{n,i}) \varphi_{n,i}^\top
 & 0 \end{bmatrix} \;,
 \quad \textnormal{and} \quad
 g_{n+1, i} := 
 \begin{bmatrix}
 \hat{r}_{n,i} \varphi_{n,i} \\
  0
 \end{bmatrix}
 \;.
\end{align*}
\STATE Update $\theta_n$, $\varrho_n = [ w_n^\top , \vartheta_n^\top]^\top$, $\Gamma_n$ as follows:
\begin{align}
\theta_{n+1} &= \theta_n + \alpha_n (\vartheta_{n+1}- \theta_n) \;, \\
\varrho_{n+1} 
&= \varrho_n + \beta_n 
\langle \Gamma_{n+1} \rangle^{-1} (G_{n+1} \varrho_n - g_{n+1})
\label{eq:update-vartheta} \;, \\
\Gamma_{n+1} &= \Gamma_n  + \gamma_n (G_{n+1} - \Gamma_n)
 \label{eq:update-w} \;.
\end{align}

%\STATE $\Gamma_{n+1} = \Gamma_n  + \gamma_n (\Gamma_{n} - \hat{G}_n)$
%%\STATE $\Gamma_{n+1} = \langle \hat{G}_{n+1} \rangle^{-1} $
%\STATE $\varrho_{n+1} = \varrho_n  + \beta_n \langle \Gamma_{n+1} \rangle^{-1} (G_{n+1} \varrho_n - \varrho_n)$
%\STATE $\theta_{n+1} = \theta_n  + \alpha_n (\vartheta_n - \theta_n)$ recalling $\varrho_n = [ w_n^\top , \vartheta_n^\top]^\top$

%   \FOR{$i=1$ {\bfseries to} $m-1$}
%   \IF{$x_i > x_{i+1}$}
%   \STATE Swap $x_i$ and $x_{i+1}$
%   \STATE $noChange = false$
%   \ENDIF
%   \ENDFOR
\STATE $n = n+1$.
   \UNTIL{$\theta_n$ converges}
\end{algorithmic}
\end{algorithm*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi









%I’d like to share a note on using (Moore-Penrose) pseudoinverse $A^\dagger$, although it is rough. I found that $||Ax - b||_2$ is minimized at $x = A^\dagger b$. Hence, differently from my initial doubt on the pseudoinverse, it seems best for ZAP Q learning (even with singular $A$) since the role of gain matrix is to regularize fluctuation. In addition, I also found that empirically, pseudoinverse outperforms over using identity matrix when $\hat{A}$ is not invertible.

{\note In summary: the main idea of \alg is in twofolds: stability from separating between control and temporal learnings,
and agility from using gain matrix in temporal learning.
}


$Q$-evaluation problem (without function approximation)
finds the true action-value function, which is the fixed point of Bellman operator in \eqref{eq:bellman-operator}.
This naturally induces $Q$-approximation problem (with function approximation)
that finds a fixed point $\theta^*$ of the projected Bellman operator,
such that $Q_{\theta^*} = \bold{T} \bold{B}^\pi Q_{\theta^*}$.
To find the fixed point, we consider the minimization of mean square projected Bellman error (MSPBE)
\cite{sutton2009fast,antos2008learning,liu2015finite}
\begin{align} 
\mathcal{E}(\theta, \theta') &:=  \| Q_\theta - \bold{T} \bold{B}^{\pi_{\theta'}} Q_\theta \|^2_{\mu} \;, \label{eq:MSPBE-sutton}
\end{align}
which is minimized at $\theta^*$.
 $Q$-approximation problem can be formulated in another form \cite{sutton1988TD,mnih2013playing,melo2007q,melo2008analysis}
to find fixed point of Bellman operator instead of {\it projected} Bellman operator,
or equivalently, to minimize mean square Bellman error (MSBE), defined as $\| Q_\theta -  \bold{B}^\pi Q_\theta \|^2_{\mathcal{H}}$, instead of 
MSPBE $\mathcal{E}(\theta)$.
However, since the Bellman operator can move $Q_\theta \in \mathcal{Q}$ to outside of $\mathcal{Q}$,
the fixed point of Bellman operator might not exist and MSBE might have unstable minimizers.
Thus, this formulation leads to unstable algorithms.
In fact, 
the convergence analysis of such algorithms \cite{melo2007q,melo2008analysis} require a strong assumption for the existence and stability of equilibrium, and \citet{baird1995residual} provide the counterexamples in which algorithm corresponding to MSBE diverges, whereas the one corresponding to MSPBE converges \cite{sutton2009fast}.



%stores
%At the $n$-th iteration, it selects a random subset of size $B$ from
%
%
%transition uniformly at random
%among the last $W$ recent transitions, where $(\hat{s}_n, \hat{a}_n, \hat{r}_n, \hat{s}'_n)$ is drawn from window $W_n$
%= $\{({s}_{n+k}, {a}_{n+k}, {r}_{n+k}, {s}_{n+k+1}) : 0 \le k < W \}$ uniformly at random. In particular, when $W = 1$, it is identical to the {\it trajectory sampling}
%which uses transitions in the order observed, i.e.,
%$\hat{s}_n = s_n$, $\hat{a}_n = a_n$, $\hat{r}_n = r_n$, $\hat{s}'_n = s_{n+1}$.
%%which uses transitions in the observed order, i.e.,
%%$\hat{s}_n = s_n$, $\hat{a}_n = a_n$, $\hat{r}_n = r_n$, $\hat{s}'_n = s_{n+1}$.



 experience-replay
iterative algorithms, of which iteration takes a {\it minibatch} of few samples drawn from a large dataset,
have been widely adopted, e.g., \cite{melo2007q,melo2008analysis,sutton2009convergent,sutton2009fast,mnih2013playing},
since such a minibatch approach with small batch size $B$ secures the scalability with respect to size of dataset.

There have been proposed various concepts of best approximation to design algorithms.

algorithms to address off-policy learning with linear function approximation.

definitions of the best approximation to design


objectives evaluating approximation and defining best approximation, e.g.,
mean squared projected Bellman error

evaluations of approximation.
Denote by $\mathcal{Q}$ the set of all the possible approximation, i.e.,
$\mathcal{Q} := \{ Q_\theta : \theta \in \mathbb{R}^d \}$.






\subsection{Sampling Scheme and Iterative Update}

To address $Q$-approximation problem,
iterative algorithms, of which iteration takes a {\it minibatch} of few samples drawn from a large dataset,
have been widely adopted, e.g., \cite{melo2007q,melo2008analysis,sutton2009convergent,sutton2009fast,mnih2013playing},
since such a minibatch approach with small batch size $B$ secures the scalability with respect to size of dataset.




%The sampling mechanism is of our particular interest.
%We first fix\footnote{We could extend our results to various iterative update rules.} iterative update rule of $\theta_n$,  called gradient temporal difference (GTD/GTD2) \cite{sutton2009fast}, 
%which uses single sample $(\hat{s}_n, \hat{a}_n, \hat{r}_n, \hat{s}'_n)$ at $n$-th update of parameters,
%where we observe transition from $\hat{s}_n$ to $\hat{s}'_n$ by selecting action $\hat{a}_n$, and receive reward $\hat{r}_n$:
%\begin{align}  
%\theta_{n+1} 
%&= \theta_n + \alpha_n  (\phi_n - \lambda \phi'_n)
%\phi^\top_n w_n
%\label{eq:update-theta} \;, \\
%w_{n+1} &=w_n + \alpha_n (\delta_n(\theta_n) - \phi^\top_n w_n)
%\phi_k 
% \label{eq:update-w} \;.
%\end{align}
%Here $\{\alpha_n\}$  and $\{\beta_n\}$ are sequences of step sizes, and we define, 
%for all $\theta \in \mathbb{R}^d$,
%\begin{align*}
%\delta_{n}(\theta) &:= \hat{r}_n + \lambda \theta^\top \phi'_n - \theta^\top \phi_n \nonumber \;, \\
%\phi_n &:= \Phi (\hat{s}_n, \hat{a}_n) \;, \\ %\quad \text{and} \quad 
%\phi'_n &:= \sum_{a \in \mathcal{A}} \pi(a \mid \hat{s}'_{n}) \Phi(\hat{s}'_n, a) \;. %\label{eq:sutton-phi-phi'}
%\end{align*}
%We note that this update rule corresponds to the stochastic gradient method of minimizing $\mathcal{E}(\theta)$,
%where 
% the auxiliary parameter $w_k$ is necessary to make the corresponding estimation of $\nabla_\theta \mathcal{E}(\theta)$ unbiased, c.f., see Section~4 of \cite{sutton2009fast} for more discussion.


The random sampling is popularly assumed in convergence analysis, e.g., \cite{sutton2009fast, sutton2009convergent}, since it breaks the correlation between two successive updates.
However, it requires the mighty ability to simulate the MDP,
which is often intractable in practice.
Hence, experience replay is often used as an approximation of the random sampling in practice
and provides a meaningful success, e.g., \cite{mnih2013playing}.
Despite the practical success of experience replay,
its theoretical understanding is shallow.
Only a special case of experience replay, i.e., $W=1$ or 
the trajectory sampling, is analyzed in 
\cite{melo2007q,melo2008analysis}, where
the convergence additionally requires fast mixing of the underlying Markov chain,
which might not be observed in practice.
%Hence, ER sampling is used as an approximation of the random sampling in practice,
%and its success with properly chosen window size $m$, e.g., \cite{mnih2013playing},
%provides experimental evidence that it helps the convergence by breaking or weakening the correlation between successive updates.
In the next section, we provide the convergence analysis with experience replay,
where the convergence is guaranteed either with properly chosen window size $W$
or canonical assumption on step size $\{\alpha_k\}, \{\beta_k\}$ even when the underlying Markov chain is not mixed at all, i.e., periodic chain.
%where ER sampling indeed resolves some convergence issue if the window size is sufficiently large.


%where $\pi(s, a)$ is the probability that target policy $\pi$ selects $a$ at state $s$.
%Then, the temporal-difference error \cite{sutton1988TD} is defined as

 
}

\clearpage


==> proof.tex <==
% !TEX root =  main.tex

\section{Proof of Proposition~\ref{prop:translation}}

Consider 
an optimal deterministic policy $f \in \Pi^*(\phi)$.
It is well known that
the optimal policy $f$ has the constant average reward $g^f_\phi(x) = g^*_\phi$ for all $x \in \set{S}$ in the communicating MDP \cite{puterman1994markov}.
Furthermore, it is also well known that assuming finite state space and finite reward, i.e., $|\set{S}| < \infty$ and $|R_{\max}| < \infty$,
we can always find a bias function $h^f_\phi$ of policy $f$ which has a finite span,
i.e., $\max_{x,y \in \set{S}} h^f_\phi(x)- h^f_\phi (y) < \infty$ for all $x \in \set{S}$ and verifies
\begin{align}
g^f_\phi + h^f_\phi (x) = 
(\mathbf{B}^*_\phi h^f_{\phi})(x)
=
\max_{a \in \set{A}} \left\{
r_\phi(x,a) + \sum_{y \in \set{S}} p_\phi (y \mid x,a) h^f_\phi(y)  \right\}  \;.   \label{eq:bel-opt-recall}
\end{align}


%it is well known, c.f., Theorem~A.7 in \cite{puterman1994markov}, that
%as $n \to \infty$,
%\begin{align*}
%V^*_n(x ; \phi) = n \cdot g^*_\phi +h^*_\phi(x) +  O(1) 
%\end{align*}
%since $g^*_\phi(x) = g^*_\phi$ for each initial state $x$.

Pick a policy $\pi \in \Pi$ and
define
\begin{align*}
D^\pi_n (x_0; f, \phi) := n \cdot g^*_\phi +h^f_\phi(x_0) - V^\pi_n (x_0; \phi) \;,
\end{align*}
which allow us to write the regret of policy $\pi$ as 
\begin{align*}
R^\pi_n(x_0) &= n \cdot g^*_\phi - V^\pi_n (x_0; \phi) \\
&=    D^\pi_n (x_0; \phi)  - h^f_\phi(x_0)\;,
\end{align*}

We then rewrite $V^\pi_n (x_0; \phi)$ as follows:
\begin{align*}
V^\pi_n (x_0; \phi) =
\EXP^\pi_{\phi \mid x_0} \left[ \EXP_{A_0}\left[ \EXP_{X_1} \left[
 r_\phi (x_0, A_0) +V^\pi_{n-1} (X_1 ; \phi)
 \right]  \right] \right]\;,
\end{align*}
where the expectations $\EXP_{A_0}$ and $\EXP_{X_1}$ are taken with
respect to $A_0$ and $X_1$, respectively, under model $\phi$ and
policy $\pi$ given $X_0 = x_0$.
Then, we obtain
\begin{align*}
& D^\pi_n (x_0;f, \phi) \\
&= n \cdot g^*_\phi +h^f_\phi(x_0) - 
\EXP^\pi_{\phi \mid x_0} \left[ \EXP_{A_0}\left[ \EXP_{X_1} \left[
 r_\phi (x_0, A_0) +V^\pi_{n-1} (X_1 ; \phi)
 \right]  \right] \right] \\
&= 
 g^*_\phi +h^f_\phi(x_0)
- \EXP^\pi_{\phi \mid x_0} \left[ \EXP_{A_0}\left[ 
 r_\phi (x_0, A_0) \right] \right] +
\EXP^\pi_{\phi \mid x_0} \Big[ 
\EXP_{A_0}\Big[
 \EXP_{X_1} \Big[
 \underbrace{
(n-1) \cdot g^*_\phi - V^\pi_{n-1} (X_1 ; \phi)
}_{= D^\pi_{n-1}(X_1 ;f, \phi) - h^f_\phi(X_1) }
 \Big]  \Big]
 \Big] \\
&= g^*_\phi +h^f_\phi(x_0)
- \EXP^\pi_{\phi \mid x_0} \left[ \EXP_{A_0}\left[ 
 r_\phi (x_0, A_0) +  \sum_{y \in \set{S}} p_{\phi}(y \mid x_0, A_0) h^f_\phi(y) \right] \right] +
\EXP^\pi_{\phi \mid x_0} \Big[ 
D^\pi_{n-1}(X_1 ;f, \phi) \Big] \\
&= 
\EXP^\pi_{\phi \mid x_0} \left[ \delta^*(x_0, A_0 ;f, \phi) \right] +
\EXP^\pi_{\phi \mid x_0} \Big[ 
D^\pi_{n-1}(X_1 ;f, \phi) \Big] \;,
\end{align*}
where for the last equality, we use
\eqref{eq:bel-opt-recall} and rewrite
\begin{align*}
\delta^*(x, a ; f, \phi ) 
&:=  (\mathbf{B}^*_\phi h^f_\phi) (x) - (\mathbf{B}^a_\phi h^f_\phi) (x)  \\ 
& = g^*_\phi +h^f_\phi (x) -
\left(
r_\phi (x, a)  + \sum_{y \in \set{S}} p_\phi (y  \mid x, a) h^f_\phi (y) 
\right) \;.
\end{align*}
Noting $V^\pi_0 (x;\phi) = 0$ and $D^\pi_0 (x; \phi) = h^*_\phi(x)$,
it follows that
\begin{align*}
D^\pi_n (x_0; f, \phi) 
&= 
\EXP^\pi_{\phi \mid x_0} [ h^*_\phi(X_n)]+
\sum_{k=0}^{n-1} \EXP^\pi_{\phi \mid x_0} \left[ \delta^*(X_k, A_k ; f, \phi) \right] \\
&= 
\EXP^\pi_{\phi \mid x_0} [ h^*_\phi(X_n)]+
\sum_{x \in \set{S}}  \sum_{a \in \set{A}}
 \EXP^\pi_{\phi \mid x_0}[T_n(x,a)] \cdot \delta^*(x, a ;f, \phi)\;,
\end{align*}
which completes the proof of Proposition~\ref{prop:translation}
recalling $\max_{x,y \in \set{S}} h^f_{\phi}(x) - h^f_{\phi}(y) = O(1)$ as $n \to \infty$
and $R^\pi_n(x_0) = D^\pi_n (x_0; \phi)  - h^f_\phi(x_0)$.


\iffalse
$f \in \Pi^*(\phi)$, i.e., $\forall x \in \set{S}$, $f(x) \in \set{O}(x; \phi)$.


\begin{align*}
g^{f}_\phi + h^f_\phi (x) =  r_\phi(x,f(x)) +\sum_{y \in \set{S}} p_\phi (y \mid x,f(x)) h^f_\phi (y) \;.  
\end{align*}

There exists $(x', a')$ such that $a' \notin \set{O}(x ; \phi)$ and
$a' \in \set{O}(x ;h^f_\phi, \phi)$.
\begin{align*}
g^{f}_\phi + h^f_\phi (x') 
&=  r_\phi(x',f(x')) +\sum_{y \in \set{S}} p_\phi (y \mid x',f(x')) h^f_\phi (y)  \\ 
 &< r_\psi(x', a') +\sum_{y \in \set{S}} p_\psi (y \mid x',a') h^f_\phi (y) \;.
\end{align*}

Let
\begin{align*}
 \delta := r_\psi(x', a') +\sum_{y \in \set{S}} p_\psi (y \mid x',a') h^f_\phi (y) -  (g^{f}_\phi + h^f_\phi (x')) >0 
\end{align*}
Let
\begin{align*}
f'(x) = 
\begin{cases}
a' & \text{if $x = x'$}\\
f(x) & \text{otherwise}
\end{cases}\;.
\end{align*}

We want to obtain $g^{f'}_\psi (x)$ and $h^{f'}_\psi (x)$.
\begin{align*}
g^{f'}_\psi (x) 
&= r_\psi(x,f'(x)) + \sum_{y \in \set{S}} p_{\psi}(y \mid x, f'(x)) g^{f'}_\psi (y)  \\
%&=  r_\psi(x,f'(x)) + 
%p_{\psi}(x' \mid x, f'(x)) g^{f'}_\psi (y) 
%+  
%\sum_{y \in \set{S}: y \neq x'} p_{\psi}(y \mid x, f'(x)) g^{f'}_\psi (y)  \\
\end{align*}

\begin{align*}
g^{f'}_\psi (x) 
&= r_\psi(x,f'(x)) + \sum_{y \in \set{S}} p_{\psi}(y \mid x, f'(x)) g^{f'}_\psi (y)  \\
%&=  r_\psi(x,f'(x)) + 
%p_{\psi}(x' \mid x, f'(x)) g^{f'}_\psi (y) 
%+  
%\sum_{y \in \set{S}: y \neq x'} p_{\psi}(y \mid x, f'(x)) g^{f'}_\psi (y)  \\
\end{align*}

\fi


\section{Proof of Theorem~\ref{thm:g-r-lower}} \label{sec:g-r-lower}

We start with the decomposition of $\Delta_{\Phi} (\phi)$
into $\Delta_{\Phi} (x,a; \phi)$.
\begin{lemma}
Consider irreducible model $\phi$
and a perturbed model $\psi$ such that
$\kl_{\phi \mid \psi}(x,a) = 0$ for all $(x,a)$ such that $a\in \set{O}(x;\phi)$.
\begin{align*}
\Pi^*(\phi) \cap \Pi^*(\psi) = \emptyset
\iff \exists (x,a) \in \set{S} \times \set{A} ~\text{such that}~ a \in
\set{O}(x; h^*_\phi, \psi)  \setminus 
 \set{O}(x; h^*_\phi, \phi) \;.
\end{align*}
\end{lemma}
\begin{proof}
Since in the irreducible model $\phi$, the entire space of states becomes the recurrent set under any policy, i.e., there is no transient states,
it is well known, c.f., \cite{ross1983}, %\cite{puterman1994markov}
that the optimal average reward $g^*_\phi$ is a constant, and
a bias function of an optimal deterministic policy $f \in \Pi^*(\phi)$ can be that of another optimal deterministic policy $f' \in \Pi^*(\phi)$.
Therefore, we can express
\begin{align*}
\Pi^*(\phi) 
&:= \{f \in \Pi_{\TN{D}}: g^f_\phi = g^*_\phi \} \\
&= \{f \in \Pi_{\TN{D}}: f(x) \in \set{O}(x; h^*_\phi, \phi) = \set{O}(x; \phi)\} \;,
\end{align*}
where $h^*_\phi$ is a bias function of an optimal deterministic policy  
$f \in \Pi^*(\phi)$  which is arbitrarily chosen.

In addition, we note that an optimal policy $f \in \Pi^*(\phi)$ will
behaves the same under $\phi$ and $\psi$ since
$\kl_{\phi \mid \psi}(x,a) = 0$ for all $(x,a)$ such that $a\in \set{O}(x;\phi)$.
Hence, the optimal policy $f$ has the same average reward $g^f_\phi$
and bias function $h^f_\phi$ in perturbed $\psi$, i.e.,
for all $f \in \Pi^*(\phi)$, 
\begin{align} \label{eq:}
g^*_\phi = g^f_\phi =  g^f_\psi \;, \quad \text{and} \quad
h^*_\phi  = h^f_\phi =  h^f_\psi \;.
\end{align} 

($\implies$)  
We prove by contradiction. Suppose that for all $x \in \set{S}$,
$\set{O}(x; h^*_\phi, \psi) \setminus \set{O}(x; h^*_\phi, \phi) = \emptyset$, i.e.,
$\set{O}(x; h^*_\phi, \psi) \subset \set{O}(x; h^*_\phi, \phi)$.
Recalling 





($\impliedby$)


We first suppose 
that there exists $(x,a)$ such that $a \notin \set{O}(x; h^*_\phi, \phi)$ and $a \in \set{O}(x; h^*_\phi, \psi)$.
Then, $h^*_\phi$


$\Pi^*(\phi) \cap \Pi^*(\psi) = \emptyset$
\end{proof}


\begin{lemma}
Consider irreducible $\phi$ so that the optimal bias function $h^*_\phi$ is unique up to constant.
For $x \in \set{S}$, function $h: \set{S} \to \mathbb{R}$ and model $\psi$,
define 
\begin{align*}
\set{O}(x;  h, \psi) = 
\left\{a \in \set{A}: 
r_\psi (x, a)+ \sum_{y\in \set{S}}  p_\psi (y \mid x,a) h(y)
\ge 
r_\psi (x, b)+ \sum_{y\in \set{S}}  p_\psi (y \mid x,b) h(y)
~\forall b \in \set{A}
\right\}\;.
\end{align*}
Then,
\begin{align*}
\Pi^*(\phi) &= \{f \in \Pi_D : f(x) \in \set{O}(x;h^*_\phi, \phi)\} 
\;, \quad \text{and} \\
\Delta_{\Phi} (\phi) 
&= \bigcup_{(x,a): x \in \set{S}, a \notin \set{O}(x;h^*_\phi, \phi) }
\Delta_{\Phi} (x,a; \phi) \;,
\end{align*}
where $\Delta_{\Phi} (x,a; \phi)
:= 
\{\psi \in \Phi : 
\kl_{\phi \mid \psi}(x',a') = 0~  \forall(x',a') \text{ such that } a' \in \set{O}(x';\phi),
\text{and }
a \in \set{O}(x; h^*_\phi, \psi)\}$.
\end{lemma}




Using a standard change-of-measure argument
 from $\phi$ to $\psi \in \Delta_\Phi(\phi)$,
 we obtain a characterization of behavior of uniformly good algorithms as follows:
\begin{theorem} \label{thm:uniform-lbd} 
Consider an irreducible model $\phi$.  Then,  for any policy $\pi \in \Pi_{\textnormal{UG}}$, and $x_0 \in \set{S}$ and 
any perturbed model $\psi \in \Delta_{\Phi}(\phi)$,
we have
\begin{align} \label{eq:regret-basic-bound}
\liminf_{n \to \infty } \sum_{(x,a) \in \set{S} \times \set{A}: a \notin \set{O}(x;\phi)} \frac{\EXP^\pi_{\phi \mid x_0} [T_n (x, a)]}{\log n } \cdot    \kl_{\phi \mid \psi}(x, a) \ge 1 \;.
\end{align}
%and a state $x \in \set{S}$ such that
%$x \in \set{S}_{O(\phi)}$, i.e., $ $If under $\phi$,
\end{theorem}

We stress that Theorem~2 in \cite{burnetas1997optimal} considers 
only a specific form of unrelated structure where the reward and 
the set of feasible transitions are known in advance.
Hence, the analysis in \cite{burnetas1997optimal} is limited to
the case when 
both $\phi$ and $\psi$ are irreducible and
the perturbation is only at transition kernel of a pair of state and action. 
However, we relax such limitations in the analysis of Theorem~\ref{thm:uniform-lbd}. 



The above theorem with $\psi \in \Delta_{\Phi}(\phi)$ provides
a corresponding necessary condition on $[{\EXP^\pi_{\phi \mid x_0} [T_n (x, a)]}/{\log n }]_{(x,a)}$ for any uniformly good $\pi \in \Pi_{\TN{UG}}$.
Hence, combining Proposition~\ref{prop:translation}
and Lemma~\ref{lem:uniform-lbd}, we directly obtain
the lower bound of regret of uniformly good algorithms 
as the form of the minimization \eqref{eq:g-r-opt}.





The conditions on the perturbed model $\psi$ ensures that
there exists $x \in \set{S}$ such that for all $\alpha  >0$,
\begin{align*}
\EXP^\pi_{\psi \mid x_0}
\left[ \sum_{a \in \set{O}(x ; \phi)} T_n (x, a)\right] = o(n^\alpha) \;.
\end{align*}



$(x', a') \in \set{S} \times \set{A}$ such that 
$a' \notin \set{O}(x' ;\phi)$ and
$a' \in \set{O}(x';h^*_\phi, \psi)$, i.e.,
for all $a \in \set{O}(x' ;\phi)$,
\begin{align*}
r_{\psi}(x', a)  + \sum_{y \in \set{S}} p_{\psi}(y \mid  x', a) h^*_\phi (y)
& = r_{\phi}(x', a)  + \sum_{y \in \set{S}} p_{\phi}(y \mid  x', a) h^*_\phi (y)\\
&< 
r_{\psi}(x', a')  + \sum_{y \in \set{S}} p_{\psi}(y \mid  x', a') h^*_\phi (y) \;.
\end{align*}
Otherwise, any $f \in \Pi^*(\phi)$ of which 
$g^f_\phi$ and $h^f_\phi$ verify the Bellman optimal equation 
\eqref{eq:undis-BO} with respect to perturbed model $\psi$, i.e.,
$\Pi^*(\phi) \cap \Pi^*(\psi) \neq \emptyset$,
since $f(x) \in \set{O}(x; \phi)$ for all $x \in \set{S}$
and policy $f$ has the same Markov process of $X_k$'s  under
$\phi$ and $\psi$.








\begin{align*}
\EXP^\pi_{\phi \mid x_0}
 \left[
 \sum_{x \in \set{X}} \sum_{a \in \set{O}(x; \phi)} T_n(x,a)
 \right] <n -  \sqrt{n}
\end{align*}
not happen since if so, regret is $\Omega(\sqrt{n})$

\begin{align*}
\EXP^\pi_{\psi \mid x_0}
 \left[
 \sum_{x \in \set{X}} \sum_{a \in \set{O}(x; \phi)} T_n(x,a)
 \right] < n - \sqrt{n}
\end{align*}
happen since 

\section{Proof of Lemma~\ref{lem:uniform-lbd}}\label{sec:pf-uniform-lbd} 

We use the change-of-measure argument from $\phi$ to $\psi$ such that
$\Pi^*(\phi) \cap \Pi^*(\psi) = \emptyset$ and $\kl_{\phi  \mid \psi } (x,a) = 0$
if 
Assumption~\ref{asm:irreduce} ensures the uniqueness (up to additive constant) of the optimal bias function $h^*_\phi$, i.e.,
for all optimal policies $f, f' \in \Pi^*(\phi)$ and $x, y \in \set{S}$,
$h^{f}_\phi (x) - h^{f}_\phi (y) = h^{f'}_\phi (x) - h^{f'}_\phi (y)$.
Hence, $\set{O} (x ; h^*_\phi, \phi)$ is well-defined.
From $\Pi^*(\phi) \cap \Pi^*(\psi) = \emptyset$,
it follows that there must exist $(x,a) \in \set{S} \times \set{A}$ such that
$a \notin \set{O}(x; \phi)$ but $a \in \set{O} (x; h^*_\phi, \phi)$.
If not, 

\begin{lemma}{Lemma~1, \cite{kaufmann2016complexity}} \label{lem:change-of-measure}
  Consider two models $\phi$ and $\psi$ such that kernel of $\phi$ is
  absolutely continuous with respect to that of $\psi$, i.e.,
  for all $x,y \in \set{S}$, $a \in \set{A}$,
  $r \in \set{R}$, $p_\phi(y\mid x,a) =0$ if 
  $p_{\psi}(y \mid x,a) = 0$, and $q_\phi(r\mid x,a) =0$ if 
   $q_{\psi}(r \mid x,a) = 0$. For any almost-surely finite stopping
  time $\tau$ with respect to $\set{H}_k$, any policy $\pi \in \Pi$, and any $x_0 \in \set{S}$
\begin{align*}
\sum_{(x,a) \in \set{S} \times \set{A}} 
\EXP^\pi_{\phi \mid x_0} [T_\tau(x,a)] \cdot \kl_{\phi \mid \psi}(x,a) \ge
\sup_{\set{E} \in \sigma(\set{H}_\tau)} d(\Pr^\pi_{\phi \mid x_0}[ \set{E}], \Pr^\pi_{\psi \mid x_0}[ \set{E}]) \;,
\end{align*}
where $T_n (x,a) : = \sum_{k=0}^{n}\mathbbm{1}[X_k = x, A_k = a]$ is the
number of occurrences of pair $(x,a)$,
$\kl_{\phi \mid \psi}(x,a) $
is the KL divergence between kernels of $\phi$ and $\psi$ at $(x,a)$
which we define as:
\begin{align*}
\kl_{\phi \mid \psi}(x,a) 
:= \left(\sum_{y\in \set{S}} p_\phi(y \mid x,a)  \log \frac{p_\phi(y \mid x,a) }{p_\psi(y \mid x,a) }  \right)
+
\left(
\int_{r \in \set{R}} q_\phi(r \mid x,a) \log \frac{q_\phi(r \mid x,a)}{q_\psi(r \mid x,a) }dr 
\right) \;.
\end{align*}
Here, $d(u,v ) := u\log \frac{u}{v} + (1-u) \log \frac{1-u}{1-v}$, with
the convention that $d(0,0) = d(1,1) = 0$.
\end{lemma}

Let $\set{E} = \{ \sum_{x \in \set{S}} \sum_{a \in \set{O}(x ; \phi) } \}$ be the event that the total number of selecting suboptimal actions
exceeds a sublinear function of time spent.


\section{Proof of Lemma~\ref{lem:change-of-measure}}
\label{sec:pf-change-of-measure}


\section{Proof of Theorem~\ref{thm:lip}} \label{sec:pf-lip}
To upper bound the minimal $K_{\Phi}(\phi)$, we construct a feasible $\eta =[\eta(x,a)]_{x \in \set{S}, a \in \set{A}}$ verifying \eqref{eq:g-r-set} given $\Phi$ of \ref{item:lip}. Then, we will obtain an upper bound of objective value of the constructed $\eta$.

As a part of constructing $\eta$, we find sequences of 
sets $[\set{X}_i]_{i =1,2, \ldots, I+1}$ and pairs $[(x_i, a_i)]_{i =1,2, \ldots, I}$
such that
$X_{I+1} = \emptyset$, and
 for each $i \le I$, $\set{X}_i \supset X_{i+1}$ and
$(x_i, a_i) = \argmax_{(x,a) \in \set{X}_i} \delta^* (x,a; \phi)$.
\note{The choice of $(x_i, a_i)$ can be arbitrary if $(x_i,a_i) \in \set{X}_i$.
But I think this specific choice of $(x_i, a_i)$ will provide better practical performance of algorithm based on this construction of $\eta$...}
We begin with $\set{X}_1 = \{(x,a) : x\in \set{S}, a \notin \set{O}(x; \phi), i.e., \delta^*(x, a;\phi) > 0 \}$.
Recursively, for each $i =1, 2, ...$, let 
\begin{align}
\set{B}_i &= \left\{(x,a) \in \set{X}_i :  L (\ell(x,x_i))^\alpha +L' (\ell(a, a_i))^{\alpha'}  \le \frac{1}{2} \cdot \frac{\delta_{\min}}{R_{\max} + H_{\max}} \right\} \;, \quad \text{and} \nonumber \\
\set{X}_{i+1} &= \set{X}_i \setminus \set{B}_i  \;. \label{eq:X-i}
\end{align}
Let $I$ be the last index with non-empty $\set{X}_i$, i.e., $\set{X}_I \neq \emptyset$ and $\set{X}_{I+1} = \emptyset$.
Construct $\eta$ as
\begin{align} \label{eq:eta-construct}
\eta (x,a) = 
\begin{cases}
8 \cdot \left( \frac{\delta_{\min}}{R_{\max} + H_{\max}} \right)^{-2} &\text{if $\exists i \in [1, I]$ such that $(x,a) = (x_i, a_i)$}\\
0 &\text{Otherwise}
\end{cases} \;. 
\end{align}
Then, noting that $\eta$ has strictly positive values at $I$-many points $(x_i, a_i)$'s,
\begin{align*}
\sum_{(x,a) \in \set{S} \times \set{A}}\delta^*(x,a ; \phi) \eta(x,a)  \le 
8 \cdot \frac{R_{\max} + H_{\max}}{\delta^2_{\min}} \cdot I
\end{align*}
since $\delta^*(x,a; \phi) \le R_{\max} + H_{\max}$ for all $(x,a)$.
We bound the length of sequence $\set{X}_i$'s using covering and packing numbers of
the hypercubes $[0, D]^d$ and $[0, D']^{d'}$, in which the states and actions are located, respectively.
\begin{lemma} \label{lem:I-bound}
The generation of $\set{X}_i$'s in \eqref{eq:X-i} 
must stop in $(S_{\textnormal{lip}} \cdot A_{\textnormal{lip}}+1)$ iterations, i.e., $I \le S_{\textnormal{lip}} \cdot A_{\textnormal{lip}}$.
\end{lemma}
We provide the proof of Lemma~\ref{lem:I-bound} in Section~\ref{sec:pf-I-bound}.
Therefore, it suffices to show that $\eta$ verifies all the constraints with the structure $\Phi$ in \ref{item:lip}.

To check the feasibility $\eta$, we first divide the constraints as follows:
\begin{lemma}
Consider irreducible $\phi$ so that the optimal bias function $h^*_\phi$ is unique up to constant.
For $x \in \set{S}$, function $h: \set{S} \to \mathbb{R}$ and model $\psi$,
define 
\begin{align*}
\set{O}(x;  h, \psi) = 
\left\{a \in \set{A}: 
r_\psi (x, a)+ \sum_{y\in \set{S}}  p_\psi (y \mid x,a) h(y)
\ge 
r_\psi (x, b)+ \sum_{y\in \set{S}}  p_\psi (y \mid x,b) h(y)
~\forall b \in \set{A}
\right\}\;.
\end{align*}
Then,
\begin{align*}
\Pi^*(\phi) &= \{f \in \Pi_F : f(x) \in \set{O}(x;h^*_\phi, \phi)\} 
\;, \quad \text{and} \\
\Delta_{\Phi} (\phi) 
&= \bigcup_{(x,a): x \in \set{S}, a \notin \set{O}(x;h^*_\phi, \phi) }
\Delta_{\Phi} (x,a; \phi) \;,
\end{align*}
where $\Delta_{\Phi} (x,a; \phi)
:= 
\{\psi \in \Phi : 
\kl_{\phi \mid \psi}(x',a') = 0~  \forall(x',a') \text{ such that } a' \in \set{O}(x';\phi),
\text{and }
a \in \set{O}(x; h^*_\phi, \psi)\}$.
\end{lemma}


Fix $(x,a) \in \set{S}  \times \set{A}$ such that $a \notin \set{O}(x;h^*_\phi, \phi)$,
and pick $\psi  \in \Delta_\Phi(x, a ; \phi)$.
Let $i \in \{1, \ldots, I\}$ denote the index such that $(x,a) \in \set{B}_i$.
Note that there must exist such an index $i$ since 
$(x,a) \in \set{X}_1$ and $\set{X}_{I+1} = \emptyset$.
To complete the proof, it is sufficient to check
if $\eta$ verifies the constraint corresponding to $\psi$:
\begin{align} \label{eq:feasibility-psi}
\sum_{(x',a') \in \set{S} \times \set{A}} \eta(x', a') \kl_{\phi \mid \psi}(x',a') \ge 1\;.
\end{align}
From the construction of $\eta$ in \eqref{eq:eta-construct},
it follows that
\begin{align*}
\sum_{(x',a') \in \set{S} \times \set{A}} \eta(x', a') \kl_{\phi \mid \psi}(x',a') 
&\ge  \eta(x_i, a_i) \cdot \kl_{\phi \mid \psi}(x_i,a_i) \\
& =
8 \cdot
\left( \frac{\delta_{\min}}{R_{\max}+H_{\max}} \right)^{-2}
 \cdot \kl_{\phi \mid \psi}(x_i,a_i) \\
 & \ge
4 \cdot
\left( \frac{\delta_{\min}}{R_{\max}+H_{\max}} \right)^{-2}
 \cdot \left(\tv (\phi(x_i,a_i), \psi(x_i, a_i)) \right)^2 \;,
\end{align*}
where we use Pinsker’s inequality for the last inequality,
and we denote the total variation between two kernels $\phi(x, a)$ and $\psi(x', a')$ by
\begin{align*}
\tv (\phi(x,a), \psi(x', a')) := \sum_{y \in \set{S}} |p_\phi(y \mid x, a) - p_\psi(y \mid x', a')| 
+ \int_{r \in \set{R}} |q_\phi(r \mid x, a) - q_\psi(r \mid x', a')| \;.
\end{align*}
Hence, for \eqref{eq:feasibility-psi}, we will show
\begin{align*}
\tv (\phi(x_i,a_i), \psi(x_i, a_i)) \ge 
\frac{1}{2} \cdot \frac{\delta_{\min}}{R_{\max}+H_{\max}}\;.
\end{align*}


Recalling $\psi  \in \Delta_\Phi(x, a ; \phi)$, i.e.,
$a \in \set{O}(x; h^*_\phi, \psi)$,
we have
\begin{align}
r_{\psi}(x, a) + \sum_{y \in \set{S}} p_\psi (y \mid x,a) h^*_{\phi}(y)
& \ge
\max_{b \in \set{A}}
r_{\phi}(x, b) + \sum_{y \in \set{S}} p_\phi (y \mid x,b) h^*_{\phi}(y) \nonumber \\
&\ge
r_{\phi}(x, a) + \sum_{y \in \set{S}} p_\phi (y \mid x,a) h^*_{\phi}(y)
+ \delta_{\min} \label{eq:minimum-perturbation}
\end{align}
where the last inequality follows from the definition of $\delta_{\min}$ and
the choice of $a \notin \set{O}(x;h^*_\phi, \phi)$.
Note that by adding some constant to $h^*_\phi$,
we can always make $-H_{\max} \le h^*_\phi(x) \le H_{\max}$.
Thus, with \eqref{eq:minimum-perturbation}, this leads
\begin{align*}
\delta_{\min}
&\le
\int^{R_{\max}}_{-R_{\max}}
\left(q_{\psi}(r \mid x, a) - q_{\phi}(r \mid x, a) \right) dr
  + \sum_{y \in \set{S}} \left(p_\psi (y \mid x,a) - p_\phi (y \mid x,a) \right) h^*_{\phi}(y) \\
&  \le
{R_{\max}} \cdot \int
\left|q_{\psi}(r \mid x, a) - q_{\phi}(r \mid x, a) \right| dr
  + H_{\max} \cdot \sum_{y \in \set{S}} \left|p_\psi (y \mid x,a) - p_\phi (y \mid x,a) \right|  \\
  &\le (R_{\max} + H_{\max}) \cdot \tv (\phi(x,a), \psi(x, a))\;,
\end{align*}
which implies 
\begin{align} \label{eq:minimum-TV}
\tv (\phi(x,a), \psi(x, a)) \ge \frac{\delta_{\min}}{R_{\max} + H_{\max}} \;.
\end{align}
In addition, from the triangular inequalities, it follows that
\begin{align}
\tv (\phi(x,a), \psi(x, a)) 
&\le
\tv (\phi(x,a), \phi(x_i, a_i)) 
+ \tv (\phi(x_i,a_i), \psi(x_i, a_i)) 
+ \tv (\psi(x_i,a_i), \psi(x, a))  \nonumber \\
&\le
\tv (\phi(x_i,a_i), \psi(x_i, a_i)) 
+ 2L (\ell (x, x_i)^\alpha)
+ 2L' (\ell (a, a_i)^{\alpha'})  \label{eq:use-lip}
\end{align}
where the last inequality follows from
Lipschitz continuity in \ref{item:lip}.
Combining \eqref{eq:minimum-TV} and \eqref{eq:use-lip}, 
we have
\begin{align}
\tv (\phi(x_i,a_i), \psi(x_i, a_i)) 
&\ge 
 \frac{\delta_{\min}}{R_{\max} + H_{\max}} 
- 2L (\ell (x, x_i)^\alpha)
- 2L' (\ell (a, a_i)^{\alpha'}) \nonumber \\
& \ge
\frac{1}{2} \cdot \frac{\delta_{\min}}{R_{\max} + H_{\max}}  \label{eq:tv-bound}\;,
\end{align}
which verifies the feasibility of $\eta$ for $\psi$ in \eqref{eq:feasibility-psi}.
This completes the proof of Theorem~\ref{thm:lip} due to
the arbitrary choice of $(x,a)$ and $\psi$.






\section{Proof of Lemma~\ref{lem:I-bound}}
\label{sec:pf-I-bound}

%We first introduce some useful notions: covering number and packing number.
A $\delta$-{\em packing} of  a set $\set{D}$ with respect to a metric $\rho$ 
is a set $\{x_1, ..., x_n\} \subset \set{D}$ such that 
$\rho(x_i- x_j)  > \delta$ for all different $i, j \in \{1, ..., n\}$.
The {\em $\delta$-packing number} $I_{\textnormal{p}}(\delta, \set{D}, \rho)$ 
is the cardinality of the largest $\delta$-packing.
The construction of $\set{X}_i$ ensures that for different $i, j \in \{1, ..., I\}$,
\begin{align*}
\ell_{\TN{lip}}((x_i, a_i), (x_j, a_j) )
 %L (\ell(x_i, x_j))^\alpha +L' (\ell(a_i, a_j))^{\alpha'}  
> \delta := \frac{1}{2} \cdot \frac{\delta_{\min}}{R_{\max} + H_{\max}}\;,
\end{align*}
where 
for $(x,a), (x',a') \in \mathbb{R}^d \times \mathbb{R}^{d'}$, 
\begin{align*}
\ell_{\TN{lip}}((x, a), (x', a') ) :=  L (\ell(x, x'))^\alpha +L' (\ell(a, a'))^{\alpha'}   \;.
\end{align*}
Then, using the definition of packing  number, we have
\begin{align*}
I \le I_{\TN{p}} \left(\delta,
\set{S} \times \set{A},
 %[0, D]^d \times[0, D']^{d'},
  \ell_{\TN{lip}} \right )\;.
\end{align*}
To obtain an upper bound of the packing number, we define
the covering number.
A $\delta$-cover of a set $\set{D}$ with respect to a metric $\rho$ 
is a set $\{x_1, ..., x_I\} \subset \set{D}$ such that for each $x \in \set{D}$,
there exists some $i \in \{1, ..., I\}$ such that $\rho(x, x_i) \le \delta$.
The $\delta$-covering number $I_{\TN{c}}(\delta, \set{D}, \rho)$ is 
the smallest cardinality of $\delta$-cover. Then, we have the following relation
between packing and covering numbers.
\begin{lemma} \label{lem:cover-pack}
 For all $\delta >0$, $\set{D}, \set{D}'$ such that $\set{D} \subset \set{D}'$, 
 \begin{align*}
 I_{\TN{p}}(2 \delta, \set{D}, \rho) \le I_{\TN{c}}(\delta, \set{D}, \rho)
\le I_{\TN{c}}(\delta, \set{D}', \rho) \;.
\end{align*}
\end{lemma}
The proof of Lemma~\ref{lem:cover-pack} in Section~\ref{sec:cover-pack}.
Define metrics $\ell^{(1)}_{\max}, \ell^{(2)}_{\max}, \ell_{\max}$ for $\mathbb{R}^{d}, \mathbb{R}^{d'}, \mathbb{R}^{d} \times \mathbb{R}^{d'}$, respectively, as follows:
\begin{align*}
\ell^{(1)}_{\max}(x, x')
&:= \left( \frac{1}{\sqrt{d}} \left(\frac{\delta}{2L}\right)^{1/\alpha}  \right)^{-1} \| x - x' \|_{\infty}
\;, \\
\ell^{(2)}_{\max}(a, a') 
&:= \left( \frac{1}{\sqrt{d'}} \left(\frac{\delta}{2L'}\right)^{1/\alpha'}  \right)^{-1} \| a - a' \|_{\infty} 
\;, \\%\quad \text{and} \\
\ell_{\max}((x,a), (x',a')) 
&:= \max \left\{  \ell^{(1)}_{\max}(x, x'),  \ell^{(2)}_{\max}(a, a') \right\} \;,
\end{align*}
where $\|\cdot\|_\infty$ is infinite norm.
Then, it follows that
for any $(x,a), (x',a')\in \mathbb{R}^d \times \mathbb{R}^{d'}$, 
\begin{align*}
\ell_{\max}((x,a), (x',a')) \le 1 \implies
\ell_{\TN{lip}}((x,a), (x',a')) \le  \delta \;.
\end{align*}
Hence, we have
 \begin{align*}
 I &\le I_{\TN{c}} (\delta, \set{S} \times \set{A}, \ell_{\TN{lip}})  \\
 &\le I_{\TN{c}} (1, \set{S} \times \set{A}, \ell_{\max})  \\ 
  &\le I_{\TN{c}} (1, \set{S}, \ell^{(1)}_{\max})  \cdot
  I_{\TN{c}} (1, \set{A}, \ell^{(2)}_{\max}) 
\end{align*}
since 
for any $1$-cover $\set{S}'$
of $\set{S}$ with metric $\ell^{(1)}_{\max}$ 
and 
any $1$-cover $\set{A}'$ of $\set{A}$ 
with metric $\ell^{(2)}_{\max}$,
their Cartesian product $\set{S}' \times \set{A}' = \{(x,a) : x \in \set{S}', a \in \set{A}' \}$
is $1$-cover of $\set{S} \times \set{A}$ with metric $\ell_{\max}$.
We now study $I_{\TN{c}} (1, \set{S}, \ell^{(1)}_{\max})$ and $I_{\TN{c}} (1, \set{A}, \ell^{(2)}_{\max})$.
Recalling $\set{S} \subset [0,D]^d$ and using Lemma~\ref{lem:cover-pack}, it directly follows that
\begin{align*}
I_{\TN{c}} (1, \set{S}, \ell^{(1)}_{\max}) &\le
I_{\TN{c}} (1, [0, D]^d, \ell^{(1)}_{\max}) \\
& = I_{\TN{c}} \left( \frac{1}{\sqrt{d}} \left( \frac{\delta}{2L} \right)^{1/\alpha}, [0, D]^d, \|\cdot \|_{\max} \right)  \\
&\le \left( \frac{D}{\frac{1}{\sqrt{d}} \left( \frac{\delta}{2L} \right)^{1/\alpha}} +1 \right)^d\;,
\end{align*}
which implies
\begin{align*}
I_{\TN{c}} (1, \set{S}, \ell^{(1)}_{\max}) 
&\le  
\min \left\{|\set{S}|, 
\left( \frac{D}{\frac{1}{\sqrt{d}} \left( \frac{\delta}{2L} \right)^{1/\alpha}} +1 \right)^d
\right\}  = S_{\TN{lip}}
\end{align*}
where for the first inequality, we use the fact that $I_{\TN{c}} (1, \set{S}, \ell^{(1)}_{\max}) \le |\set{S}|$.
Similarly, we have
\begin{align*}
I_{\TN{c}} (1, \set{A}, \ell^{(2)}_{\max}) 
&\le  
\min \left\{|\set{A}|, 
\left( \frac{D'}{\frac{1}{\sqrt{d'}} \left( \frac{\delta}{2L'} \right)^{1/\alpha'}} +1 \right)^{d'}
\right\}  = A_{\TN{lip}}\;.
\end{align*}
This completes the proof of Lemma~\ref{lem:I-bound}.



\section{Proof of Lemma~\ref{lem:cover-pack}}
\label{sec:cover-pack}

Consider a $\delta$-cover $\set{X}$ and a $2\delta$-pack $\set{Y}$
of set $\set{D}$ with respect to metric $\rho$.
Then, there is no $x \in \set{X}$ such that
$y, y' \in \set{B}(\delta, x) = \{x' \in \set{D}: \rho(x, x') \le \delta \}$
for two different $y, y' \in \set{Y}$.
Otherwise, we have
$\rho(x, y) \le \delta$ and
$\rho(x, y') \le \delta$ which
imply $\rho(y, y') \le 2\delta$ from the triangle inequality,
contradict to the fact that $y, y'$ are two different elements of $2\delta$-cover, i.e.,
$\rho(y, y') > 2\delta$. 
Thus, it is not possible that the cardinality of $\set{Y}$ is larger than
that of $\set{X}$. Due to the arbitrary choice of 
$\delta$-cover $\set{X}$ and a $2\delta$-pack $\set{Y}$,
we conclude $I_{\TN{p}}(2 \delta, \set{D}, \rho) \le I_{\TN{c}}(\delta, \set{D}, \rho)$.

Since a $\delta$-cover $\set{X}$ of 
of set $\set{D'}$ is also
a $\delta$-cover of the smaller set $\set{D}$,
it straightforwardly follows that $I_{\TN{c}}(\delta, \set{D}, \rho)
\le I_{\TN{c}}(\delta, \set{D}', \rho)$. This completes the proof of Lemma~\ref{lem:cover-pack}.







\section{Proof of Theorem~\ref{thm:}}

\section{Proof of Theorem~\ref{thm:}}
\section{Proof of Theorem~\ref{thm:}}
\section{Proof of Theorem~\ref{thm:}}


\section{Proof of Lemma~\ref{lem:gen-decom}} \label{sec:pf-gen-decom}
  We will prove the contraposition of Lemma~\ref{lem:gen-decom}. Assume
  $\Pi^*(\phi) \cap \Pi^*(\psi') \neq \emptyset$ and
  $\Pi^*(\phi) \cap \Pi^*(\psi'') \neq \emptyset$. 
  Let $\Pi^*(\phi, \psi', \psi'') :=  \Pi^*(\phi) \cap \Pi^*(\psi') \cap \Pi^*(\psi'')$.
It suffices to show  
\begin{align}
(i)~ \Pi^*(\phi, \psi', \psi'') \neq \emptyset  \;, \quad \text{and} \quad
(ii)~ \Pi^*(\phi, \psi', \psi'') \subseteq \Pi^*(\psi)  \;,
\label{eq:decom-wts}
\end{align}
which imply $\Pi^*(\phi) \cap \Pi^*(\psi) \neq \emptyset$.
An important observation for this proof is that a policy $f \in \Pi^*(\phi)$
has the same average reward and bias vectors in any of $\psi, \psi', \psi''$
since the suboptimality of $\set{S}'$ and $\set{S}''$ in $\phi$ implies $(x, f(x)) \notin \set{S}' \cup \set{S}''$, and the kernels of $\psi, \psi', \psi''$ are identical
at every $(x,a) \notin \set{S}' \cup \set{S}''$. More formally,
for policy $f \in \Pi^*(\phi)$,
\begin{align} \label{eq:identical}
g^f_\psi =  g^f_{\psi'} = g^f_{\psi''}   \quad \text{and} \quad 
h^f_\psi =  h^f_{\psi'} = h^f_{\psi''}  \;.
\end{align}



To prove the first part of \eqref{eq:decom-wts}, 
consider policy $f' \in \Pi^*(\phi) \cap \Pi^*(\psi')$ and policy $f'' \in \Pi^*(\phi) \cap \Pi^*(\psi'')$.
Then, from the optimality of $f'$ under $\psi'$, it follows that 
for each $x \in \set{S}$,
\begin{align} \label{eq:one-side-ineq}
g^*_{\psi'}(x) = g^{f'}_{\psi'}(x) \ge g^{f''}_{\psi'}(x) = g^{f''}_{\psi''} (x)= g^{*}_{\psi''} (x)\;, 
\end{align}
where for the second equality, we use \eqref{eq:identical}.
Similarly, it follows that for each $x \in \set{S}$,
\begin{align*}
g^*_{\psi''}(x) = g^{f''}_{\psi''}(x) \ge g^{f'}_{\psi''}(x) = g^{f'}_{\psi'}(x)= g^{*}_{\psi'} (x)\;.
\end{align*}
which implies $g^*_{\psi'} = g^*_{\psi''}$ together with  \eqref{eq:one-side-ineq}.
Therefore, this concludes $\Pi^*(\phi, \psi', \psi'') = \Pi^*(\phi) \cap \Pi^*(\psi') = \Pi^*(\phi) \cap \Pi^*(\psi'') \neq \emptyset$.


We now prove the second part of \eqref{eq:decom-wts}.
%To do so, we construct model $\phi'$ with 
%\begin{align*}
%p_{\phi'}(\cdot \mid x,a) = 
%\begin{cases}
%p(\cdot \mid x, a) & \text{if $(x, a) \in \set{S}^*$} \\
%p_\phi(\cdot \mid x, a) & \text{otherwise}
%\end{cases} \;,  \quad \text{and} \quad
%q_{\phi'}(\cdot \mid x,a) = 
%\begin{cases}
%q(\cdot \mid x, a) & \text{if $(x, a) \in \set{S}^*$} \\
%q_\phi(\cdot \mid x, a) & \text{otherwise}
%\end{cases} \;.
%\end{align*}
Pick a policy $f \in \Pi^*(\phi, \psi', \psi'')$ and state $x \in \set{S}$.
%Then, similarly to \eqref{eq:identical}, it is straightforward to show that 
%\begin{align*}
%h^f_{\psi'} = h^f_{\psi''} = h^f_{\psi} \;.
%\end{align*}
Thus,
it is sufficient to show $g^f_\psi(x)$ and $h^f_\psi(x)$ verify the Bellman optimality equation \eqref{eq:undis-BO} for model $\psi$. % since the choice of $x$ is arbitrary.
Using \eqref{eq:identical} and the optimality of $f$ under $\psi'$,
it follows that for all $a\in \set{A}$, if $(x,a) \notin \set{S}''$, then
\begin{align} 
r_{\psi} (x, f(x)) + \sum_{y \in \set{S}} p_{\psi}(y \mid x, f(x)) h^f_{\psi} (y) 
 & \overset{(a)}{=} r_{\psi'} (x, f(x)) + \sum_{y \in \set{S}} p_{\psi'}(y \mid x, f(x)) h^f_{\psi'} (y) \nonumber \\
&\overset{(b)}{\ge}
r_{\psi'} (x, a) + \sum_{y \in \set{S}} p_{\psi'}(y \mid x, a) h^f_{\psi'} (y) \nonumber \\
& \overset{(c)}{=} r_{\psi} (x, a) + \sum_{y \in \set{S}} p_{\psi}(y \mid x, a) h^f_{\psi} (y) \;,
\label{eq:BO-S'}
\end{align} 
where for (a) and (c), we use \eqref{eq:identical} and the fact that the kernels of $\psi$ and $\psi'$
are the same at every $(x,a) \notin \set{S}''$,
and for (b), we use $g^f_{\psi'}$ and $h^f_{\psi'}$ verify the Bellman optimality equation \eqref{eq:undis-BO} for model $\psi'$.
Similarly, using the optimality of $f$ under $\psi''$, it follows that 
for $(x,a) \in \set{S}''$, 
\begin{align} 
r_{\psi} (x, f(x)) + \sum_{y \in \set{S}} p_{\psi}(y \mid x, f(x)) h^f_{\psi} (y) 
 & = r_{\psi''} (x, f(x)) + \sum_{y \in \set{S}} p_{\psi''}(y \mid x, f(x)) h^f_{\psi''} (y) \nonumber \\
& \ge
r_{\psi''} (x, a) + \sum_{y \in \set{S}} p_{\psi''}(y \mid x, a) h^f_{\psi''} (y) \nonumber  \\
& = r_{\psi} (x, a) + \sum_{y \in \set{S}} p_{\psi}(y \mid x, a) h^f_{\psi} (y) \;. \label{eq:BO-S''}
\end{align} 
Combining \eqref{eq:BO-S'} and \eqref{eq:BO-S''}, for all $(x,a) \in \set{S} \times \set{A}$,
\begin{align*} 
r_{\psi} (x, f(x)) + \sum_{y \in \set{S}} p_{\psi}(y \mid x, f(x)) h^f_{\psi} (y) 
&\ge
r_{\psi} (x, a) + \sum_{y \in \set{S}} p_{\psi}(y \mid x, a) h^f_{\psi} (y) \;,
\end{align*} 
which implies $(\mathbf{B}^f_\psi h^f_\psi) = (\mathbf{B}^*_\psi h^*_\psi)$ and thus
$g^f_\psi$ and $h^f_\psi$ verify the Bellman optimality equation \eqref{eq:undis-BO} under model $\psi$. This completes the proof of the second part of \eqref{eq:decom-wts} and thus
concludes Lemma~\ref{lem:gen-decom}.



\section{Proof of Lemma~\ref{lem:dis-gen-decom}} \label{sec:pf-dis-gen-decom}
The proof of Lemma~\ref{lem:dis-gen-decom} is analog to that of Lemma~\ref{lem:gen-decom}.
We will prove the contraposition of Lemma~\ref{lem:dis-gen-decom}. Assume
  $\Pi^*_\gamma(\phi) \cap \Pi^*_\gamma(\psi') \neq \emptyset$ and
  $\Pi^*_\gamma(\phi) \cap \Pi^*_\gamma(\psi'') \neq \emptyset$. 
  Let $\Pi^*_\gamma(\phi, \psi', \psi'') :=  \Pi^*_\gamma(\phi) \cap \Pi^*_\gamma(\psi') \cap \Pi^*_\gamma(\psi'')$.
It suffices to show  
\begin{align}
(i)~ \Pi^*_\gamma(\phi, \psi', \psi'') \neq \emptyset  \;, \quad \text{and} \quad
(ii)~ \Pi^*_\gamma(\phi, \psi', \psi'') \subseteq \Pi^*_\gamma(\psi)  \;,
\label{eq:dis-decom-wts}
\end{align}
which imply $\Pi^*_\gamma(\phi) \cap \Pi^*_\gamma(\psi) \neq \emptyset$.
An important observation for this proof is that a policy $f \in \Pi^*_\gamma(\phi)$
has the same value function in any of $\psi, \psi', \psi''$
since the $\gamma$-suboptimality of $\set{S}'$ and $\set{S}''$ in $\phi$ implies $(x, f(x)) \notin \set{S}' \cup \set{S}''$, and the kernels of $\psi, \psi', \psi''$ are identical
at every $(x,a) \notin \set{S}' \cup \set{S}''$. More formally,
for policy $f \in \Pi^*_\gamma(\phi)$,
\begin{align} \label{eq:dis-identical}
V^f_\psi =  V^f_{\psi'} = V^f_{\psi''} \;.
\end{align}



To prove the first part of \eqref{eq:dis-decom-wts}, 
consider policy $f' \in \Pi^*_\gamma(\phi) \cap \Pi^*_\gamma(\psi')$ and policy $f'' \in \Pi^*_\gamma(\phi) \cap \Pi^*_\gamma(\psi'')$.
Then, from the $\gamma$-optimality of $f'$ under $\psi'$, it follows that 
for each $x \in \set{S}$,
\begin{align} \label{eq:dis-one-side-ineq}
V^*_{\psi'}(x) = V^{f'}_{\psi'}(x) \ge V^{f''}_{\psi'}(x) = V^{f''}_{\psi''} (x)= V^{*}_{\psi''} (x)\;, 
\end{align}
where for the second equality, we use \eqref{eq:dis-identical}.
Similarly, it follows that for each $x \in \set{S}$,
\begin{align*}
V^*_{\psi''}(x) = V^{f''}_{\psi''}(x) \ge V^{f'}_{\psi''}(x) = V^{f'}_{\psi'}(x)= V^{*}_{\psi'} (x)\;.
\end{align*}
which implies $V^*_{\psi'} = V^*_{\psi''}$ together with  \eqref{eq:dis-one-side-ineq}.
Therefore, this concludes $\Pi^*_\gamma (\phi, \psi', \psi'') = \Pi^*_\gamma (\phi) \cap \Pi^*_\gamma (\psi') = \Pi^*_\gamma (\phi) \cap \Pi^*_\gamma (\psi'') \neq \emptyset$.


We now prove the second part of \eqref{eq:dis-decom-wts}.
%To do so, we construct model $\phi'$ with 
%\begin{align*}
%p_{\phi'}(\cdot \mid x,a) = 
%\begin{cases}
%p(\cdot \mid x, a) & \text{if $(x, a) \in \set{S}^*$} \\
%p_\phi(\cdot \mid x, a) & \text{otherwise}
%\end{cases} \;,  \quad \text{and} \quad
%q_{\phi'}(\cdot \mid x,a) = 
%\begin{cases}
%q(\cdot \mid x, a) & \text{if $(x, a) \in \set{S}^*$} \\
%q_\phi(\cdot \mid x, a) & \text{otherwise}
%\end{cases} \;.
%\end{align*}
Pick a policy $f \in \Pi^*_\gamma(\phi, \psi', \psi'')$ and state $x \in \set{S}$.
%Then, similarly to \eqref{eq:identical}, it is straightforward to show that 
%\begin{align*}
%h^f_{\psi'} = h^f_{\psi''} = h^f_{\psi} \;.
%\end{align*}
Thus,
it is sufficient to show the value function $V^f_\psi$ of policy $f$ under $\psi$ verifies the Bellman optimality equation \eqref{eq:dis-BO} of model $\psi$. % since the choice of $x$ is arbitrary.
Using \eqref{eq:identical} and the $\gamma$-optimality of $f$ under $\psi'$,
it follows that for all $a\in \set{A}$, if $(x,a) \notin \set{S}''$, then
\begin{align} 
r_{\psi} (x, f(x)) + \gamma \sum_{y \in \set{S}} p_{\psi}(y \mid x, f(x)) V^f_{\psi} (y) 
 & \overset{(a)}{=} r_{\psi'} (x, f(x)) + \gamma \sum_{y \in \set{S}} p_{\psi'}(y \mid x, f(x)) V^f_{\psi'} (y) \nonumber \\
&\overset{(b)}{\ge}
r_{\psi'} (x, a) + \gamma \sum_{y \in \set{S}} p_{\psi'}(y \mid x, a) V^f_{\psi'} (y) \nonumber \\
& \overset{(c)}{=} r_{\psi} (x, a) + \gamma \sum_{y \in \set{S}} p_{\psi}(y \mid x, a) V^f_{\psi} (y) \;,
\label{eq:dis-BO-S'}
\end{align} 
where for (a) and (c), we use \eqref{eq:dis-identical} and the fact that the kernels of $\psi$ and $\psi'$
are the same at every $(x,a) \notin \set{S}''$,
and for (b), we use the fact that $V^f_{\psi'}$ verifies the $\gamma$-Bellman optimality equation \eqref{eq:dis-BO} for model $\psi'$.
Similarly, using the $\gamma$-optimality of $f$ under $\psi''$, it follows that 
for $(x,a) \in \set{S}''$, 
\begin{align} 
r_{\psi} (x, f(x)) + \gamma \sum_{y \in \set{S}} p_{\psi}(y \mid x, f(x)) V^f_{\psi} (y) 
 & = r_{\psi''} (x, f(x)) + \gamma \sum_{y \in \set{S}} p_{\psi''}(y \mid x, f(x)) V^f_{\psi''} (y) \nonumber \\
& \ge
r_{\psi''} (x, a) +\gamma \sum_{y \in \set{S}} p_{\psi''}(y \mid x, a) V^f_{\psi''} (y) \nonumber  \\
& = r_{\psi} (x, a) + \gamma \sum_{y \in \set{S}} p_{\psi}(y \mid x, a) V^f_{\psi} (y) \;. \label{eq:dis-BO-S''}
\end{align} 
Combining \eqref{eq:dis-BO-S'} and \eqref{eq:dis-BO-S''}, for all $(x,a) \in \set{S} \times \set{A}$,
\begin{align*} 
r_{\psi} (x, f(x)) + \gamma \sum_{y \in \set{S}} p_{\psi}(y \mid x, f(x)) V^f_{\psi} (y) 
&\ge
r_{\psi} (x, a) +\gamma \sum_{y \in \set{S}} p_{\psi}(y \mid x, a) V^f_{\psi} (y) \;,
\end{align*} 
which implies $(\mathbf{B}^f_{\psi, \gamma} V^f_\psi) = (\mathbf{B}^*_{\psi, \gamma} h^*_\psi)$ and thus
$V^f_\psi$ verifies the $\gamma$-Bellman optimality equation \eqref{eq:dis-BO} under model $\psi$. This completes the proof of the second part of \eqref{eq:dis-decom-wts} and thus
concludes Lemma~\ref{lem:dis-gen-decom}.









%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "./main"
%%% End: 


==> prooflemS7.tex <==
% !TEX root =  appendix.tex


\subsection{Proof of Lemma~\ref{lem:bound-3}}
\label{sec:pf-bound-3}



%Intuitively, we show that by the design of the algorithm, the restricted bias function $h'_t$ is monotonically improved so that it eventually converges to the optimal bias function $h^*_\phi$ with high probability. In this analysis, we provide a more sophisticated concentration inequality than the one in \cite{burnetas1997optimal}. This concentration inequality is particularly important to bound the regret generated by the exploitation phase. 

Recall that:
\begin{align*}
\set{E}_t(\varepsilon) :=
\left\{ 
\Pi^*(\phi'_t) \subseteq \Pi^*(\phi)
~\text{and}~
|r_t(x,a) - r_{\phi}(x,a) | + |h'_t (x) - h^*_\phi(x)| \le \varepsilon 
~\forall x \in \set{S}, \forall a \in \set{O}(x;\phi'_t)
\right\} .
\end{align*}

Hence when $\set{E}_t(\varepsilon)$ occurs, ($i$) the estimation of the bias function in the restricted MDP $\phi(\set{C}_t)$ is accurate and ($ii$) the restricted MDP includes the optimal policies of $\phi$. We first focus on the accuracy of the estimated bias function, and then show that the gain of the restricted MDP $\phi(\set{C}_t)$ is monotone increasing and that it eventually includes an optimal policy for the (unrestricted) MDP. 

{\bf Estimation error in bias function. } 
We begin with some useful notations.
Let $K:= A^S$ be the number of all the possible fixed policies.
Fix $\beta \in \left(0, \frac{1}{K + 1}\right)$. 
For sufficiently large $t > \frac{1}{\frac{1}{K +1} - \beta}$,
divide the time interval from $1$ to $t$
into $(K+1)$ subintervals $\set{I}^t_0, \set{I}^t_1, \dots, \set{I}^t_{K}$
such that $\set{I}^t_k := \{u \in \mathbb{N} : i^t_k \le u < i^t_{k+1} \}$
where $i^t_0 :=1$ and $i^t_k := t +1- (K +1- k) \lfloor \frac{t}{K+1}\rfloor$
for $k \in \{1, ...,  K+1\}$.
%Then, We first provide some useful properties of the interval division.
Then, it is easy to check that for each $k \in \{0, ..., K\}$, 
\begin{align*}
|\set{I}^t_k| = i^t_{k+1} - i^t_k > \beta t .
\end{align*}
Indeed, for $k = 0$, $i^t_1 - i^t_0 = t - K \lfloor \frac{t}{K+1} \rfloor \ge \frac{t}{K+1} > \beta t$,
and for $k \in [1, K]$, $i^t_{k+1} - i^t_k =  \lfloor \frac{t}{K+1} \rfloor
 \ge \frac{t}{K+1} > \beta t$ as $t > \frac{1}{\frac{1}{K +1} - \beta}$, i.e., 
each subinterval length grows linearly with respect to $t$.
%In addition, for $k \ge 1$, $\frac{i^t_{k+1}}{i^t_k} < \frac{1}{k\beta} \le \frac{1}{\beta}$


For $k \in [0, K]$, $x \in \set{S}$ and $a \in \set{A}$,
let $M^t_k (x) := N_{i^t_{k+1}} (x) -  N_{i^t_{k}} (x) $
and $M^t_k (x, a) := N_{i^t_{k+1}} (x, a) -  N_{i^t_{k}} (x, a)$.
%For
% $x \in \set{S}$, $a \in \set{A}$,
% and $u, v > 0$ such that $u \le v$,
%let $N_{u,v}(x) := N_{v}(x) - N_{u}(x)$
% and
% $N_{u,v}(x, a) := N_{v}(x, a) - N_{u}(x, a)$. 
Using $\rho > 0$ in \eqref{eq:erg}, for $\zeta > 0$, define an event $\set{D}_t (\zeta)$ as
\begin{align} \label{eq:define-D_t}
\set{D}_t (\zeta) := \set{D}'_t \cap \set{E}'_t(\zeta)
\end{align}
where we let
\begin{align*}
\set{D}'_t &:= 
\left\{
M^t_{k}(x) > \rho \beta t, 
\forall x \in \set{S}, \forall k \in [0, K]
\right\}  \\
\set{E}'_t (\zeta) &:= 
\left\{
\| \phi'_u - \phi(\set{C}_u) \| \le  \zeta, 
\forall u \in [i^t_1, t]
\right\} .
\end{align*}
When $\set{D}_t(\zeta)$ occurs, then in each subinterval, each state is linearly visited,
and after the first subinterval, the estimation on the restricted MDP is accurate, i.e., $\phi(\set{C}_t) \simeq \phi_t(\set{C}_t)$.
Note that $\set{E}_t(\varepsilon)$ bounds the error in the estimated gain and bias functions.
Hence, we establishy the correspondence between $\zeta$ in $\set{D}_t(\zeta)$ and $\varepsilon$ in $\set{E}_t(\varepsilon)$
using the continuity of the gain and bias functions in $\phi$:  
\begin{lemma}  \label{lem:translate-eps-to-zeta}
Consider an ergodic MDP $\phi$ with Bernoulli rewards.
Then, for $\varepsilon >0$.
there exists $\zeta_0 = \zeta_0(\varepsilon, \phi) >0 $ such that
for any $\zeta \in (0, \zeta_0)$, policy $f \in \Pi_D$ and MDP $\psi$,
if $\|\psi - \phi \| \le \zeta$ and $\psi \ll \phi$, then $\psi$ is ergodic, $|g^f_\psi - g^f_\phi | \le \varepsilon$  and $\|h^f_\psi - h^f_\phi \| \le \varepsilon$.
\end{lemma}
The proof of Lemma~\ref{lem:translate-eps-to-zeta} is in Section~\ref{sec:pf-translate-eps-to-zeta}.  
Observe that on the event $\set{D}_t (\zeta)$, for $u \ge i^t_1$, every state is visited more than
$\rho\beta t$, i.e., $\log^2 N_u (x) \ge \log^2 \rho \beta t \ge 1$ for all $x\in \set{S}$ and sufficiently large $t$, and thus, for all $(x,a) \in \set{S} \times \set{A}$ such that $a \in \set{C}_u(x)$,
 $\phi_u(x,a)$ is indeed the estimation of $\phi(x,a)$, i.e., $\phi'_u = \phi_u(\set{C}_u) \ll \phi(\set{C}_u)$.
 %From now on, we consider sufficiently small $\zeta \le \zeta_0(\varepsilon, \phi)$
%where $\zeta_0(\varepsilon, \phi)$ is from Lemma~\ref{lem:translate-eps-to-zeta}.
Then, using Lemma~\ref{lem:translate-eps-to-zeta},
it follows that there exists constant $t_0>0$ such that for $t > t_0$
and $\zeta \in(0, \min\{\zeta_0(\varepsilon/2, \phi), \varepsilon / 2\})$, 
\begin{align}
\set{D}_t(\zeta) \subseteq 
 \{
\text{$\phi'_u$ is ergodic}~\forall u \in [i^t_1, t]
\}
\cap
\set{E}''_t (\varepsilon)  \label{eq:on-D-connect}
\end{align}
where 
\begin{align*}
\set{E}''_t (\varepsilon) := 
\left\{
| r_{\phi'_u}(x, f(x)) - r_{\phi} (x, f(x)) |
+
| h^f_{\phi'_u}(x)- h^f_{\phi}(x) | \le  \varepsilon
~\forall u \in [i^t_1, t], \forall f \in  \Pi_{D}(\set{C}_u),
\forall x \in \set{S}
\right\},
\end{align*}
and where for restriction $\set{C} : \set{S} \twoheadrightarrow \set{A}$,
we denote by $\Pi_{D} (\set{C})$ the set of all the possible deterministic policies on the restricted MDP $\phi(\set{C})$.



{\bf Monotone improvement. } 
Based on \eqref{eq:on-D-connect}, we can identify instrumental properties of DEL algorithm when $\set{D}_t(\zeta)$ occurs:
\begin{lemma} \label{lem:D-implies}
For structure $\Phi$ with Bernoulli rewards and an ergodic MDP $\phi \in \Phi$,
consider $\pi = \textnormal{DEL}$.
There exists $\zeta_1 > 0$ and $t_1 > 0$ such that
for any $\zeta \in (0, \zeta_1)$ and $t > t_1$,
the occurrence of the event $\set{D}_t(\zeta)$ implies that 
\begin{align}
\Pi^*(\phi'_u)  \subseteq \Pi^*(\phi(\set{C}_u)),
 \quad \text{and}\quad
g^*_{u+1}  \ge g^*_{u}, \quad
\forall u \in [i^t_1, t]
\label{eq:D-implies}
\end{align}
where we denote by $g^*_{u} := g^*_{\phi(\set{C}_u)}$ 
and $h^*_{u} := h^*_{\phi(\set{C}_u)}$  the optimal gain and bias functions, respectively,
on the restricted MDP $\phi(\set{C}_u)$ with true parameter $\phi$.
%where we consider the gain function $g^*_{\phi(\set{C}_u)}$ as a real number
%due to the ergodicity of in \eqref{eq:on-D-connect}.
\end{lemma}
The proof of Lemma~\ref{lem:D-implies} is presented in Section~\ref{sec:pf-D-implies}. 

Define the event
\begin{align*}
\set{M}_t := \left\{g^*_{i^t_{k+1}} > g^*_{i^t_{k}}~\forall k \in [1, K]
 ~\text{or}~
g^*_{i^t_{k+1}} = g^*_{i^t_{k}} = g^*_\phi~\text{for some $k\in [1, K]$}
\right\}.
\end{align*}
Then, by selecting $\zeta$ as in in Lemma~\ref{lem:D-implies} and \eqref{eq:on-D-connect},
we can connect the events $\set{M}_t $ and $ \set{D}_t (\zeta)$ to the event $\set{E}_t(\varepsilon)$
as follows: for $\zeta \in (0, \min\{\zeta_0(\varepsilon/2, \phi), \varepsilon/2, \zeta_1\})$ and sufficiently large $t > t_1$,
\begin{align}  \label{eq:MD-implies-E}
\set{M}_t \cap \set{D}_t (\zeta) \subseteq \set{E}_t(\varepsilon).
\end{align}
On the event $\set{M}_t$, there must exists $k\in[1, K+1]$ such that $g^*_{i^t_k} = g^*_\phi$
since the number $K$ of subintervals is the number of all the possible policy $\Pi^* $.
In addition, for such a $k\in[1, K+1]$, on the event $\set{D}_t (\zeta)$,
it follows from Lemma~\ref{lem:D-implies} that for all $u \in [ i^t_k, t]$, $g^*_{i^t_k} = g^*_\phi \le g^*_u \le g^*_t$, i.e., $g^*_t =g^*_\phi$ and thus $\Pi^*(\phi(\set{C}_t)) \subseteq \Pi^*(\phi)$.
Therefore, when both of the events $\set{M}_t$ and $\set{D}_t (\zeta)$ occur,
\begin{align*}
\Pi^*(\phi) \supseteq \Pi^*(\phi(\set{C}_t))  \supseteq \Pi^*(\phi'_t) 
\end{align*}
(again thanks to Lemma~\ref{lem:D-implies}).
Then, we indeed get $\set{M}_t \cap \set{D}_t (\zeta) \subseteq \set{E}_t(\varepsilon)$: the ergodicity of $\phi'_t$ guaranteed from  \eqref{eq:on-D-connect} implies 
that the optimal bias function $h'_t$ of $\phi'_t$ is  unique, and the event $\set{E}''_t(\varepsilon)$ in \eqref{eq:on-D-connect}
always occurs on the event $\set{D}_t (\zeta)$. Thus the estimated bias function $h'_t$ is close to $h^*_{\phi}$.


Using \eqref{eq:MD-implies-E} and \eqref{eq:define-D_t}, for small enough
$\zeta \in (0, \min\{\zeta_0(\varepsilon/2, \phi), \varepsilon/2, \zeta_1\})$, we get
\begin{align}
\EXP^\pi_{\phi \mid x_1} \left[W^{(3)}_T(\varepsilon) \right] 
&=
\sum_{t=1}^T \Pr^\pi_{\phi \mid x_1} \left[\neg \set{E}_t(\varepsilon) \right]  \nonumber  \\
&\le O(1) 
+\sum_{t=t_1}^T \Pr^\pi_{\phi \mid x_1} \left[\neg\set{D}_t(\zeta) \right] 
+ \sum_{t=t_1}^T \Pr^\pi_{\phi \mid x_1} \left[\set{D}_t(\zeta), \neg\set{M}_t \right] 
 \nonumber \\
&\le O(1)
+\sum_{t=t_1}^T \Pr^\pi_{\phi \mid x_1} \left[\neg\set{D}'_t \right]  
+\sum_{t=t_1}^T \Pr^\pi_{\phi \mid x_1} \left[\set{D}'_t, \neg\set{E}'_t(\zeta)\right]  
 + \sum_{t=t_1}^T \Pr^\pi_{\phi \mid x_1} \left[\set{D}_t(\zeta), \neg\set{M}_t \right] 
\label{eq:bound-3-final}
\end{align}
where the first and last inequalities are from \eqref{eq:MD-implies-E}
and \eqref{eq:define-D_t}, respectively.
%the additional term $O(1)$ in the first inequality is from the fact that
%the relationship in \eqref{eq:MD-implies-E} holds for sufficiently large $t$,
To complete the proof of Lemma~\ref{lem:bound-3}, we provide upper bounds of each term in the r.h.s. of \eqref{eq:bound-3-final}. the first term can be easily bounded. Indeed, using \eqref{eq:erg} and a union bound, we get for $t$ sufficiently,
\begin{align}
\Pr^\pi_{\phi \mid x_1} [\neg\set{D}'_t] 
\le 
\sum_{x \in \set{S}}
\sum_{k \in [0, K]}
\Pr^\pi_{\phi \mid x_1} [M^t_{k}(x) \le \rho \beta t]  = o(1/t)
\label{eq:bound-3-first-sum}
\end{align}
where the last equality is from \eqref{eq:erg} conditioned on $X_{i^t_k}$ for each $k$.
 
Lemma \ref{lem:difficult-bound-3} below deals with the last term. 

\begin{lemma} \label{lem:difficult-bound-3}
For structure $\Phi$ with Bernoulli rewards and an ergodic MDP $\phi \in \Phi$,
consider $\pi = \textnormal{DEL}$.
Suppose $\phi$ is in the interior of $\Phi$, i.e., 
there exists a constant $\zeta_0 >0$ such that for any $\zeta \in (0, \zeta_0)$,
$\psi \in \Phi$ if $\|\phi - \psi\| \le \zeta$.
There exists $\zeta_2 > 0 $ such that for $\zeta \in (0, \zeta_2)$,
\begin{align*}
\sum_{t=t_1}^T \Pr^\pi_{\phi \mid x_1} \left[\set{D}_t(\zeta), \neg\set{M}_t \right]  = o(\log T)
\quad \text{as $T \to \infty$}.
\end{align*}
\end{lemma}
We provide the proof of Lemma~\ref{lem:difficult-bound-3} in Section~\ref{sec:pf-difficult-bound-3}. There, the assumption that $\phi$ is in the interior of $\Phi$ plays an important role when studying the behavior of the algorithm in the exploitation phase.

To bound the second term in the r.h.s. of \eqref{eq:bound-3-final}, we use the following concentration inequality:
\begin{lemma} \label{lem:concen-exp}
Consider any $\pi$ and $x_1 \in \set{S}$.
There exist $C_0, c_0, u_0 > 0$ such that for any $(x,a) \in \set{S} \times \set{A}$
and $u \ge u_0$,
\begin{align*}
\Pr^\pi_{\phi \mid x_1} [ |\phi_t (x,a) -  \phi (x,a)| >  \zeta, N_t (x,a) = u] \le  C_0 e^{- c_0 u } .
\end{align*}
\end{lemma}
{\bf Proof of Lemma~\ref{lem:concen-exp}. }
The proof is immediate from Lemma~4(i)
in \cite{burnetas1997optimal}, which is an application of Cramer's theorem for estimating Bernoulli random variables. 
Let $\hat{\phi}_t(x,a)$ be the estimator of $\phi(x,a)$ from $t$ i.i.d. reward and transition samples when action $a$ is selected in state $x$. From Lemma~4(i) in \cite{burnetas1997optimal}, there are positive constants $C(x,a)$, $c(x,a)$, and $u_0(x,a)$ (which may depend on $(x,a)$), such that for $u \ge u_0(x,a)$,
\begin{align*}
\Pr^\pi_{\phi \mid x_1} [ |\phi_t (x,a) -  \phi (x,a)| >  \zeta, N_t (x,a) = u] 
& \le \Pr [ |\hat{\phi}_u (x,a) -  \phi (x,a)| >  \zeta]  \\
& \le  C_0(x,a)  e^{- c_0(x,a) u }.
\end{align*}
%where the first inequality is due to i.i.d. realization of $R_t$ and $X_{t+1}$ given $(X_t, A_t) = (x,a)$,
%and the second inequality is from Lemma~4(i) in \cite{burnetas1997optimal}.
We complete the proof by taking $C_0 := \max_{(x,a) \in \set{S} \times \set{A}} C_0(x,a)$,
$c_0 := \min_{(x,a) \in \set{S} \times \set{A}} c_0(x,a)$, and
$u_0 := \max_{(x,a) \in \set{S} \times \set{A}} u_0(x,a)$.
\ep

Now observe that:
\begin{align*} 
&\Pr^\pi_{\phi \mid x_1} [\set{D}'_t, \neg\set{E}'_t(\zeta)] \\
&= \Pr^\pi_{\phi \mid x_1} [\set{D}'_t, 
\| \phi_u(x,a) - \phi(x,a) \| > \zeta, 
\text{for some}~ u \in [ i^t_1,t],  x \in \set{S}, a \in \set{C}_u (x)
]  \\
&\le 
\sum_{u=i^t_1}^t
\sum_{x \in \set{S}}
\sum_{a \in \set{C}_u(x)}
\Pr^\pi_{\phi \mid x_1} [\set{D}'_t, 
\| \phi_u(x,a) - \phi(x,a) \| > \zeta]  \\
&\le
\sum_{u=i^t_1}^t
\sum_{x \in \set{S}}
\sum_{a \in \set{C}_u(x)}
\Pr^\pi_{\phi \mid x_1} [ %\set{D}^{(1)}_T, 
\| \phi_u(x,a) - \phi(x,a) \| > \zeta, N_u(x,a) \ge \log^2 N_u(x), \rho \beta t \le N_u(x) \le u]  \\
&\le
\sum_{u=i^t_1}^t
\sum_{x \in \set{S}}
\sum_{a \in \set{C}_u(x)}
\sum_{u' = \rho \beta t}^u
\sum_{u'' = \log^2 {u'}}^{u'}
\Pr^\pi_{\phi \mid x_1} [
\| \phi_u(x,a) - \phi(x,a) \| > \zeta, N_u(x,a) =  u''] 
\end{align*}
where the second inequality follows from the definition of $\set{C}_u(x)$ and the fact that
on the event $\set{D}'_t$,  $ \rho \beta t \le M_0^t(x) \le N_u(x)$ for $u \in[ i^t_1, t]$.
Then, applying Lemma~\ref{lem:concen-exp}, 
we have
\begin{align} 
\Pr^\pi_{\phi \mid x_1} [\set{D}'_t, \neg\set{E}'_t(\zeta)] 
&\le
\sum_{u=i^t_1}^t
\sum_{x \in \set{S}}
\sum_{a \in \set{C}_u(x)}
\sum_{u' = \rho \beta t}^u
\sum_{u'' = \log^2 u'}^{\infty}
C_0 e^{-c_0 u''} \nonumber \\
&\le SA C_0  t^2 \frac{e^{-c_0 \log^2 (\rho \beta t)}}{1-e^{-c_0}} \nonumber  \\
& = \frac{SA C_0}{{1-e^{-c_0}}}  t^2 e^{-c_0 (\log^2 (\rho \beta) + \log t (\log t+2 \log (\rho \beta)))}
\nonumber  \\
& = 
\frac{SA C_0}{{1-e^{-c_0}}} 
e^{-c_0 \log^2 (\rho \beta) }
 t^{2 -  2c_0  \log (\rho \beta) - c_0 \log t} = o(1/t) . \label{eq:bound-3-second-sum}
\end{align}
Combining Lemma~\ref{lem:difficult-bound-3}, \eqref{eq:bound-3-first-sum}
and \eqref{eq:bound-3-second-sum}
to \eqref{eq:bound-3-final}, we complete the proof of Lemma~\ref{lem:bound-3}.

 

\ep











\subsubsection{Proof of Lemma~\ref{lem:translate-eps-to-zeta}}
\label{sec:pf-translate-eps-to-zeta}

%Define two strictly positive constants:
%\begin{align*}
%\zeta_q (\phi) &:= 
%\min \left\{
%\frac{q_{\phi}(x,a)}{2} : \forall x \in \set{S}, \forall a \in \set{A} \text{ s.t. } q_{\phi}(1 \mid x,a) > 0 
%\right\} 
%\end{align*}

Define the positive constant:
\begin{align*}
 \zeta_p (\phi) &:= 
\min \left\{
\frac{p_{\phi}(y \mid x,a)}{2} : \forall x,y \in \set{S}, \forall a \in \set{A} \text{ s.t. } p_{\phi}(y\mid x,a) > 0  \right\}. 
\end{align*} 
Then, it is straightforward to show that $\psi$ is ergodic if $\|\psi - \phi\| < \zeta_p (\phi)$ since for any $x,y \in \set{S}$ and $a \in \set{A}$,
$p_{\phi}(y \mid x,a) > 0$ implies that $p_{\psi}(y \mid x,a) \ge p_{\phi}(y \mid x,a)/2 > 0$.
Therefore, for $\zeta_0 \le \zeta_p (\phi)\}$, $\psi$ is ergodic.

%Then, it is straightforward to show that $\phi \ll \psi$ if $\|\psi - \phi\| < \min \{\zeta_q (\phi),  \zeta_p (\phi)\}$ since for any $x,y \in \set{S}$ and $a \in \set{A}$,
%$p_{\phi}(y \mid x,a) > 0$ implies that $p_{\psi}(y \mid x,a) \ge p_{\phi}(y \mid x,a)/2 > 0$,
%and
%$q_{\phi}(1 \mid x,a) > 0$ implies that $q_{\psi}(1 \mid x,a) \ge q_{\phi}(1 \mid x,a)/2 > 0$.
%Therefore, for sufficiently small $\zeta_0 \le \min \{\zeta_q (\phi),  \zeta_p (\phi)\}$, 
%the above observation  and the supposition that $\psi \ll \phi$
%provide the mutually absolute continuity between $\phi$ and $\psi$
%and thus the ergodicity of $\psi$.

Now, we focus on the continuity of gain and bias functions for given policy $f$.
For notational convenience, let $g^f_\phi$ (resp. $g^f_\psi$) and 
$h^f_\phi$ (resp. $h^f_\psi$)
denote the (column) vector of gain and bias functions, respectively, under $\phi$ (resp. $\psi$).
Let $P^f_{\phi}$ (resp. $P^f_\psi$) and $r^f_\phi$ (resp. $r^f_\phi)$ are the transition matrix and reward vector w.r.t. policy $f$ under $\phi$ (resp. $\psi$), respectively.
Then, we can write the policy evaluation equations of stationary policy $f$ under $\phi$ and $\psi$ as vector and matrix multiplications, c.f., \cite{puterman1994markov}:
\begin{align*}
g^f_\phi &= P^f_\phi g^f_\phi  \\
h^f_\phi &= r^f_\phi - g^f_\phi + P^f_\phi h^f_\phi. 
\end{align*}
Similarly $g^f_\psi = P^f_\psi g^f_\psi$ and $h^f_\psi = r^f_\psi - g^f_\psi + P^f_\psi h^f_\psi$.
Since both $\phi$ and $\psi$ are ergodic, by forcing $h^f_{\phi} (x_1) = h^f_{\psi} (x_1) = 0$ for some $x_1 \in \set{S}$, the bias functions $h^f_{\phi}$ and $h^f_{\psi}$ can be uniquely defined. 
Let $D^f := P^f_\phi - P^f_\psi$ and $d^f := h^f_\phi - h^f_\psi$.
Then, $\| D^f \| \le |\set{S}| \delta$ where $\|\cdot \|$ is the max norm.
Noting that the ergodicity of $\phi$ and $\psi$ further provides the invertibility of $I - P^f_\phi$ and $I - P^f_\psi$.
A basic linear algebra, c.f., Lemma~7 in \cite{burnetas1997optimal}, leads to that for any $\varepsilon  > 0$, $ \|d^f\| \le \varepsilon$ if
\begin{align*}
\| D^f\| \le \frac{\varepsilon}{\|(I-P^f_\phi)^{-1} \| (\|h^f_\phi \|+ \varepsilon)}
\end{align*}
where the upper bound is independent of $\psi$.
From the above continuity of $h^f_{\psi}$ (and thus that of $g^f_\psi$) 
with respect to $\psi$ at $\phi$, we can find $\zeta_0(f, \varepsilon, \phi) > 0$
such that for any $\psi$, $|g^f_\psi - g^f_\phi| \le \varepsilon$ and
$\|h^f_\psi - h^f_\phi \| \le \varepsilon$ if 
$\|\psi -\phi\| \le \zeta_0(f, \varepsilon,\phi)  \le \min \{\zeta_q(\phi), \zeta_p(\phi)\}$.
Noting the arbitrary choice of $f \in \Pi_D$,
we conclude the proof of Lemma~\ref{lem:translate-eps-to-zeta}
by taking $\zeta_0 (\varepsilon, \phi) = \min_{f \in \Pi_D} \zeta_0(f, \varepsilon,\phi)$.
\ep


\subsubsection{Proof of Lemma~\ref{lem:D-implies}}
\label{sec:pf-D-implies}

Let $\varepsilon_1 := \min \{ |g^f_\phi - g^{f'}_\phi| :  f, f' \in \Pi_D,g^f_\phi  \neq g^{f'}_\phi \} > 0$. Let $\zeta_1 := \min \{\zeta_0( \frac{\varepsilon_1}{2S}, \phi), \frac{\varepsilon_1}{2S}\}$ and consider $t$ sufficiently large, i.e., $t  >t_0$.
For $\zeta \in  (0,  \zeta_1)$, assume that the event $\set{D}_t(\zeta)$ occurs.


{\bf Proof of the first part of \eqref{eq:D-implies}.}
Then, %noting that $\phi$ and $\phi'_u$ are ergodic due to \eqref{eq:on-D-connect},
for any $u \in [i^t_1, t]$ and $f \in \Pi_D(\set{C}_u)$,
it follows from \eqref{eq:on-D-connect} that for any $x \in \set{S}$, 
\begin{align}
|g^f_{\phi'_u} -g^f_{\phi}|  
& =
|(\mathbf{B}^f_{\phi'_u}h^f_{\phi'_u})(x) -(\mathbf{B}^f_{\phi}h^f_{\phi}) (x)| \nonumber \\
& \le | r_{\phi'_u}(x, f(x)) - r_{\phi} (x, f(x)) |
+  \sum_{y \in \set{S}}  | h^f_{\phi'_u}(y) - h^f_{\phi}(y) |  \nonumber \\
& \le S \frac{\varepsilon_1}{2S} =  \frac{\varepsilon_1}{2}   \label{eq:D-implies-1}
\end{align}
where the last inequality stems from the definition of $\set{E}''_t(\frac{\varepsilon_1}{2S})$
in \eqref{eq:on-D-connect}.
Then, for any $u \in [i^t_1, t]$, $f \in  \Pi^*(\phi'_u)$, and $f' \in \Pi_D(\set{C}_u)$, we have:
\begin{align*}
g^f_{\phi} ~\ge~ g^f_{\phi'_u} - \frac{\varepsilon_1}{2} 
~\ge~ g^{f'}_{\phi'_u} - \frac{\varepsilon_1}{2} 
~\ge~ g^{f'}_{\phi} - \varepsilon_1
\end{align*}
where the first and last inequalities stem from \eqref{eq:D-implies-1},
and the second inequality is deduced from the optimality of $f$ under $\phi'_u$.
Noting that $f, f' \in \Pi_D(\set{C}_u)$,
it follows that
$g^f_{\phi(\set{C}_u)} = g^f_{\phi} \ge  g^{f'}_{\phi} = g^{f'}_{\phi(\set{C}_u)}$. 
Hence $f$ is optimal under $\phi(\set{C}_u)$ (the choice of $f' \in \Pi_D(\set{C}_u)$ is arbitrary). This completes the proof of the first part in \eqref{eq:D-implies}.

{\bf Proof of the second part of \eqref{eq:D-implies}.}
Fix $u \in [i^t_1, t]$.
Assume that
\begin{align} \label{eq:D-implies-assum}
\Pi_D(\set{C}_{u+1}) \cap  \Pi^*(\phi'_u) \neq \emptyset .
\end{align} 
Then, from the first part of \eqref{eq:D-implies}, we deduce that:
\begin{align*}
\Pi_D(\set{C}_{u+1}) \cap  \Pi^*(\phi'_u) 
~\subseteq~ \Pi_D(\set{C}_{u+1}) \cap  \Pi^*(\phi(\set{C}_u)).
\end{align*}
Combining this with the assumption \eqref{eq:D-implies-assum}, we get that $\Pi_D(\set{C}_{u+1}) \cap  \Pi^*(\phi(\set{C}_u))\neq\emptyset$, which implies that $g^*_{u+1}  \ge g^*_{u}$. 
%This means that at least one optimal policy in both $\phi'_u$ and $\phi(\set{C}_u)$
%remains in the restricted MDP 
It remains to prove \eqref{eq:D-implies-assum}. 


Let $x = X_u$. We first show that: 
\begin{equation}\label{eq:qqq}
\set{C}_{u+1} (x) \cap \set{O} (x ; \phi'_u) \neq \emptyset.
\end{equation}

If the algorithm enters the monotonization phase, i.e., the event $\set{E}^\mnt_u$ occurs, then it selects action $a=A_u\in {\cal C}_u(x) \cap \set{O} (x ; \phi'_u)$. We deduce that: 
\begin{align*}
N_u(x, a) \ge \log^2( N_u(x)), \quad
N_{u+1}(x, a)  = N_{u}(x, a)  + 1,  \quad\text{and}\quad 
N_{u+1}(x)  = N_{u}(x)  + 1
\end{align*}
Thus, using the fact that $\log^2 (n) +1 > \log^2 (n+1)$, we obtain
\begin{align}
N_{u+1}(x,a)  \ge \log^2 (N_u (x)) +1  \ge \log^2 (N_u (x) +1) 
= \log^2 (N_{u+1} (x)). \label{eq:monotone-log-trick}
\end{align}
We have shown that $a\in \set{C}_{u+1}(x)$ and thus $a \in \set{C}_{u+1} (x) \cap \set{O} (x ; \phi'_u) \neq \emptyset$.

In case that the event $\set{E}^\mnt_u$ does not occur, 
there must exist an action $a \in \set{O}(x; \phi'_u)$ such that 
$N_u(x, a) \ge \log^2( N_u(x)) + 1$. Hence, as for \eqref{eq:monotone-log-trick}, we get: 
\begin{align*}
N_{u+1}(x,a) \ge N_{u}(x,a)  \ge \log^2 (N_u (x)) +1  \ge \log^2 (N_u (x) +1) 
= \log^2 (N_{u+1} (x)) 
\end{align*}
which implies $a \in \set{C}_{u+1} (x) \cap \set{O} (x ; \phi'_u) \neq \emptyset$. 

Now \eqref{eq:qqq} implies \eqref{eq:D-implies-assum} (since for any $y \in \set{S}$ such that $y \neq x$, $\set{C}_u (y) = \set{C}_{u+1} (y)$). This completes the proof of the second part in \eqref{eq:D-implies} and that of  Lemma~\ref{lem:D-implies}.
\ep



\subsubsection{Proof of Lemma~\ref{lem:difficult-bound-3}}
\label{sec:pf-difficult-bound-3}


We first define 



\begin{lemma} \label{lem:concentr}
Consider any $\phi$ and $\pi$ with Bernoulli reward. Then, as $T \to \infty$,
\begin{align} \label{eq:kl-concentration}
\sum_{t=1}^T \Pr\left[\sum_{x\in \set{S}} \sum_{a\in \set{A}} N_t(x,a) \kl_{\phi_t \mid \phi}(x,a) \geq \log t + \log^2 \log t \right]  \le o(\log T).
\end{align}
\end{lemma}



\ep



==> proofth4.tex <==
% !TEX root =  appendix.tex


\section{Proof of Theorem~\ref{thm:ORL}}


We focus on the performance of DEL with $P(\phi, \set{F}_{\Phi}(\phi))$,
and we provide insights into analyze the performance of the two other versions of DEL. 
The proof is articulated around upper bounding the number of times a suboptimal action $a \notin \set{O}(x; \phi)$ may be selected in one of the three phases (exploitation, exploration, and estimation) of DEL. Hence, we will divide the regret into three terms correspondingly. We first define the following events:
\begin{align*}
\set{A}(t) &:= \left\{ N_t(X_t, a) \ge \left(\eta_t (X_t, a) + \sqrt{\delta_t} \right) \log N_t (X_t)~\forall a \in \set{A}\right\}, \\
\set{B}(t)&:= \{\|\phi - \phi_t\|  > \delta(\kappa)\}.
\end{align*}
$\set{A}(t)$ is the event that the algorithm enters the exploitation phase at time $t$,
and $\set{B}(t)$ is the event that the estimated model $\phi_t$ is inaccurate.
Remember that $r(x,a) \in [0, 1]$ for all $(x,a)$, and hence we can bound $\max_{(x,a)}\delta^*(x, a; \phi)$ with $S$, which further implies that the regret can be bounded as follows:
\begin{align}
R^\pi_T( x_1) \le   
 \EXP^\pi_{\phi \mid x_1}[W_1(T) ]+  S  \EXP^\pi_{\phi \mid x_1}[W_2(T) ]+  S\EXP^\pi_{\phi \mid x_1} [W_3(T)] + O(1) \label{eq:regret-decomp}
\end{align}
where 
\begin{align*}
W_1(T) &:= \sum_{t =1}^T \sum_{x \in \set{S}} \sum_{a \in \set{A}}  \delta^*(x, a; \phi)  \mathbbm{1}[(X_t, A_t)=(x, a), \neg \set{A}(t), \neg \set{B}(t)]  , \\
W_2 (T) &:=  \sum_{t = 1}^T    \mathbbm{1}[  \neg \set{A}(t), \set{B}(t), A_t \notin \set{O}(X_t;\phi)] ,  \\
W_3(T) &:=  \sum_{t = 1}^T   \mathbbm{1}[  \set{A}(t), A_t \notin \set{O}(X_t;\phi) ].
\end{align*}
We use the standard notation $\neg\set{U}$ to represent the event that $\set{U}$ does not occur.





For given $\phi$, let $\eta^*(\phi) = (\eta^*(x,a; \phi))_{(x,a)}$ denote the solution of $P(\phi, \set{F}_{\Phi}(\phi))$.








The proof of Lemma~\ref{lem:continuous} is provided at the end of this section, where we essentially show 
the continuity of $\delta^*(x, a;\phi )$ w.r.t. kernel parameters.
Since the weights on the feasibility set $\set{F}_{\TN{un}} (\phi)$ or $\set{F}_{\TN{lip}} (\phi)$ are continuous w.r.t. $\delta^*(x, a;\phi )$, we can find such 
$\delta(\kappa)$ for $P(\phi, \set{F}_{\TN{un}} (\phi))$ and $P(\phi, \set{F}_{\TN{lip}} (\phi))$.
%Recalling Proposition~\ref{prop:communicating-traslation}, we conclude the upper bound of regret by tracking all the events of selecting suboptimal actions.
Next define the following events: 

\medskip
{\bf Estimation and exploration.}
To bound $W_1(T)$, assume that $\neg \set{A}(t)$ and $(X_t,A_t) = (x,a)$ occur.
%, i.e., the algorithm selects suboptimal action $\underline{A}_t$ or
%$\overline{A}_t$ while the estimation $\phi_t$ is accurate.
We first obtain an upper bound of $s_t(x)$ and then bound $N_t(x,a)$.
%\begin{align}  \label{eq:s_t-bound}
%s_t(X_t) \le  |\set{A}|   \|\eta^*(\phi_k) \|_\infty  \log T 
%\end{align}
Hence, $\neg \set{A}(t)$ implies that there exists $a' \notin \set{O}(x; \phi_t)$ such that
\begin{align} 
N_t(x, a') &\le \eta^* (x, a' ; \phi_t) (1 + \gamma ) \log N_t(x)\label{eq:not-exploit-1} \\
& \le \|\eta^* (\phi_t)  \|_{\infty} (1+ \gamma) \log t . \label{eq:not-exploit-2}
\end{align}
If $a = \underline{A}_t$, then $N_t(x, a) \le N_t(x,  a')$, and thus \eqref{eq:not-exploit-2} implies
$N_t (x, a) \le \|\eta^* (\phi_t)  \|_{\infty} (1+ \gamma) \log t$. 
If $a = \overline{A}_t$,  then we have 
\begin{align}
N_t(x, a) &\le \eta^*(x, a ; \phi_t) \frac{N_t(x, a')}{\eta^*(x, a' ; \phi_t)} \nonumber \\
&\le \eta^*(x, a ; \phi_t) (1 + \gamma ) \log t  \label{eq:over-A}
\end{align}
where the last inequality follows from \eqref{eq:not-exploit-1}.
This implies $N_t (x, a) \le \|\eta^* (\phi_t)  \|_{\infty} (1+ \gamma) \log t$, and thus
\begin{align*}
s_t(x) \le |\set{A}| \|\eta^* (\phi_t)  \|_{\infty} (1+ \gamma) \log t,
\end{align*}
since $s_t(x)$ is incremented by $1$ only when $\neg \set{A}(t)$ occurs and $X_t = x$.
When $a = \underline{A}_t$, i.e., $N_t(x, a) \le \varepsilon s_t(x)$, the upper bound of $s_t(x)$ implies
\begin{align}
N_t(x, a) &\le \varepsilon s_t(x) \nonumber \\
& \le \varepsilon |\set{A}| \|\eta^* (\phi_t)  \|_{\infty} (1+ \gamma) \log t . \label{eq:under-A}
\end{align}
Combining \eqref{eq:over-A} and \eqref{eq:under-A}, we obtain
\begin{align} \label{eq:suboptimal-W3}
\sum_{t= 1}^T \mathbbm{1}[(X_t, A_t) = (x,a),  \neg \set{A}(t), \neg \set{B}(t)] 
\le  
\left(  \eta^*(x, a ; \phi_t) + \varepsilon |\set{A}| \|\eta^* (\phi_t)  \|_{\infty} \right) (1+\gamma) \log T  \;.
\end{align}
The construction of $\delta(\kappa)$ in Lemma~\ref{lem:continuous} 
and $\neg \set{B}(t)$
ensure that $\set{O}(x; \phi) = \set{O}(x ; \phi_t)$ and that:
\begin{align*}
 K_{\Phi}(\phi_t) &= \sum_{x \in \set{S}} \sum_{a \in \set{A}} \delta^*(x, a; \phi_t) \eta^*(x, a ;\phi_t)  
\le K_{\Phi}(\phi) (1+ \kappa)   \\
\varepsilon \xi( \phi_t) &= \varepsilon |\set{S}| \cdot |\set{A}| \|\eta^*(\phi_t) \|_{\infty} 
 \sum_{x\in \set{S}}\sum_{a \in \set{A}} \delta^*(x,a;\phi_t) 
\le 2 \varepsilon  \xi( \phi) \;.
\end{align*}
From \eqref{eq:suboptimal-W3}, we obtain
$W_1(T) \le ( K_\Phi (\phi) (1+\kappa) + 2 \varepsilon \xi(\phi) ) (1+\gamma) \log T$
which implies
\begin{align} \label{eq:W1-bound}
\limsup_{T \to \infty}
\frac{W_1(T)}{\log T} \le ( K_\Phi (\phi) + 2 \varepsilon \xi(\phi) ) (1+\gamma), 
\end{align}
since the choice of $\kappa >0$ is arbitrary.
If we solve the optimization problem $P(\phi, \set{F}_{\TN{un}} (\phi))$ or $P(\phi, \set{F}_{\TN{lip}} (\phi))$,
we may have $K_{\TN{un}} (\phi)$ or $K_{\TN{lip}} (\phi)$, respectively, instead of $K_\Phi (\phi)$. 


%Then, recalling \eqref{eq:regret-decomp}, it follows that
%\begin{align*}
%\limsup_{T \to \infty}\frac{R^\pi_T(x_1)}{\log T} 
%\le 
%( K_\Phi (\phi) (1+\kappa) + 2 \varepsilon \xi(\phi) ) (1+\gamma) 
%+ 
%\frac{ |\set{S}| \cdot \EXP^\pi_{\phi \mid x_1}[W_3(T) + W_2(T) ]  }{ \log T}
%+o(1) \;.
%\end{align*}
%Hence, for the proof, it is sufficient to obtain a constant upper bound of $\EXP^\pi_{\phi \mid x_1}[W_3(T) + W_2(T) ]$
%since the choice of $\kappa$ is arbitrary.

\medskip
{\bf Concentration.} To bound $W_2(T)$, we use the following concentration result:
\begin{lemma}  \label{lem:deviation}
\cite{Combes2014}
Consider any $\phi$, $\pi$, $\epsilon > 0$ with Bernoulli reward distribution. Define ${\cal H}_t$ the $\sigma$-algebra generated by
$( Z_s )_{1 \leq s \leq t}$. Let $\set{B} \subset \mathbb{N}$ be a (random) set of rounds. Assume that there exists a sequence of (random) sets $(\set{B}(s))_{s\ge 1}$ such that (i) $\set{B} \subset \cup_{s \geq 1} \set{B}(s)$, (ii) for all $s\ge 1$ and all $t\in \set{B}(s)$, $N_t(x, a) \ge \epsilon s$, (iii) $|\set{B}(s)| \leq 1$, and (iv) the event $t \in \set{B}(s)$ is ${\cal H}_t$-measurable. Then for all $\delta > 0$, and $x_1, x, y \in \set{S}$, $a \in \set{A}$,
\begin{align*}
 \sum_{t \geq 1} \Pr^\pi_{\phi \mid x_1}[ t \in \set{B} , | r_t(x, a) - r_\phi ( x,a ) | > \delta] & \leq 
  \frac{1}{\epsilon \delta^2} \\
 \sum_{t \geq 1} \Pr^\pi_{\phi \mid x_1}[ t \in \set{B} , | p_t(y \mid x, a) - p_\phi (y \mid x,a ) | > \delta] &\leq 
  \frac{1}{\epsilon \delta^2} 
\end{align*}
\end{lemma}
\citet{Combes2014} provides a rigorous proof of the first part.
Now the occurrence of a transition under action $a$ from state $x$ to state $y$ is a Bernoulli random variable, and the second part of the lemma directly follows from the first part.

To use Lemma~\ref{lem:deviation}, we define $\set{B}(x,a; t)$ as the event that $\neg \set{A}(t)$ and $\|\phi(x, a) - \phi_t(x,a) \| > \delta(\kappa)$.
%and $\set{B} (x; t) :=  \cup_{a \in \set{A}} \set{B}(x,a; t)$
so that $\neg \set{A}(t)\cap \set{B}(t) = \cup_{(x,a) \in \set{S} \times \set{A}} \set{B}(x,a; t)$.
 We claim that $\min_{a \in \set{A}} N_t(x,a) \ge \frac{\varepsilon s_t(x)}{2}$ when $s_t(x)$ is large.
The claim can be proved by contradiction. Suppose that this is false, i.e., 
 $\min_{a \in \set{A}}N_t(x,a) < \frac{\varepsilon s_t(x)}{2}$. Up to time $t$, there exist $\lfloor \frac{s_t(x)}{2}\rfloor$ rounds $\{\tau_1, ...,  \tau_{\lfloor \frac{ s_t(x)}{2} \rfloor}  \}  \subset  \{1, ..., t\}$ such that $\neg \set{A}(\tau_i)$ occurs, $X_{\tau_i} = x$, and $\frac{s_t(x)}{2} \le s_{\tau_i}(x)$, i.e.,
 \begin{align*}
 \min_{a \in \set{A}}N_{\tau_i}(x,a) \le \min_{a \in \set{A}}N_t(x,a) \le \varepsilon s_{\tau_i}(x) \;.
\end{align*}
In such rounds, the algorithm always picks an action with the minimum occurrences. 
Since for $A$ of such rounds, the minimum occurrence have been incremented by at least $1$, we have $\min_{a \in \set{A}}N_{\tau_i}(x,a) \ge \frac{1}{|\set{A}|} \cdot \lfloor \frac{s_t(x)}{2} \rfloor$ which yields a contradiction if we choose $\varepsilon < \frac{1}{A}$.
Hence, when both $\neg \set{A}(t)$ and $\set{B}(x, a; t)$ occur, we have 
$\min_{a \in \set{A}} N_t(x,a) \ge \frac{\varepsilon s_t(x)}{2}$.
Applying Lemma~\ref{lem:deviation}, we obtain
\begin{align*}
\sum_{t \ge 1} \Pr^\pi_{\phi \mid x_1}[ \set{B}(x, a;t)]  \le  \frac{|\set{S}+1|}{\varepsilon \delta^2(\kappa)}
\end{align*}
where the union bound w.r.t. $y \in \set{S}$ and reward gives the factor $|\set{S}+1|$.
Hence, using the union bound, we bound $\EXP^\pi_{\phi \mid x_1}[W_2(T)]$ as follows:
\begin{align*}
\EXP^\pi_{\phi \mid x_1}[W_2(T)]
&\le  \sum_{t = 1}^T    \Pr^\pi_{\phi \mid x_1}[ \neg \set{A}(t), \set{B}(t)]   \\
&\le  \sum_{t \ge 1} \sum_{x\in \set{S}}
\sum_{a \in  \set{A}} \Pr^\pi_{\phi \mid x_1}[ \set{B}(x, a;t)]  \\
& \le  \frac{|\set{S}+1||\set{S}||\set{A}|}{\varepsilon \delta^2(\kappa)} 
\end{align*}
which is constant in $T$ and thus
\begin{align} \label{eq:W2-bound}
\limsup_{T \to \infty} \frac{\EXP^\pi_{\phi \mid x_1}[W_2(T)]}{\log T} = 0 .
\end{align} 



\medskip
{\bf Exploitation Phase.} Finally we bound $W_3(T)$.
Assume $\set{A}(t)$ occurs and $A_t \notin \set{O}(X_t; \phi)$.
Further, assume that $\phi \in  \Delta_\Phi(\phi_t)$. Then we must have
\begin{align*}
\sum_{x \in \set{S} } \sum_{a \in \set{A}} 
N_t(x,a)  \kl_{\phi_t \mid \phi} (x,a)  \ge (1+ \gamma ) \log t 
\end{align*}
since $\eta^*(\phi_t)$ is a feasible solution of $\set{F}_\Phi (\phi_t)$ and $\set{A}(t)$ occurs, i.e.,
for all $\psi \in \Delta_\Phi (\phi_t)$,
$\sum_{x \in \set{S} } \sum_{a \in \set{A}} 
N_t(x,a)  \kl_{\phi_t \mid \psi} (x,a)  \ge (1+ \gamma ) \log t $.
In this case, the following concentration provides an upper bound of $W_3(T)$ :
\begin{lemma} \label{lem:concentr}
\cite{magureanu2014}
Consider any $\phi$ and $\pi$ with Bernoulli reward.
Then there exists a function $G$ such that
\begin{align} \label{eq:kl-concentration}
\sum_{t \ge 1} \Pr\left[\sum_{x\in \set{S}} \sum_{a\in \set{A}} N_t(x,a) \kl_{\phi_t \mid \phi}(x,a) \geq (1+\gamma) \log~t\right]  \le G(\gamma,|\set{S}|, |\set{A}|).
\end{align}
\end{lemma}
From Lemma~\ref{lem:concentr} and our assumptions, we have 
\begin{align*}
\sum_{t = 1}^T   \EXP^\pi_{\phi \mid x_1}[  \set{A}(t), A_t \notin \set{O}(x;\phi), \phi \in \Delta_{\Phi}(\phi_t) ]
\le G(\gamma,|\set{S}|, |\set{A}|).
\end{align*}
Recall Theorem~\ref{thm:unrelated}~and~\ref{thm:lip}: for unstructured $\Phi$, we have $\set{F}_{\TN{un}}(\phi) \subset \set{F}_{\Phi} (\phi)$,
and for Lipschitz $\Phi$, we have $\set{F}_{\TN{lip}}(\phi) \subset \set{F}_{\Phi} (\phi)$.
Hence, for both cases, we also ensure \eqref{eq:kl-concentration} on the event $\set{A}(t), A_t \notin \set{O}(x;\phi), \phi \in \Delta_{\Phi}(\phi_t)$, and thus obtain the same upper bound.



We now suppose that $\phi \notin \Delta_\Phi(\phi_t)$. Since we assume the uniqueness of the optimal deterministic policy $f^* \in \Pi^*(\phi) = \{f^*\}$, we have $\Pi^*(\phi) \cap \Pi(\phi_t) = \emptyset$.
In addition, when $\set{A}(t)$ occurs, the algorithm ensures that 
$\min_{a\in\set{A}}N_t(X_t, a) > 0$. Then due to (\ref{eq:erg}), 
$\Pr^\pi_{\phi \mid x_1} [N_t(x) \le \rho t] \le C \exp (- \rho t/2)$,  which implies 
\begin{align*}
\sum_{ t =1}^T \Pr^\pi_{\phi \mid x_1} 
\left[ \min_{(x,a) \in \set{S} \times \set{A}}N_t (x, a)  \right] \le  |\set{S}||\set{A}| C \frac{1}{1- e^{\rho/2}} \;.
\end{align*}
From the above inequality, we can restrict our attention to the case where the estimated $\phi_t$ is absolutely continuous w.r.t. $\phi$. Hence, on this event, $\phi\notin\Delta_\Phi(\phi_t)$ implies that $\phi_t$ is  inaccurate at some $(x, a)$ such that $a \in \set{O}(x ; \phi_t)$, i.e., there exists $\delta > 0$ such thats
\begin{align*}
\max_{(x,a): a \in \set{O} (x; \phi_t)} \|\phi(x,a) - \phi_t(x,a)\| > \delta 
\end{align*}
where the existence of $\delta$ can be guaranteed as in Lemma \ref{lem:continuous}.
Therefore, applying Lemma~\ref{lem:deviation} and (\ref{eq:erg}) again, c.f., Proposition~5 in \cite{burnetas1997optimal},
\begin{align*}
\sum_{t = 1}^T  \EXP^\pi_{\phi \mid x_1}[ \set{A}(t), A_t \notin \set{O}(x;\phi), \phi \notin \Delta_{\Phi}(\phi_t) ]
= o(\log T) \;.
\end{align*}
Combining \eqref{eq:W1-bound} and \eqref{eq:W2-bound}, this completes the proof of Theorem~\ref{thm:ORL}. \ep

%{\bf  Regret analysis with simplified problem.} 
%We now consider s
%Since only the optimization problem is replaced, we check how this replacement impact on the proof.
%First, we need to show continuity so that the same $\delta(\kappa)$
%Since 
%Note that we have \eqref{eq:W1-bound} 
%
%First, it is straight forward to check 



{\bf Proof of Lemma~\ref{lem:continuous}.} 
%For any $\psi \in \Phi$, the feasible set $\set{F}_\Phi (\psi)$ is convex and $\delta^*(x, a ; \psi)$ is 
Recalling the assumption that $P(\phi, \set{F}_\Phi (\phi))$ has a unique solution and $\phi$ has a unique optimal stationary policy, it suffices to show that the mappings $\psi \mapsto \delta^*(x, a;\psi)$ and $\psi \mapsto \kl_{\psi \mid \phi}( x, a)$ 
are continuous at $\phi$
since they imply that the mappings $\psi \mapsto K_{\Phi}(\psi)$ and $\psi \mapsto \eta^*(\psi)$ are continuous at $\phi$. 
To do so, we first note that there exists $\delta>0$ such that $\phi \ll  \psi$ for all $\psi$ verifying $\|\phi - \psi\| < \delta$.
Hence, with our assumption $\psi \ll \phi$, this implies that $\phi$ and $\psi$ are mutually absolutely continuous
and thus $\psi$ is also ergodic. Hence, the KL divergence of $\psi$ to $\phi$ is bounded and continuous at $\phi$ w.r.t. $\psi$.
From now on, we consider $\psi$ which is mutually absolutely continuous with $\phi$.


Consider the policy evaluation equations of stationary policy $f$ under $\phi$ and $\psi$, which can be written 
as vector and matrix multiplications:
\begin{align*}
g^f_\phi &= P^f_\phi g^f_\phi  \\
h^f_\phi &= r^f_\phi - g^f_\phi + P^f_\phi h^f_\phi 
\end{align*}
similarly 
$g^f_\psi = P^f_\psi g^f_\psi$ and $h^f_\psi = r^f_\psi - g^f_\psi + P^f_\psi h^f_\psi$,
where $P^f_{\phi}$ (resp. $P^f_\psi$) and $r^f_\phi$ (resp. $r^f_\phi)$ are the transition matrix and reward vector w.r.t. policy $f$ under $\phi$ (resp. $\psi$), respectively, c.f., \cite{puterman1994markov}.
Since both $\phi$ and $\psi$ are ergodic, by forcing $h^f_{\phi} (x_1) = h^f_{\psi} (x_1) = 0$ for some $x_1$,
the bias functions $h^f_{\phi}$ and $h^f_{\psi}$ can be uniquely defined. 
Let $D^f := P^f_\phi - P^f_\psi$ and $d^f := h^f_\phi - h^f_\psi$.
Then, $\| D^f \| \le |\set{S}| \delta$ where $\|\cdot \|$ is the max norm.
Noting that the ergodicity of $\phi$ and $\psi$ further provides the invertibility of $I - P^f_\phi$ and $I - P^f_\psi$.
a basic linear algebra, c.f., Lemma~7 in \cite{burnetas1997optimal}, leads to that for any $\epsilon  > 0$, $ \|d^f\| \le \epsilon$ if
\begin{align*}
\| D^f\| \le \frac{\epsilon}{\|(I-P^f_\phi)^{-1} \| (\|h^f_\phi \|+ \epsilon)} \;.
\end{align*}
The above continuity of $h^f_{\psi}$ w.r.t. $\psi$ at $\phi$ is valid for arbitrary $f$. Hence, $h^*_{\psi}$ and thus $\delta^*_\psi$ are continuous at $\phi$. 
%Then, noting $g^*_\phi$ and $h^*_\phi$ can be obtained by solving linear equations, basic algebra provides us to estimate in $t$. A more precise argument is made in \cite{combes17} using Berge's maximal theorem.
\ep















==> result.tex <==
% !TEX root =  main.tex

\section{Analysis}

In this section, we analyze the convergence of Dab Q-learning. We first establish that $\theta_n$ tends to $\theta^\star$, the parameter of the optimal, i.e., that minimizing the projected Bellman error. We then study the asymptotic covariance of the algorithm, and finally highlight the role of ER. 

We make the following assumptions:
\begin{enumerate}[label={(A\arabic*)}]
\item \label{A:step} 
%We consider $\alpha_n = (n+1)^{-\alpha}$, $\beta_n = (n+1)^{-\beta}$ with $1\ge \alpha > \beta > 1/2$.
%{\tt Please change the corresponding explains... Actually, we need little bit tricky conditions on step size. However, once we choose $\alpha_n = (n+1)^{-\alpha}$, $\beta_n = (n+1)^{-\beta}$, where $1\ge \alpha > \beta > 1/2$. Everything that we need is satisfied. }
(i) $\sum_{n =0}^\infty \alpha_n = \infty,  \sum_{n =0}^\infty \beta_n= \infty$, \\
$\sum_{n =0}^\infty \alpha_n^2 < \infty,  \sum_{n =0}^\infty \beta_n^2 < \infty$;\\
(ii) $\lim_{n \to \infty} \frac{ \alpha_n}{\beta_n}  = 0$;\\
(iii)$\forall n$, $0 \le {\alpha_n} - {\alpha_{n+1}} \le \alpha_n^2$, $0 \le {\beta_n} - {\beta_{n+1}}  \le  \beta^2_n$.

\item \label{A:invert} $A(\theta')$ is invertible for all $\theta \in \mathbb{R}^d$ so that
for each greedy policy w.r.t. $\theta$, solution of $A(\theta')\theta + b = 0$  is unique.
\item \label{A:contract} $\bold{T}\bold{B}^{\star}$ is a contraction mapping w.r.t. some norm $\|\cdot \|_c$, i.e., there exists a constant $\gamma \in [0,1)$ such that for all $\theta, \theta' \in \mathbb{R}^d$,
$\|\bold{T}\bold{B}^{\star} Q_{\theta} - \bold{T}\bold{B}^{\star} Q_{\theta'}\|_{c}
 \le \gamma \|Q_{\theta} - Q_{\theta'}\|_{c}$.
\end{enumerate}

Note that we do not assume that the Markov chain describing the system dynamics under the behavior policy$\pi_b$ is aperiodic. This contrasts with existing convergence analysis of previously proposed algorithms (strong mixing, e.g., $\alpha$-mixing or aperiodicity is often assumed, which explicitly regulates correlation between consecutive samples. 

\ref{A:step}(i) is an essential condition for convergence of stochastic approximation algorithms \cite{borkar2008book}. \ref{A:step}(ii) means that the time-scales at which $\theta_n$ and $\hat{A}_n(\theta_m')$ are separated. \ref{A:step}(iii) implies that each sequence of step sizes is decreasing smoothly. This is necessary to eliminate a potential risk of divergence due to resonance between the step sizes and the behavior of system under $\pi_b$ if the resulting Markov chain is periodic. \ref{A:step}(iii) is not necessary when the Markov chain is aperiodic. \ref{A:step} holds for the following choice of step sizes: $\alpha_n = (n+1)^{-\alpha}$, $\beta_n = (n+1)^{-\beta}$, where $1\ge \alpha > \beta > 1/2$.

Further observe that since the state and action spaces are finite, the set of all possible greedy policies $\pi_\theta$, $\theta\in \mathbb{R}^d$ is finite. Thus, the number of all possible $A(\theta)$ is also finite. \ref{A:invert} is necessary to ensure the uniqueness of the fixed point of $\bold{T}\bold{B}^{\theta}$ for every greedy policy $\pi_\theta$. This is an essential assumption that allows the corresponding ODE \eqref{eq:ode2} has a unique asymptotically global equilibrium which is ensured by the invertibility of $A(\theta)$. The same assumption on $A(\theta)$ is also made in previous works, e.g., \cite{sutton2009fast}.

Finally, together with the facts that the feature function $(\phi_i)_{i=1,\ldots,d}$ are linearly independent, \ref{A:contract} is needed to ensure the existence and uniqueness of the parameter $\theta^\star$ minimizing $e(\theta)$. Indeed, although $\bold{B}^*$ is contraction with respect to $\| \cdot \|_\infty$ and $\bold{T}$ is non-expanding with respect to $\| \cdot \|_{\mu}$,
we cannot guarantee that $\bold{T}\bold{B}^*$ is contraction in $\| \cdot \|_{\infty}$ or $\| \cdot \|_{\mu}$. Also note that in absence of function approximation, \ref{A:contract} and \ref{A:invert} with $\|\cdot\|_c=\|\cdot \|_\infty$ are verified if the behavior policy visits every state and action infinitely often, i.e., $\mu(s, a) >0$. See Section~2.1 of \cite{bertsekas2011approximate} for a more detailed  discussion on sufficient conditions under which \ref{A:contract} holds.


\subsection{Convergence guarantee}

\begin{theorem} \label{thm:convergence}
Assume that 
\ref{A:step}, \ref{A:invert}, and \ref{A:contract}
 hold, and that the Dab Q-learning algorithm uses samples $\xi_n$ extracted by i.i.d. sampling or sampling with ER with $W \ge B\ge 1$. Then $\theta_n$ converges almost surely to $\theta^\star$ minimizing $e(\theta)$ over $\theta$ (i.e., ${e}(\theta^\star)=0=\mathcal{E}(\theta^\star, \theta^\star) = 0$).
\end{theorem}

The proof of the above theorem is provided in Appendix, and leverages ODE  techniques as in \cite{kushner1997} for the analysis of stochastic approximation algorithms. These techniques are adapted and extended to our general setting where the Markov chain describing the system dynamics can be periodic (hence introducing a periodic behavior of the {\it noise} averaged by the algorithm). We prove that between two updates in the target policy, the system behaves like the solution of an ODE, which then allows us to study the convergence of the target policy.

Experience Replay does not play any specific role in the convergence of the algorithm as convergence is achieved even for any $W$ and $B$ and even when $W=1=B$ (i.e., without ER). Actually, ER makes the analysis challenging due to the inherent correlations among successive samples (with ER, the same transition can be used in several iterations of the algorithm). In the proof of Theorem \ref{thm:convergence}, we establish that the proposed implementation of sampling with ER together with step sizes satisfying (A1) ensure that the sample correlations do not accumulate and are mitigated over time even when chain is periodic.

It is worth noting that most previous analysis, see e.g. \citet{sutton2009fast}, \cite{melo2008analysis}, assume that the Markov chain induced by $\pi_b$ is aperiodic, so that it has fast mixing, e.g., uniformly or geometrically ergodic. In addition, sample correlations are generally not handled carefully. In particular, Assumption \ref{A:step}(iii) on the step-sizes is not considered in earlier work, and seems critical to handle these correlations, and to derive unbiased observations.

%Indeed, one can easily find a counterexample, in which sample-dependent step size
%causes divergence, e.g., using $\alpha_n = \frac{1}{n}$ for some set of observation.
%Beside this, their proof has some logical gap
%\cite{sutton2009convergent, melo2008analysis}
%\footnote{The proof of Theorem~5.1 of \cite{sutton2009convergent} is unsound in calculating the conditional expectation.
%In \cite{melo2008analysis}, 
%the analysis mainly relies on Theorem~17 of \cite{benveniste2012adaptive}, but
%there is no proof that the conditions are satisfied even when two consecutive updates are correlated due to the trajectory sampling.}.

 \citet{devraj2017zap} analyze the convergence of Zap Q-learning, which can be seen as a version of Dab Q-learning without ER nor function approximation, and with $\tau=0$. They consider aperiodic Markov chains only, and make the assumption that the frequency at which the target greedy policy is updated  is controlled: $\sum_{n= 0}^\infty \beta_n 1_{ [\pi_{\theta_n} \neq \pi_{\theta_{n+1}}]} < \infty$. Having $\tau >0$ in Dab Q-learning simplifies the analysis and removes the need for this assumption. 

%\footnote{Consider a Markov chain with state space $\mathcal{S}$.
% and stationary distribution $\mu$ over $\mathcal{S}$ 
%such that for measurable set $U \subset \mathcal{S}$,
%there exist bounded functions $f$ and $g$ such that 
%$\left| \Pr[S_n \in U \mid \mathcal{H}_0] - \mu(U) \right| \le 
% f(U)g(n)$.
%When $g(n) = \rho^{\lfloor {n}/{n'} \rfloor}$ with $\rho \in [0,1)$, we say the Markov chain is
% uniformly ergodic.  If $g(n) = \rho^{n}$ with $\rho \in [0,1)$ and some constant $n'$, then we say it is geometrically ergodic. 
%}.




%In particular, our result extends the convergence for the periodic case, i.e., $L_{\max} \ge 2$,
%unless the chain has a unique stationary distribution.
%We note that the Markov chain with finite state space has a unique stationary distribution
%if and only if it has a unique essential communicating class.
%Hence, our convergence result do not require the chain to be aperiodic or mixing fast.
%However, in such periodic or slow-mixing cases,
%we additionally need to use either experience replay with $W \ge L_{\max}$ or non-increasing step size, e.g., $\alpha_n = \frac{1}{n}$, which are easily implemented in practice.




\subsection{Convergence rate}\label{sec:rate}

For simplicity, we assume here that the step size used in the $n$-th iteration is $\alpha_n = (n+1)^{-\alpha}$, $\beta_n = (n+1)^{-\beta}$, where $1\ge \alpha > \beta > 1/2$. In other words, we ignore the impact of the fact that step-sizes are updated at renewal epochs only (this happens regularly in steady-state). We study the rate of convergence of DAB Q-learning through the asymptotic behavior of the scaled error sequence $(\theta_n - \theta^*)/\sqrt{\alpha_n}$. We further assume that the Markov chain generated under policy $\pi_b$ is aperiodic. This assumption is needed to ensure that the asymptotic covariance matrix $\Sigma_{\theta^\star} : = \lim_{n \to \infty}  \frac{1}{\alpha_n} \EXP \left[  (\theta_n - \theta^\star)   (\theta_n - \theta^\star)^\top \right]$ is well defined. In case of periodic Markov chain, the limit might not exist due to oscillations. The following theorem establishes the convergence in distribution of the scaled error $(\theta_n - \theta^*)/\sqrt{\alpha_n}$ to a normal distribution of covariance matrix $\Sigma_{\theta^\star}$, and provides an explicit expression of this matrix.

\begin{theorem} \label{thm:covariance}
Assume that (A1), (A2), and (A3) hold, and that the Dab Q-learning algorithm uses samples $\xi_n$ extracted by i.i.d. sampling or sampling with ER with $W \ge B\ge 1$. Further assume that the system starts in steady-state\footnote{Remember that when ER is used with a window size equal to $W$, the system is started at time $-W+1$. Hence, we assume that $(s_0,a_0)\sim\mu$ without ER, and that $(s_{-W+1},a_{-W+1})\sim\mu$ with ER.}. The scaled error sequence $({\theta}_n- \theta^\star)/\sqrt{\alpha_n}$ weakly converges to a normal distribution $\mathcal{N}(0, \Sigma_{\theta^\star})$ where
\begin{align} \label{eq:asymp-cov}
\Sigma_{\theta^\star} & = \lim_{n \to \infty}  \frac{1}{\alpha_n} \EXP \left[  (\theta_n - \theta^\star)   (\theta_n - \theta^\star)^\top \right]\nonumber\\
& = (A^\star)^{-1} \Sigma (A^\star)^{-\top}.
\end{align}
In the above expression, we have $A^\star := A(\theta^\star)$, and 
\begin{align} \label{eq:core-cov}
\Sigma &:=
\Sigma_0
+
\sum_{n =1}^{\infty}
( \Sigma_n
+
\Sigma_n^\top
)\;, \\
\Sigma_n &:=  
%\left(\sum_{i = 1}^B \right)
\EXP  \left[
( {A}^\star_{n} \theta^\star  + {b}_{n}) ( {A}^\star_{0} \theta^\star  + {b}_{0})^\top \right]  \;,
\nonumber
\end{align}
where  ${A}^\star_{n} := \frac{1}{B}\sum_{i = 1}^B A_{n, i}(\theta^\star)$,  ${b}_{n} := \frac{1}{B}\sum_{i = 1}^B b_{n,i}$. The covariance matrix $\Sigma$ is referred to the core covariance.
\end{theorem}

The asymptotic covariance matrix $\Sigma_{\theta^\star}$ obtained under Dab Q-learning is optimal in the following sense. If we assume that the parameter $\theta_m'$ is fixed to $\theta^\star$, and assume that instead of using the gain matrix $\Gamma_n$ in the updates of $\theta_n$, we use a fixed gain matrix $\Gamma$ such that $\Gamma A^\star$ and $\Gamma A^\star+I/2$ are Hurwitz. The latter conditions ensure that the algorithm would yield a finite asymptotic covariance matrix for the scaled error (see Appendix A.1 in \citet{devraj2017zap}), and denote by $\Sigma_{\theta^\star}(\Gamma)$ this covariance matrix. Then we have $\Sigma_{\theta^\star}(\Gamma) \ge \Sigma_{\theta^\star}$ in the sense that for all $x \in \mathbb{R}^d$, $x^\top (\Sigma_{\theta^\star}(\Gamma) - \Sigma_{\theta^\star}) x \ge 0$.

%Using almost identical analysis to Theorems~\ref{thm:convergence}~and~\ref{thm:covariance},
%we can also show that GTD or GTD2 with gain matrix $\Gamma$ 
%converges to $\theta^*$ and  the same asymptotic covariance if
%$C := \EXP_\mu [\varphi \varphi^\top]$ is invertible.
%A formal description is provided in the supplementary material.

\subsection{The Role of Experience Replay}

As stated in Theorem \ref{thm:convergence}, ER does not play any role in the convergence of Dab Q-learning. However, ER may affect the rate at which the algorithm converges. In this section, we study the impact of ER on the asymptotic covariance matrix of the scaled error derived in Theorem \ref{thm:covariance}. 

The way we sample the trajectory generated under $\pi_b$ does not influence the matrix $A^\star$. Hence we are interested in how ER affects the core covariance matrix $\Sigma$. As a reference, we define the {\it unit} core covariance matrix $S_0$ as that obtained in steady-state using a single sample $B=1$: 
$$
S_0=\mathbb{E}_\mu \left[ ( \tilde{A} \theta^\star  + \tilde{b}) ( \tilde{A} \theta^\star  + \tilde{b})^\top  \right],
$$ 
where $\tilde{A} = \varphi (\lambda \varphi'(\theta^\star) - \varphi )^\top$ and $\tilde{b} = \hat{r} \varphi$. Define $\Sigma_{\iid} (B)$ and $\Sigma_{\ER} (B, W)$ as the core covariance matrices \eqref{eq:core-cov} under i.i.d. sampling with batch size $B >0$
and ER with batch size $B > 0$ and window size $W \ge B$, respectively.

\begin{proposition} \label{prop:covariance-calc}
We have: for any $1\le B\le W$,  \\
(i) $\Sigma_{\iid}(B) = \frac{1}{B} S_0=\lim_{W \to \infty }\Sigma_{\ER}(B, W)$;\\
(ii) $\Sigma_{\ER}(W, W) = \Sigma_{\ER}(1, 1)$.
\end{proposition}

(i) suggests that to reduce the asymptotic covariance matrix and to increase the convergence rate, we should use large sample batches, and even much bigger windows. (ii) indicates that we can not expect performance gains when the batch size is similar to the window size. These observations are well aligned with the choices made by practioners, e.g. $B = 32$ and $W = 10^7$ in \cite{mnih2013playing}.










==> result_js.tex <==
% !TEX root =  main.tex

\section{Analysis}

In this section, we analyze the convergence of DAB Q-learning. We first establish that $\theta_n$ tends to $\theta^\star$, the parameter of the optimal, i.e., that minimizing the projected Bellman error. We then study the asymptotic covariance of the algorithm. 

We make the following assumptions:
\begin{enumerate}[label={(A\arabic*)}]
\item \label{A:step} 
%We consider $\alpha_n = (n+1)^{-\alpha}$, $\beta_n = (n+1)^{-\beta}$ with $1\ge \alpha > \beta > 1/2$.
%{\tt Please change the corresponding explains... Actually, we need little bit tricky conditions on step size. However, once we choose $\alpha_n = (n+1)^{-\alpha}$, $\beta_n = (n+1)^{-\beta}$, where $1\ge \alpha > \beta > 1/2$. Everything that we need is satisfied. }
(i) $\sum_{n =0}^\infty \alpha_n = \infty,  \sum_{n =0}^\infty \beta_n= \infty$, \\
$\sum_{n =0}^\infty \alpha_n^2 < \infty,  \sum_{n =0}^\infty \beta_n^2 < \infty$;\\
(ii) $\lim_{n \to \infty} \frac{ \alpha_n}{\beta_n}  = 0$;\\
(iii)$\forall n$, $0 \le {\alpha_n} - {\alpha_{n+1}} \le \alpha_n^2$, $0 \le {\beta_n} - {\beta_{n+1}}  \le  \beta^2_n$.

\item \label{A:invert} $A(\theta')$ is invertible for all $\theta \in \mathbb{R}^d$ so that
for each greedy policy w.r.t. $\theta$, solution of $A(\theta')\theta + b = 0$  is unique.
\item \label{A:contract} $\bold{T}\bold{B}^{\star}$ is a contraction mapping w.r.t. some norm $\|\cdot \|_c$, i.e., there exists a constant $\gamma \in [0,1)$ such that for all $\theta, \theta' \in \mathbb{R}^d$,
$\|\bold{T}\bold{B}^{\star} Q_{\theta} - \bold{T}\bold{B}^{\star} Q_{\theta'}\|_{c}
 \le \gamma \|Q_{\theta} - Q_{\theta'}\|_{c}$.
\end{enumerate}

Note that we do not assume that the Markov chain describing the system dynamics under the behavior policy$\pi_b$ is aperiodic. This contrasts with existing convergence analysis of previously proposed algorithms (strong mixing, e.g., $\alpha$-mixing or aperiodicity is often assumed, which explicitly regulates correlation between consecutive samples. 

\ref{A:step}(i) is an essential condition for convergence of stochastic approximation algorithms \cite{borkar2008book}. \ref{A:step}(ii) means that the time-scales at which $\theta_n$ and $\hat{A}_n(\theta_m')$ are separated. \ref{A:step}(iii) implies that each sequence of step sizes is decreasing smoothly. This is necessary to eliminate a potential risk of divergence due to resonance between the step sizes and the behavior of system under $\pi_b$ if the resulting Markov chain is periodic. \ref{A:step}(iii) is not necessary when the Markov chain is aperiodic. \ref{A:step} holds for the following choice of step sizes: $\alpha_n = (n+1)^{-\alpha}$, $\beta_n = (n+1)^{-\beta}$, where $1\ge \alpha > \beta > 1/2$.

Further observe that since the state and action spaces are finite, the set of all possible greedy policies $\pi_\theta$, $\theta\in \mathbb{R}^d$ is finite. Thus, the number of all possible $A(\theta)$ is also finite. \ref{A:invert} is necessary to ensure the uniqueness of the fixed point of $\bold{T}\bold{B}^{\theta}$ for every greedy policy $\pi_\theta$. This is an essential assumption that allows the corresponding ODE \eqref{eq:ode2} has a unique asymptotically global equilibrium which is ensured by the invertibility of $A(\theta)$. The same assumption on $A(\theta)$ is also made in previous works, e.g., \cite{sutton2009fast}.

Finally, together with the facts that the feature function $(\phi_i)_{i=1,\ldots,d}$ are linearly independent, \ref{A:contract} is needed to ensure the existence and uniqueness of the parameter $\theta^\star$ minimizing $e(\theta)$. Indeed, although $\bold{B}^*$ is contraction with respect to $\| \cdot \|_\infty$ and $\bold{T}$ is non-expanding with respect to $\| \cdot \|_{\mu}$,
we cannot guarantee that $\bold{T}\bold{B}^*$ is contraction in $\| \cdot \|_{\infty}$ or $\| \cdot \|_{\mu}$. Also note that in absence of function approximation, \ref{A:contract} and \ref{A:invert} with $\|\cdot\|_c=\|\cdot \|_\infty$ are verified if the behavior policy visits every state and action infinitely often, i.e., $\mu(s, a) >0$. See Section~2.1 of \cite{bertsekas2011approximate} for a more detailed  discussion on sufficient conditions under which \ref{A:contract} holds.


\subsection{Convergence guarantee}

\begin{theorem} \label{thm:convergence}
Assume that 
\ref{A:step}-\ref{A:contract}
 hold, and that the Dab Q-learning algorithm uses samples $\xi_n$ extracted by ideal random sampling or sampling with Experience Replay with $B, W \ge 1$. Then $\theta_n$ converges almost surely to $\theta^\star$ minimizing $e(\theta)$ over $\theta$ (i.e., ${e}(\theta^\star)=0=\mathcal{D}(\theta^\star, \theta^\star) = 0$).
\end{theorem}

The proof of the above theorem is provided in Appendix, and leverages similar techniques developed in \cite{kushner1997} for the analysis of stochastic approximation algorithms. These techniques are adapted and extended to our general setting where the Markov chain describing the system dynamics can be periodic (hence introducing a periodic behavior of the {\it noise} averaged by the algorithm).

Somewhat surprisingly, Experience Replay does not play any specific role in the convergence of the algorithm as convergence is achieved even for any $W$ and $B$ and even when $W=1=B$ (i.e., without ER). Actually, ER makes the analysis challenging due to the inherent correlations among successive samples (with ER, the same transition can be used in several iterations of the algorithm). In the proof of Theorem \ref{thm:convergence}, we establish that the proposed implementation of sampling with ER together with step sizes satisfying (A1) ensure that the sample correlations do not accumulate and are mitigated over time even when chain is periodic.

It is worth to provide some notes on previous work with similar analysis.
To study convergence given correlated sampling, \citet{sutton2009fast, melo2008analysis}
assume aperiodic Markov chain so that 
it has fast mixing, e.g., uniformly or geometrically ergodic.
However, 
it is unfortunate that their analysis didn't study
correlation among samples carefully.
In particular, they do not have \ref{A:step}(iii), which is important to ensure
unbiased estimation.
Indeed, one can easily find a counterexample, in which sample-dependent step size
causes divergence, e.g., using $\alpha_n = \frac{1}{n}$ for some set of observation.
Beside this, their proof has some logical gap
%\cite{sutton2009convergent, melo2008analysis}
\footnote{The proof of Theorem~5.1 of \cite{sutton2009convergent} is unsound in calculating the conditional expectation.
In \cite{melo2008analysis}, 
the analysis mainly relies on Theorem~17 of \cite{benveniste2012adaptive}, but
there is no proof that the conditions are satisfied even when two consecutive updates are correlated due to the trajectory sampling.}.

 \citet{devraj2017zap} provides convergence analysis of
 \alg with $\tau = 0$ and no function approximation.
Even though they consider aperiodic case only, 
their analysis requires somewhat strong assumption
that explicitly regulates frequency of policy change:
\begin{align*}
\sum_{n= 0}^\infty \beta_n \mathbb{I}[ \pi_{\theta_n} \neq \pi_{\theta_{n+1}}] < \infty  \;.
\end{align*}
By having $\tau >0$, we obtain analytical tractability.


%\footnote{Consider a Markov chain with state space $\mathcal{S}$.
% and stationary distribution $\mu$ over $\mathcal{S}$ 
%such that for measurable set $U \subset \mathcal{S}$,
%there exist bounded functions $f$ and $g$ such that 
%$\left| \Pr[S_n \in U \mid \mathcal{H}_0] - \mu(U) \right| \le 
% f(U)g(n)$.
%When $g(n) = \rho^{\lfloor {n}/{n'} \rfloor}$ with $\rho \in [0,1)$, we say the Markov chain is
% uniformly ergodic.  If $g(n) = \rho^{n}$ with $\rho \in [0,1)$ and some constant $n'$, then we say it is geometrically ergodic. 
%}.




%In particular, our result extends the convergence for the periodic case, i.e., $L_{\max} \ge 2$,
%unless the chain has a unique stationary distribution.
%We note that the Markov chain with finite state space has a unique stationary distribution
%if and only if it has a unique essential communicating class.
%Hence, our convergence result do not require the chain to be aperiodic or mixing fast.
%However, in such periodic or slow-mixing cases,
%we additionally need to use either experience replay with $W \ge L_{\max}$ or non-increasing step size, e.g., $\alpha_n = \frac{1}{n}$, which are easily implemented in practice.




\subsection{Convergence rate}\label{sec:rate}

For simplicity, we assume here that the step sizes are such that $\alpha_n = (n+1)^{-\alpha}$, $\beta_n = (n+1)^{-\beta}$, where $1\ge \alpha > \beta > 1/2$. We study the rate of convergence of DAB Q-learning through the asymptotic behavior of the scaled error sequence $(\theta_n - \theta^*)/\sqrt{\alpha_n}$. We further assume that the Markov chain generated under policy $\pi_b$ is aperiodic. This assumption is needed to ensure that the asymptotic covariance matrix $\Sigma_{\theta^\star} : = \lim_{n \to \infty}  \frac{1}{\alpha_n} \EXP \left[  (\theta_n - \theta^\star)   (\theta_n - \theta^\star)^\top \right]$ is well defined. In case of periodic Markov chain, the limit might not exist due to oscillations. The following theorem establishes the convergence in distribution of the scaled error $(\theta_n - \theta^*)/\sqrt{\alpha_n}$ to a normal distribution of covariance matrix $\Sigma_{\theta^\star}$, and provides an explicit expression of this matrix.

\begin{theorem} \label{thm:covariance}
Assume that (A1)-(A2)-(A3) hold, and that the DAB Q-learning algorithm uses samples $\xi_n$ extracted by ideal random sampling or sampling with Experience Replay with $B, W \ge 1$. Further assume that the system starts in steady-state\footnote{Remember that importantly, when ER is used with a window size equal to $W$, the system is started at time $-W+1$. Hence, we assume that $(s_0,a_0)\sim\mu$ without ER, and that $(s_{-W+1},a_{-W+1})\sim\mu$ with ER}. The scaled error sequence $({\theta}_n- \theta^\star)/\sqrt{\alpha_n}$ weakly converges to a normal distribution $\mathcal{N}(0, \Sigma_{\theta^\star})$ where
\begin{align} \label{eq:asymp-cov}
\Sigma_{\theta^\star} & = \lim_{n \to \infty}  \frac{1}{\alpha_n} \EXP \left[  (\theta_n - \theta^\star)   (\theta_n - \theta^\star)^\top \right]\nonumber\\
& = (A^\star)^{-1} \Sigma (A^\star)^{-\top}.
\end{align}
In the above expression, we have $A^\star := A(\theta^\star)$, and 
\begin{align} \label{eq:core-cov}
\Sigma &:=
\Sigma_0
+
\sum_{n =1}^{\infty}
( \Sigma_n
+
\Sigma_n^\top
)\;, \\
\Sigma_n &:=  
%\left(\sum_{i = 1}^B \right)
\EXP  \left[
( {A}^\star_{n} \theta^\star  + {b}_{n}) ( {A}^\star_{0} \theta^\star  + {b}_{0})^\top \right]  \;,
\nonumber
\end{align}
where  ${A}^\star_{n} := \frac{1}{B}\sum_{i = 1}^B A_{n, i}(\theta^\star)$,  ${b}_{n} := \frac{1}{B}\sum_{i = 1}^B b_{n,i}$. The covariance matrix $\Sigma$ is referred to the core covariance.
\end{theorem}

In addition, the asymptotic covariance matrix $\Sigma_{\theta^\star}$ obtained under DAB Q-learning is optimal in the following sense. If we assume that the parameter $\theta_m'$ is fixed to $\theta^\star$, and assume that instead of using the gain matrix $\Gamma_n$ in the updates of $\theta_n$, we use a fixed gain matrix $\Gamma$ such that $\Gamma A^\star$ and $\Gamma A^\star+I/2$ are Hurwitz. The latter conditions ensure that the algorithm would yield a finite asymptotic covariance matrix for the scaled error (see Appendix A.1 in \citet{devraj2017zap}), and denote by $\Sigma_{\theta^\star}(\Gamma)$ this covariance matrix. Then we have $\Sigma_{\theta^\star}(\Gamma) \ge \Sigma_{\theta^\star}$ in the sense that for all $x \in \mathbb{R}^d$, $x^\top (\Sigma_{\theta^\star}(\Gamma) - \Sigma_{\theta^\star}) x \ge 0$.

Using almost identical analysis to Theorems~\ref{thm:convergence}~and~\ref{thm:covariance},
we can also show that GTD or GTD2 with gain matrix $\Gamma$ 
converges to $\theta^*$ and  the same asymptotic covariance if
$C := \EXP_\mu [\varphi \varphi^\top]$ is invertible.
A formal description is provided in the supplementary material.

\section{The Role of Experience Replay}

As stated in Theorem \ref{thm:convergence}, ER does not play any role in the convergence of DAB Q-learning. However, ER may affect the rate at which the algorithm converges. In this section, we study the impact of ER on the asymptotic covariance matrix of the scaled error derived in Theorem \ref{thm:covariance}. 

The way we sample the trajectory generated under $\pi_b$ does not influence the matrix $A^\star$. Hence we are interested in how ER affects the core covariance matrix $\Sigma$. As a reference, we define the {\it unit} core covariance matrix $S_0$, as that obtained in steady-state using a single sample $B=1$: 
$$
S_0=\mathbb{E}_\mu \left[ ( \tilde{A} \theta^\star  + \tilde{b}) ( \tilde{A} \theta^\star  + \tilde{b})^\top  \right],
$$ 
where $\tilde{A} = \varphi (\lambda \varphi'(\theta^\star) - \varphi )^\top$ and $\tilde{b} = \hat{r} \varphi$.

Define $\Sigma_{\iid} (B)$ and $\Sigma_{\ER} (B, W)$ as the core covariance matrices \eqref{eq:core-cov} under ideal random sampling with batch size $B >0$
and ER with batch size $B > 0$ and window size $W \ge B$, respectively.

\begin{proposition} \label{prop:covariance-calc}
We have: for any $1\le B\le W$,
\begin{align} 
 \Sigma_{\iid}(B) &= \frac{1}{B} S_0,\label{eq:iid-cov}\\
 \Sigma_{\ER}(W, W) &= \Sigma_{\ER}(1, 1),\label{eq:WW-cov}\\
\lim_{W \to \infty }\Sigma_{\ER}(B, W) &= \frac{1}{B} \sigma_0.\label{eq:BW-cov}
\end{align}
\end{proposition}

The first part suggests us to use large $B$. However, somewhat surprisingly, when $W$ is not huge compared to $B$,
we don't expect much gain from experience replay.
%large $B = W$ would be helpful to reduce
%
%improve transient behavior since it provides
%  when target policy is changing. Hence, they might provide faster convergence in reality.
Our result explains the choice of $B = 32$ and $W = 10^7$ made in \cite{mnih2013playing}.


To minimize the asymptotic perturbation $\theta_n$, we can choose $\alpha_n = 1/n$.










==> section2.tex <==
% !TEX root =  main.tex

\section{Structured Ergodic Markov Decision Processes}  \label{sec:model}
%\section{Reinforcement Learning with Undiscounted Reward}

We consider a Markov Decision Process (MDP) $\phi = (\set{S}, \set{A}, p, q)$ with finite state space $\set{S}$ and finite action space $\set{A}$, transition kernel $p$ and reward kernel $q$. Specifically, when in state $x$, under action $a$, the system moves to state $y$ with probability $p(y|x,a)$, and a reward drawn from distribution $q(\cdot|x,a)$ is collected. This reward is bounded, w.l.o.g. in $[0,1]$, and of average $r(x,a)$. We assume that for any $(x,a)$, $q(\cdot |x,a)$ is absolutely continuous w.r.t. some measure $\lambda$ on $[0,1]$\footnote{$\lambda$ can be the Lebesgue measure; alternatively, if rewards take values in $\{0,1 \}$, $\lambda$ can be the sum of Dirac measures at 0 and 1.}. The random vector $Z_t=(X_t, A_t, R_t)$ represents the state, the action, and the collected reward at step $t$. A policy $\pi$ selects an action, denoted by $a=\pi_t(x)$, in step $t$ when the system is in state $x$ based on the history captured through ${\cal H}_t^\pi$, the $\sigma$-algebra generated by $(Z_1,\ldots, Z_{t-1},X_t)$ observed under $\pi$: $\pi_t(x)$ is $\set{H}_t^\pi$-measurable. We denote by $\Pi$ the set of all such policies. We further introduce $\Pi_{S}$ the set of stationary Markovian deterministic policies, i.e. when in state $X_t=x$, $\pi\in \Pi_{S}$ select an action $\pi(x)$ (independent of $t$). Unless otherwise specified, we assume that $\phi$ is {\it ergodic}, meaning that under any policy $\pi\in \Pi_{S}$, the Markov chain $(X_t)_{t\ge 1}$ is irreducible. 

The expected cumulative reward up to step $T$ of a policy $\pi\in \Pi$ when the system starts in state $x$ is:
$
V_T^\pi(x) = \mathbb{E}_x^\pi[\sum_{t=1}^T R_t],
$
where $\mathbb{E}_x^\pi[\cdot]$ denote the expectation under policy $\pi$ given that $X_1=x$. For any $\pi\in \Pi_{S}$, we denote by $g^\pi$ its ergodic gain: $g^\pi=\lim_{T\to\infty}{1\over T}V_T^\pi(x)$ (which does not depend on the initial state $x$ since $\phi$ is ergodic). The {\it bias function} $h^\pi$ of $\pi$ is defined by $h^\pi(x)=C-\lim_{T\to\infty} \mathbb{E}_x^\pi[R_t - g^\pi]$ and quantifies the advantage of starting in state $x$. $g^\pi$ and $h^\pi$ satisfy: for all state $x\in\set{S}$,
$$
g^\pi + h^\pi(x) = (\mathbf{B}^\pi  h^\pi) (x),
$$
where $\mathbf{B}^\pi$ is the Bellman operator of $\pi$ defined by for any $h: \set{S} \mapsto \mathbb{R}$
and $x \in \set{S}$,
\begin{align*}
(\mathbf{B}^\pi h)(x) =  r(x,\pi(x)) + \sum_{y \in \set{S}} p(y| x,\pi(x)) h(y).
\end{align*}

We denote by $\Pi^\star(\phi)$ the set of stationary Markovian deterministic policies with maximal gain: $\Pi^\star(\phi)=\{ \pi\in \Pi_{S}: g^\pi \ge \sup_{\pi'\in  \Pi_{S}} g^{\pi'}\}$, and denote their gain and bias function by $g^\star$ and $h^\star$, respectively. We have: for any $x\in \set{S}$,
$$
g^\star + h^\star(x) = (\mathbf{B}^\star  h^\star) (x),
$$
where $\mathbf{B}^\star$ is the optimal Bellman operator defined by for any $h: \set{S} \mapsto \mathbb{R}$
and $x \in \set{S}$,
\begin{align*}
(\mathbf{B}^\star h)(x) =  \max_{a\in\set{A}}\left\{ r(x,a) + \sum_{y \in \set{S}} p(y | x,a) h(y)\right\}.
\end{align*}

\subsection{Structures}

We assume that the MDP considered $\phi$ is initially unknown but belongs to a known set $\Phi$ of ergodic MDPs, encoding its structure. This known structure is instrumental to   ...\\

\noindent
{\bf Unstructured MDPs.}

\medskip
\noindent
{\bf Lipschitz MDPs.}

\medskip
\noindent


\subsection{Online Learning Problem}

Assume that the system starts in state $x$ and evolves according to the initially unknown MDP $\phi\in \Phi$. The objective is to devise an online learning policy $\pi\in \Pi$ converging as fast as possible to an optimal stationary Markovian policy for $\phi$. The performance of a learning policy $\pi\in \Pi$ is quantified through its regret up to step $T$ defined as the difference between the cumulative reward of an optimal stationary policy and that obtained under $\pi$:
$$
R_T^\pi(x)= V^\star_T(x) - V^\pi_T(x).
$$
We are in particular interested in quantifying the gain in terms of regret one gets when optimally exploiting the known structure.






==> section3_old.tex <==
% !TEX root =  main.tex

\section{Regret Lower Bounds}

In this section, we present an (asymptotic) regret lower bound satisfied by any {\it uniformly good} learning algorithm. An algorithm $\pi\in \Pi$ is uniformly good if for all MDP $\phi\in \Phi$, for any initial state $x$, the regret of $\pi$ satisfies $R_T^\pi(x)=o(T^\alpha)$ for any $\alpha>0$. 

To state our lower bound, we introduce the following notations. Let $\phi,\psi\in \Phi$. We define the KL-divergence $\kl_{\phi \mid \psi}(x,a)$ between $\phi$ and $\psi$ in (state, action) pair $(x,a)$ as the KL-divergence between the distributions of the next state and collected reward if the state is $x$ and $a$ is selected under these two MDPs:
\begin{align*}
\kl_{\phi \mid \psi}(x,a) 
= \sum_{y\in \set{S}} p_\phi(y | x,a)  \log \frac{p_\phi(y | x,a) }{p_\psi(y | x,a) }  
+
\int_{0}^1 q_\phi(r | x,a) \log \frac{q_\phi(r | x,a)}{q_\psi(r | x,a) }\lambda(dr)  \;.
\end{align*}
We further define the set of {\it confusing} MDPs as:
\begin{align*}
\Delta_{\Phi} (\phi) = \{\psi \in \Phi : (i) \ \kl_{\phi \mid \psi}(x,a) = 0~  \forall x, \forall a \in \set{O}(x ;\phi),  \text{ and }(ii)\  \Pi^*(\phi) \cap \Pi^*(\psi) = \emptyset \} \;.
\end{align*}
This set consists of MDPs $\psi$ (i) that coincide with $\phi$ for (state, action) pairs where the actions are optimal (the kernels of $\phi$ and $\psi$ cannot be statistically distinguished under an optimal policy), and (ii) such that optimal policies under $\psi$ are not optimal under $\phi$. 

\begin{theorem} \label{thm:g-r-lower}
Let $\phi \in \Phi$. For any uniformly good algorithm $\pi \in \Pi$ and for any $x \in \set{S}$, 
\begin{align} \label{eq:g-r-lower}
\liminf_{T \to \infty} \frac{R^\pi_T (x)}{\log T} \ge K_{\Phi}(\phi) \;, 
\end{align}
where $K_{\Phi}(\phi)$ is the value of the following optimization problem:
\begin{subequations} \label{eq:g-r-opt}
\begin{align}
& \underset{\eta(x, a)\ge 0, ~ (x,a) \in \set{S}\times \set{A} }{\textnormal{minimize}} 
~~\sum_{(x,a) \in \set{S}\times \set{A}} \eta(x, a)  \delta^*(x, a;\phi) \label{eq:g-r-obj}\\
& \textnormal{subject to} ~~
\sum_{(x,a) \in \set{S} \times \set{A}}
 \eta(x, a) \kl_{\phi\mid \psi}(x,a) \ge 1  \label{eq:g-r-set}\,,\, 
\forall \psi \in \Delta_{\Phi} (\phi).
\end{align}
\end{subequations}
\end{theorem}

The above theorem can be interpreted as follows. When selecting a sub-optimal action $a$ in state $x$, one has to pay a regret of $\delta^*(x, a;\phi)$. Then the minimal number of times any sub-optimal action $a$ in state $x$ has to be explored scales as $\eta(x,a)\log(T)$ where $\eta(x,a)$ solves the optimization problem (\ref{eq:g-r-obj})-(\ref{eq:g-r-set}). It worth mentioning that our lower bound is tight, as we present in Section \ref{sec:algo} an algorithm achieving this fundamental regret limit. 

The regret lower bound stated in Theorem \ref{thm:g-r-lower} extends the problem-specific regret lower bound derived in \cite{burnetas1997optimal} for unstructured ergodic MDPs with known reward function. Our lower bound is valid for unknown reward function, but also applies for {\it any} structure $\Phi$. Note however that at this point, it is only implicitly defined through the solution of (\ref{eq:g-r-obj})-(\ref{eq:g-r-set}). The latter seems difficult to solve. The optimization problem can actually be simplified, as shown later in this section, depending on the structure considered. This will be done by providing useful structural properties of the feasibility set 
$$
\set{F}_{\Phi}(\phi):=\{\eta(x, a)\ge 0, ~ (x,a) \in \set{S}\times \set{A}: (\ref{eq:g-r-set})\hbox{ holds}\}.
$$
The simplification will be instrumental to quantify the gain that can be achieved when optimally exploiting the structure, as well as to design efficient algorithms.  

The proof of Theorem \ref{thm:g-r-lower} combines a characterization of the regret as a function of the number of times $N_T(x,a)$ up to step $T$ (state, action) pair $(x,a)$ are visited, and of the action sub-optimality gap, and change-of-measure arguments as those recently used to prove in a very direct manner regret lower bounds in bandit optimization problems \cite{kaufmann2016complexity}. More precisely, for any uniformly good algorithm $\pi$, and for any confusing MDP $\psi\in  \Delta_{\Phi} (\phi)$, we show that $\liminf_{T\to\infty}{1\over \log(T)}\sum_{(x,a) \in \set{S} \times \set{A}}\mathbb{E}_{x_1}^\pi[N_T(x, a)] \kl_{\phi\mid \psi}(x,a)\ge 1$ for any initial state $x_1$. The theorem is then obtained by considering all possible confusing MDPs.  

In the following, we let $\eta=(\eta(x,a))_{x,a}$ and $\set{F}_0(\phi):=\{\eta\ge 0: \eta(x,a)=0, \forall (x,a): \delta^\star(x,a;\phi)=0\}$. We further denote by $P(\phi,\set{F})$ the optimization problem:
$$
 \underset{\eta\in \set{F} }{\textnormal{minimize}} 
~~\sum_{(x,a) \in \set{S}\times \set{A}} \eta(x, a)  \delta^*(x, a;\phi),
$$
so that $P(\phi,\set{F}_{\Phi}(\phi))$ corresponds to (\ref{eq:g-r-obj})-(\ref{eq:g-r-set}).



\subsection{Decoupled exploration in unstructured MDPs}

In absence of structure, the set of possible MDPs is just:
$$
\Phi=\{\psi: p_\psi(\cdot |x,a)\in \set{P}(\set{S}^+(x,a)), q_\psi(\cdot |x,a)\in  \set{P}([0,1]), \forall (x,a)\}.
$$
For such $\Phi$, we establish the following theorem:

\begin{theorem} \label{thm:unrelated}
For the unstructured model $\Phi$, we have:
\begin{align*}
\set{F}_\Phi(\phi)
=
\left\{
\eta \in \set{F}_0(\phi):  \forall (x,a)~\text{s.t.}~a \notin \set{O}(x; \phi), \eta(x, a) \kl_{\phi\mid \psi}(x,a) \ge 1 ~
\forall \psi \in \Delta_{\Phi}(x, a; \phi)
\right\} \;.
\end{align*}
where
$
\Delta_{\Phi}(x,a; \phi) :=
\{\psi \in \Phi  : \kl_{\phi \mid \psi} (y, b) = 0 ~\forall (y,b) \neq (x,a)~\text{and}~ (\mathbf{B}^a_\psi h^*_\phi)(x) > g^*_\phi + h^*_\phi(x)\}.
$
\end{theorem}

The theorem states that in the optimization problem (\ref{eq:g-r-obj})-(\ref{eq:g-r-set}), we can reduce (\ref{eq:g-r-set}) by restricting our attention to confusing MDPs $\psi$ that are different than the true MDP $\phi$ only in a single (state, action) pair $(x,a)$. Further note that the condition $(\mathbf{B}^a_\psi h^*_\phi)(x) > g^*_\phi + h^*_\phi(x)$ is equivalent to saying that action $a$ becomes optimal in state $x$ under $\psi$ (see Lemma 1(i) in \cite{burnetas1997optimal}). Hence to obtain the lower bound in MDPs lacking structure, we may just consider confusing MDPs $\psi$ that makes an initially sub-optimal action $a$ in state $x$ optimal by locally changing the kernels of $\phi$ at $(x,a)$ only. Importantly, this observation implies that an optimal algorithm $\pi$ must satisfy $\mathbb{E}_{x_0}^\pi[N_T(x,a)] \sim \log(T) / \inf_{\psi\in \Delta_{\Phi}(x,a; \phi)} \kl_{\phi\mid \psi}(x,a)$. In other words, the required levels of exploration of the various sub-optimal (state, action) pairs are {\it decoupled}, which significantly simplifies the design of optimal algorithms.

To get an idea on how the regret lower bound scales as the sizes of the state and action spaces, we can further provide an upper bound of the regret lower bound. One may easily observe (see the appendix for a proof) that $\set{F}_{\TN{un}}(\phi) \subset \set{F}_\Phi(\phi)$ where
\begin{align*}
\set{F}_{\TN{un}}(\phi)
=
\left\{
\eta  \in\set{F}_0(\phi)
: 
 \eta(x, a) \left(\frac{\delta^*(x, a;\phi)}{ H+1}\right)^2 \ge 2, ~ 
\forall (x,a)~\text{s.t.}~a \notin \set{O}(x; \phi)
\right\} \;.
\end{align*}
From this result, an upper bound of the regret lower bound is $K_{\textnormal{un}}(\phi):=2{(H+1)^2\over \delta_{\min}}SA\log(T)$, and we can devise algorithms achieving this regret scaling (see Section \ref{sec:algo}).   

Theorem \ref{thm:unrelated} relies on the following decoupling lemma (in fact valid under any structure $\Phi$).

 \begin{lemma} \label{lem:gen-decom} Let $\set{U}_1,\set{U}_2$ be two non-overlapping subsets of the (state, action) pairs such that for all $(x,a)\in \set{U}_0:=\set{U}_1\cup\set{U}_2$, $a\notin \set{O}(x;\phi)$. Define the following three MDPs in $\Phi$ obtained starting from $\phi$ and changing the kernels for (state, action) pairs in $\set{U}_1\cup\set{U}_2$. Specifically, let $(p,q)$ be some transition and reward kernels. For all $(x,a)$, define $\psi_j$, $j\in\{0,1,2\}$ as 
\begin{align*}
(p_{\psi_j}(\cdot | x, a), q_{\psi_j}(\cdot |x,a))  &=
\begin{cases}
(p(\cdot | x, a),q(\cdot |x,a)) & \text{if $(x, a) \in  \set{U}_j$}, \\
(p_{\phi}(\cdot | x, a),q_\phi(\cdot |x,a))  & \text{otherwise}. 
\end{cases} 
\end{align*} 
Then, if $\Pi^*(\phi) \cap \Pi^*(\psi_0) = \emptyset$, then 
$\Pi^*(\phi) \cap \Pi^*(\psi_1) = \emptyset$ or
$\Pi^*(\phi) \cap \Pi^*(\psi_2) = \emptyset$.
 \end{lemma}

\subsection{Lipschitz MDPs}

Lipschitz structures have been widely studied in the bandit and reinforcement learning literature. We find the following structure convenient, although one could imagine other variants in more general metric spaces. We assume that the state and action spaces can be embedded in the Euclidian spaces of respective dimensions $d$ and $d'$: $\set{S}\subset [0,D]^d$ and $\set{A}\subset [0,D']^{d'}$. We consider MDPs whose transition kernels and average rewards are Lipschitz w.r.t. the state and action. Specifically, let $L, L'>0$, $\alpha, \alpha'>0$, and 
$$
\Phi=\{\psi: p_\psi(\cdot |x,a)\in \set{P}(\set{S}^+(x,a)), q_\psi(\cdot |x,a)\in  \set{P}([0,1]): (L1)-(L2) \hbox{ hold}, \forall (x,a)\}, 
$$
where
\begin{align*}
(L1) & \quad\quad \| p_\psi(\cdot |x,a) - p_\psi(\cdot | x', a') \|_1 
\le L d(x, x')^\alpha + L' d(a,a')^{\alpha'} \;, \\
(L2) & \quad\quad |r_\psi(x,a) - r_\psi(x', a') |  \le L d(x, x')^\alpha + L' d(a,a')^{\alpha'} \;,
\end{align*}
and $d(\cdot,\cdot)$ is the Euclidean distance.


\begin{theorem} \label{thm:lip}
For the model $\Phi$ with Lipschitz structure, we have $\set{F}_{\TN{lip}}(\phi) \subset \set{F}_\Phi(\phi)$ where 
$\set{F}_{\TN{lip}}(\phi)$ is the set of $\eta \in \set{F}_0(\phi) $ satisfying for all $(x',a')$ such that $a' \notin \set{O}(x', \phi)$, 
\begin{align}
\sum_{x \in \set{S}}  \sum_{a \notin \set{O}(x,\phi)}
\eta(x, a) 
\left( \left[ \frac{\delta^*(x', a';\phi)}{H+1} - 2 \left( Ld(x,x')^\alpha
+  L' d(a,a')^{\alpha'} \right)
\right]_+ \right)^2
 \ge 2  \label{eq:ind-r-set}
\end{align}
where we use the notation $[u]_+ :=\max\{0,u\}$ for $u\in \mathbb{R}$.
Furthermore, the optimal values $K_\Phi(\phi)$ and $K_{\TN{lip}}(\phi)$ of $P(\phi, \set{F}_{\Phi}(\phi))$
and $P(\phi, \set{F}_{\TN{lip}}(\phi))$ are upper bounded by $8\frac{(H+1)^3}{\delta^2_{\min}}
\cdot S_{\textnormal{lip}} A_{\textnormal{lip}}$ where 
\begin{align*}
S_{\textnormal{lip}} := 
\min
\left\{S, 
\left( \frac{D \sqrt{d}}{ \left( \frac{\delta_{\min}}{8L  (H+1)} \right)^{1/\alpha}} +1 \right)^{d}
\right\},  
\text{ and }
A_{\textnormal{lip}} := 
\min
\left\{A, 
\left( \frac{D' \sqrt{d'}}{ \left( \frac{\delta_{\min}}{8L'  (H+1)} \right)^{1/\alpha'}} +1 \right)^{d'}
\right\} \;.
\end{align*}
\end{theorem}

The above theorem has important consequences. First, it states that exploiting the Lipschitz structure optimally, one may achieve a regret at most scaling as $\frac{(H+1)^3}{\delta^2_{\min}} S_{\textnormal{lip}} A_{\textnormal{lip}}\log(T)$. This scaling is independent of the sizes of the state and action spaces provided that the minimal gap $\delta_{\min}$ is fixed, and provided that the span $H$ does not scale with $S$. This typically holds for fast mixing model or for MDPs with diameter not scaling with $S$ (see e.g. \cite{regal} for a precise connection between $H$ and the diameter). Hence, exploiting the structure can really yield significant regret improvements. As shown in the next section, by just leveraging the simplified structure in $\set{F}_{\TN{lip}}(\phi)$, we may devise a simple algorithm realizing these improvements, i.e., having a regret scaling at most as $K_{\TN{lip}}(\phi)\log(T)$.
 





==> structure.tex <==
% !TEX root =  main.tex

\section{The Fundamental Limit}

minimization problem for general structure.



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "./main"
%%% End: 


==> upper-copy-copy.tex <==
% !TEX root =  main.tex

\section{Algorithms}
\label{sec:algo}

In this section, we present DEL (Directed Exploration Learning), an algorithm that achieves the regret limits identified in the previous section. DEL is an adaptation of OSSB \cite{combes17}, an asymptotically optimal algorithm for structured bandit. It aims at exploring (state, action) pairs according to the solution of $P(\phi,\set{F}_{\Phi}(\phi))$. Essentially, DEL implements a version of a bandit algorithm in each state.

In each step $t$, DEL first solves the optimization problem $P(\phi_t,\set{F}_{\Phi}(\phi_t))$ where $\phi_t$ is a MDP estimated from the previous observations\footnote{We take $\phi_t$ with reduced $\set{S}_t$ communicating to $X_t$, and 
we use $\set{O}(x; \phi_t)$ and $\delta^*(x, a ; \phi_t)$ with an arbitrarily chosen stationary optimal policy and its bias function $h^*_{\phi_t}$. }. 
Let $\eta^\star(\phi_t)$ denote the solution of this problem, where  
Theorem~1 suggests that $\eta^\star(x, a;\phi_t) \log t$ is the minimum amount of statistics on kernels at $(x,a)$
in order to make sure the current estimation on optimal policy is indeed optimal. 
%Hence, the algorithm performs the minimal exploration. 
% the number of times (state, action) pair $(x,a)$ is visited exceed $\eta^\star(x,a;\phi_t) \log t$. 
 To ensure that $\phi_t$ estimates $\phi$ well (to apply the certainty equivalence principle), and that the algorithm works as expected, DEL alternates between three phases: exploitation, estimation, and exploration. 
 In step $t$, if the system is in state $X_t$, and if $N_T(X_t,a)$ is larger than $\eta^\star(X_t,a;\phi_t) \log t$ for all actions $a$, we play an apparent best action in $X_t$ for $\phi_t$, i.e., we are in the exploitation phase. When this is not the case, we must gather more information about $\phi$ to determine the true optimal actions, and we play an action $a$ such that either $N_t(X_t,a)$ has been visited very little (estimation phase), or $N_T(X_t,a)<\eta^\star(X_t,a;\phi_t) \log t$ (exploration phase. Refer to Algorithm \ref{alg:ORL} for the pseudo-code of DEL.

For simplicity of the presentation and analysis, we assume that the rewards are Bernoulli distributed, although the analysis could be extended to one-parameter sub-gaussian distributions. We further assume that $\phi$ has a unique optimal deterministic policy and that the solution of $\set{P}(\phi, \set{F}_{\Phi} (\phi))$ is unique. Under these assumptions, we have:
\begin{theorem} \label{thm:ORL}
Consider structure $\Phi$ and ergodic $\phi \in \Phi$. %correspond to either the unstructured or the Lipschitz model defined in the previous section.
Then, for $\pi = \alg (\varepsilon, \gamma)$, we have:
\begin{align} \label{eq:upper}
\limsup_{T \to \infty}\frac{R^\pi_T(\phi)}{\log T} \le K_{\Phi}(\phi) C(\varepsilon, \gamma, \phi) \;, 
\end{align}
where $C(\varepsilon, \gamma, \phi)  \to 1$ as $\varepsilon\to 0$ and $\gamma \to 0$.

In addition, for Lipschitz $\Phi$ with (L1)-(L2) (resp. unstructured $\Phi$) if $\pi=\alg (\varepsilon, \gamma)$ solves in each step $t$, $\set{P}(\phi_t, \set{F}_{\textnormal{lip}} (\phi_t))$ (resp. $\set{P}(\phi_t, \set{F}_{\textnormal{un}} (\phi_t))$) instead of $\set{P}(\phi_t, \set{F}_{\Phi} (\phi_t))$, its regret is asymptotically smaller than $K_{\textnormal{lip}}(\phi)\log T$ (resp. $K_{\textnormal{un}}(\phi)\log T$).
\end{theorem}

It is worth noting that DEL needs to solve the MDP $\phi_t$ in each step as any algorithm for undiscounted RL problems. It further requires to solve $\set{P}(\phi_t, \set{F}_{\Phi} (\phi_t))$ which can be quite complex. However, for unstructured RL problems, its simplified version (solving $\set{P}(\phi_t, \set{F}_{\textnormal{un}} (\phi_t))$ only) is easy to implement as $\set{P}(\phi_t, \set{F}_{\textnormal{un}} (\phi_t))$ is just a linear programming (LP). DEL then just boils down to solving $\phi_t$, while its regret scales at most as ${(H+1)^2\over \delta_{\min}}SA\log T$ as that of OLP \cite{bartlett08}. Compared to DEL, OLP further needs to solve optimization problems to compute the index of each action. Further observe that the simplified version of DEL for Lipschitz MDPs requires to solve in each step $\set{P}(\phi_t, \set{F}_{\textnormal{lip}} (\phi_t))$ which is an LP. Yet this simplified version achieves a regret scaling at most as  $K_{\textnormal{lip}}(\phi)\log T$.


\begin{algorithm}[tb]
   \caption{\alg($\varepsilon$,$\gamma$)}
   \label{alg:ORL}
\begin{algorithmic}
\INPUT Model structure $\Phi$
   \STATE Initialize 
   $N_1(x) \leftarrow \mathbbm{1}[x = X_1]$,
   $N_1(x,a) \leftarrow 0$, $s_1(x) \leftarrow 0$, 
$p_1 (y \mid x,a) \leftarrow {1}/{|\set{S}|}$, $r_1 (x,a) \leftarrow 0 $ for each $x,y \in \set{S}$, $ a \in \set{A}$, and $\phi_1$ accordingly.
%   \begin{align*}
%   \hat{p}_0 (y \mid x,a) \leftarrow 
%   \begin{cases}
%   \frac{1}{|\set{S}^+_{x,a}|} & \text{if $y \in \set{S}^+_{x,a}$} \\
%0 & \text{otherwise}
%      \end{cases} \;, ~~ 
%      \text{and} ~~
%         \hat{r}_0 (x,a) \leftarrow 0  \;,
%\end{align*}
%   where $\set{S}^+_{x,a} := \{y \in \set{S} :  p_{\psi}(y \mid  x, a) > 0,  \exists \psi \in \Phi\}$.
%   \STATE{$T_0(x,a) \leftarrow |\set{S}^+(x,a)|, \forall (x,a) \in \set{S} \times \set{A}$}.
%   \STATE{$s_0(x) \leftarrow 0, \forall x \in \set{S}$}.
\FOR{$t=1,...,T$}
\STATE{Obtain a solution $\eta^*(\phi_t)$ of $P(\phi_t, \set{F}_{\Phi}(\phi_t) ) $ and set
  $s_{t+1}(x) \leftarrow s_{t}(x)~\forall x \in \set{S}$.}
\IF{$N_{t} (X_t,a) > \eta^*(X_t, a;\phi_t) (1+\gamma) \log N_{t}(X_t)~\forall a \in  \set{A}$} 
   	\STATE{{\bf Exploit: } $A_t \leftarrow \argmin_{ a\in \set{O}(X_t; \phi_t)} N_t(X_t, a)$} \hfill %\COMMENT{\underline{Exploitation}}
	\ELSE
		\STATE{$s_{t+1}(X_t) \leftarrow s_{t}(X_t) + 1$}
		\IF{$\min_{a \in \set{A}} N_{t}(X_t, a) \le \varepsilon \cdot s_{t}(X_t)$}
			\STATE{{\bf Estimate: }$A_{t} \leftarrow \underline{A}_t := \arg\min_{a \in \set{A}} N_{t}(X_t, a)$}
			%\hfill\COMMENT{\underline{Estimation}}
		\ELSE
			\STATE{{\bf Explore :} $A_{t} \leftarrow \overline{A}_t  := \arg\min_{a \in \set{A}} {N_{t}(X_t, a) \over \eta^*(X_t, a; \phi_t)}$}\footnotemark 
			%\hfill \COMMENT{\underline{Exploration}}
		\ENDIF
\ENDIF
      \STATE{Select action $A_t$, and observe the next state $X_{t+1}$ and the instantaneous reward $R_t$. }
          \STATE{ Update $\phi_{t+1}$: 
          $N_{t+1}(x) \leftarrow  N_t(x,a) + \mathbbm{1}[x = X_{t+1}]$, \\
          $N_{t+1}(x,a) \leftarrow  N_t(x,a) + \mathbbm{1}[(x,a) = (X_t, A_t)]$,\\
          \begin{minipage}{0.7\textwidth}
    \begin{align*}
    &p_{t+1}(y \mid x,a) \leftarrow 
    \begin{cases}
    \frac{N_{t}(x, a) p_{t}(y \mid x,a) + \mathbbm{1}[y=X_{t+1}]}{N_{t+1}(x, a)}  & \text{if $(x,a) = (X_t, A_t)$} \\
        p_{t}(y \mid x,a) & \text{otherwise}
	\end{cases}  \\
    &r_{t+1}(x,a) 
    \leftarrow 
    \begin{cases}
    \frac{N_{t}(x, a) r_{t}(x,a) + R_t}{N_{t+1}(x, a)}  & \text{if $(x,a) = (X_t, A_t)$} \\
        r_{t}(x,a) & \text{otherwise}
	\end{cases} 
\end{align*}
          \end{minipage},
           $ \quad \forall x,y \in \set{S}, a \in \set{A}$
   }      
   \ENDFOR
\end{algorithmic}
\end{algorithm}
%\footnotetext{We take convention of $1/0 = \infty$.}









%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "./main"
%%% End: 


==> upper-oldalgo.tex <==
% !TEX root =  main.tex


\begin{algorithm}[tb]
   \caption{\alg}
   \label{alg:ORL}
\begin{algorithmic}
\INPUT Model structure $\Phi$
   \STATE Initialize 
   $N_1(x) \leftarrow \mathbbm{1}[x = X_1]$,
   $N_1(x,a) \leftarrow 0$, $s_1(x) \leftarrow 0$, 
$p_1 (y \mid x,a) \leftarrow {1}/{|\set{S}|}$, $r_1 (x,a) \leftarrow 0 $ for each $x,y \in \set{S}$, $ a \in \set{A}$, and $\phi_1$ accordingly.
%   \begin{align*}
%   \hat{p}_0 (y \mid x,a) \leftarrow 
%   \begin{cases}
%   \frac{1}{|\set{S}^+_{x,a}|} & \text{if $y \in \set{S}^+_{x,a}$} \\
%0 & \text{otherwise}
%      \end{cases} \;, ~~ 
%      \text{and} ~~
%         \hat{r}_0 (x,a) \leftarrow 0  \;,
%\end{align*}
%   where $\set{S}^+_{x,a} := \{y \in \set{S} :  p_{\psi}(y \mid  x, a) > 0,  \exists \psi \in \Phi\}$.
%   \STATE{$T_0(x,a) \leftarrow |\set{S}^+(x,a)|, \forall (x,a) \in \set{S} \times \set{A}$}.
%   \STATE{$s_0(x) \leftarrow 0, \forall x \in \set{S}$}.
\FOR{$t=1,...,T$}
\STATE{Let $\gamma_t := \max \{1,  \log \log  N_t(X_t) \}$ and $\delta_t := 1/\gamma_t$.}
\STATE{Obtain a solution $\eta_t$ of $P(\phi_t, \set{F}^{\delta_t }_{\Phi}(\phi_t) ) $ and set
  $s_{t+1}(x) \leftarrow s_{t}(x)~\forall x \in \set{S}$.}
\IF{$N_{t} (X_t,a) > (\eta_t(X_t, a) + \sqrt{\delta_t}) \log N_{t}(X_t)~\forall a \in  \set{A}$} 
   	\STATE{{\bf Exploit: } $A_t \leftarrow \argmin_{ a\in \set{O}(X_t; \phi_t)} N_t(X_t, a)$} \hfill %\COMMENT{\underline{Exploitation}}
	\ELSE
		\STATE{$s_{t+1}(X_t) \leftarrow s_{t}(X_t) + 1$}
		\IF{$\min_{a \in \set{A}} N_{t}(X_t, a) \le \delta_t^4 s_{t}(X_t)$}
			\STATE{{\bf Estimate: }$A_{t} \leftarrow \underline{A}_t := \arg\min_{a \in \set{A}} N_{t}(X_t, a)$}
			%\hfill\COMMENT{\underline{Estimation}}
		\ELSE
			\STATE{{\bf Explore :} $A_{t} \leftarrow \overline{A}_t  := \arg\min_{a \in \set{A}} {N_{t}(X_t, a) \over \eta_t(X_t, a)}$} 
			%\hfill \COMMENT{\underline{Exploration}}
		\ENDIF
\ENDIF
      \STATE{Select action $A_t$, and observe the next state $X_{t+1}$ and the instantaneous reward $R_t$. }
          \STATE{ Update $\phi_{t+1}$: 
          $N_{t+1}(x) \leftarrow  N_t(x,a) + \mathbbm{1}[x = X_{t+1}]$, \\
          $N_{t+1}(x,a) \leftarrow  N_t(x,a) + \mathbbm{1}[(x,a) = (X_t, A_t)]$,\\
          \begin{minipage}{0.7\textwidth}
    \begin{align*}
    &p_{t+1}(y \mid x,a) \leftarrow 
    \begin{cases}
    \frac{N_{t}(x, a) p_{t}(y \mid x,a) + \mathbbm{1}[y=X_{t+1}]}{N_{t+1}(x, a)}  & \text{if $(x,a) = (X_t, A_t)$} \\
        p_{t}(y \mid x,a) & \text{otherwise}
	\end{cases}  \\
    &r_{t+1}(x,a) 
    \leftarrow 
    \begin{cases}
    \frac{N_{t}(x, a) r_{t}(x,a) + R_t}{N_{t+1}(x, a)}  & \text{if $(x,a) = (X_t, A_t)$} \\
        r_{t}(x,a) & \text{otherwise}
	\end{cases} 
\end{align*}
          \end{minipage},
           $ \quad \forall x,y \in \set{S}, a \in \set{A}$
   }      
   \ENDFOR
\end{algorithmic}
\end{algorithm}
%\footnotetext{We take convention of $1/0 = \infty$.}





\section{Algorithms}
\label{sec:algo}

In this section, we present DEL (Directed Exploration Learning), an algorithm that achieves the regret limits identified in the previous section. DEL is an adaptation of OSSB \cite{combesnips17}, an asymptotically optimal algorithm for structured bandit. It aims at exploring (state, action) pairs according to the solution of $P(\phi,\set{F}_{\Phi}(\phi))$. Essentially, DEL implements a version of a bandit algorithm in each state.

In each step $t$, DEL first solves the optimization problem $P(\phi_t,\set{F}_{\Phi}(\phi_t))$ where $\phi_t$ is a MDP estimated from the previous observations\footnote{$\phi_t$ may not be communicating. We circumvent this issue by restricting its state space to the set of states communicating with $X_t$ under $\phi_t$, so that $\phi_t$ indeed becomes communicating. We then use $\set{O}(x; \phi_t)$ and $\delta^*(x, a ; \phi_t)$ with arbitrarily chosen stationary optimal policy and its bias function $h^*_{\phi_t}$.  We note that at time $t$, DEL uses only a part of solution related to $X_t$. }. 
Let $\eta^\star(\phi_t)$ denote the solution of this problem, where  
Theorem~1 suggests that $\eta^\star(x, a;\phi_t) \log t$ is the minimum amount of statistics on kernels at $(x,a)$
in order to make sure the current estimation of the optimal policy is indeed optimal. 
%Hence, the algorithm performs the minimal exploration. 
% the number of times (state, action) pair $(x,a)$ is visited exceed $\eta^\star(x,a;\phi_t) \log t$. 
 To ensure that $\phi_t$ estimates $\phi$ well (to apply the certainty equivalence principle), and that the algorithm works as expected, DEL alternates between three phases: exploitation, estimation, and exploration. 
In step $t$, if the system is in state $X_t$, and if $N_T(X_t,a)$ is larger than $\eta^\star(X_t,a;\phi_t) \log t$ for all actions $a$, we play an apparently best action in $X_t$ for $\phi_t$, i.e., we are in the exploitation phase. When this is not the case, we must gather more information about $\phi$ to determine the true optimal actions, and we play an action $a$ such that either $N_t(X_t,a)$ has been visited very little (estimation phase), or $N_T(X_t,a)<\eta^\star(X_t,a;\phi_t) \log t$ (exploration phase). Refer to Algorithm \ref{alg:ORL} for the pseudo-code of DEL.

For simplicity of the presentation and analysis, we assume that the rewards are Bernoulli distributed, although the analysis could be extended to one-parameter sub-gaussian distributions. We further assume that $\phi$ has a unique optimal deterministic policy and that the solution of $\set{P}(\phi, \set{F}_{\Phi} (\phi))$ is unique. Under these assumptions, we have:
\begin{theorem} \label{thm:ORL}
Consider an arbitrary model $\Phi$, and let $\phi \in \Phi$ be ergodic. %correspond to either the unstructured or the Lipschitz model defined in the previous section.
Then, for $\pi = \alg (\varepsilon, \gamma)$, we have:
\begin{align} \label{eq:upper}
\limsup_{T \to \infty}\frac{R^\pi_T(\phi)}{\log T} \le K_{\Phi}(\phi) C(\varepsilon, \gamma, \phi) \;, 
\end{align}
where $C(\varepsilon, \gamma, \phi)  \to 1$ as $\varepsilon\to 0$ and $\gamma \to 0$.

In addition, for Lipschitz $\Phi$ with (L1)-(L2) (resp. unstructured $\Phi$) if $\pi=\alg (\varepsilon, \gamma)$ solves in each step $t$, $\set{P}(\phi_t, \set{F}_{\textnormal{lip}} (\phi_t))$ (resp. $\set{P}(\phi_t, \set{F}_{\textnormal{un}} (\phi_t))$) instead of $\set{P}(\phi_t, \set{F}_{\Phi} (\phi_t))$, its regret is asymptotically smaller than $K_{\textnormal{lip}}(\phi)\log T$ (resp. $K_{\textnormal{un}}(\phi)\log T$).
\end{theorem}

The proof is provided in the supplementary material.
It is worth noting that DEL needs to solve the MDP $\phi_t$ in each step as any algorithm for undiscounted RL problems. It further requires to solve $\set{P}(\phi_t, \set{F}_{\Phi} (\phi_t))$ which can be quite complex. However, for unstructured RL problems, its simplified version, solving $\set{P}(\phi_t, \set{F}_{\textnormal{un}} (\phi_t))$ only, is easy to implement as 
the solution of $\set{P}(\phi_t, \set{F}_{\textnormal{un}} (\phi_t))$ is immediate. % once we obtain $(\delta^*(x,a; \phi_t))_{x,a}$.
DEL then just boils down to solving $\phi_t$, while its regret scales at most as ${(H+1)^2\over \delta_{\min}}SA\log T$ as that of OLP \cite{bartlett08}. Compared to DEL, OLP further needs to solve optimization problems to compute the index of each action. Further observe that the simplified version of DEL for Lipschitz MDPs requires to solve in each step $\set{P}(\phi_t, \set{F}_{\textnormal{lip}} (\phi_t))$ which is a linear programming problem. This simplified version achieves a regret scaling at most as  $K_{\textnormal{lip}}(\phi)\log T$.
In the supplementary material, we demonstrate preliminary numerical experiments that illustrate our theoretical findings. In particular, we study examples of Lipschitz MDPs, for which the regret under DEL with $\set{P}(\phi_t, \set{F}_{\textnormal{lip}} (\phi_t))$ does not seem to scale with $S$ and $A$, whereas it significantly outperforms algorithms that do not exploit the structure.








%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "./main"
%%% End: 


==> upper.bak181007.tex <==
% !TEX root =  main.tex


\begin{algorithm}[tb]
   \caption{\alg($\varepsilon$,$\gamma$)}
   \label{alg:ORL}
\begin{algorithmic}
\INPUT Model structure $\Phi$
   \STATE Initialize 
   $N_1(x) \leftarrow \mathbbm{1}[x = X_1]$,
   $N_1(x,a) \leftarrow 0$, $s_1(x) \leftarrow 0$, 
$p_1 (y \mid x,a) \leftarrow {1}/{|\set{S}|}$, $r_1 (x,a) \leftarrow 0 $ for each $x,y \in \set{S}$, $ a \in \set{A}$, and $\phi_1$ accordingly.
%   \begin{align*}
%   \hat{p}_0 (y \mid x,a) \leftarrow 
%   \begin{cases}
%   \frac{1}{|\set{S}^+_{x,a}|} & \text{if $y \in \set{S}^+_{x,a}$} \\
%0 & \text{otherwise}
%      \end{cases} \;, ~~ 
%      \text{and} ~~
%         \hat{r}_0 (x,a) \leftarrow 0  \;,
%\end{align*}
%   where $\set{S}^+_{x,a} := \{y \in \set{S} :  p_{\psi}(y \mid  x, a) > 0,  \exists \psi \in \Phi\}$.
%   \STATE{$T_0(x,a) \leftarrow |\set{S}^+(x,a)|, \forall (x,a) \in \set{S} \times \set{A}$}.
%   \STATE{$s_0(x) \leftarrow 0, \forall x \in \set{S}$}.
\FOR{$t=1,...,T$}
\STATE{Obtain a solution $\eta^*(\phi_t)$ of $P(\phi_t, \set{F}_{\Phi}(\phi_t) ) $ and set
  $s_{t+1}(x) \leftarrow s_{t}(x)~\forall x \in \set{S}$.}
\IF{$N_{t} (X_t,a) > \eta^*(X_t, a;\phi_t) (1+\gamma) \log N_{t}(X_t)~\forall a \in  \set{A}$} 
   	\STATE{{\bf Exploit: } $A_t \leftarrow \argmin_{ a\in \set{O}(X_t; \phi_t)} N_t(X_t, a)$} \hfill %\COMMENT{\underline{Exploitation}}
	\ELSE
		\STATE{$s_{t+1}(X_t) \leftarrow s_{t}(X_t) + 1$}
		\IF{$\min_{a \in \set{A}} N_{t}(X_t, a) \le \varepsilon \cdot s_{t}(X_t)$}
			\STATE{{\bf Estimate: }$A_{t} \leftarrow \underline{A}_t := \arg\min_{a \in \set{A}} N_{t}(X_t, a)$}
			%\hfill\COMMENT{\underline{Estimation}}
		\ELSE
			\STATE{{\bf Explore :} $A_{t} \leftarrow \overline{A}_t  := \arg\min_{a \in \set{A}} {N_{t}(X_t, a) \over \eta^*(X_t, a; \phi_t)}$} 
			%\hfill \COMMENT{\underline{Exploration}}
		\ENDIF
\ENDIF
      \STATE{Select action $A_t$, and observe the next state $X_{t+1}$ and the instantaneous reward $R_t$. }
          \STATE{ Update $\phi_{t+1}$: 
          $N_{t+1}(x) \leftarrow  N_t(x,a) + \mathbbm{1}[x = X_{t+1}]$, \\
          $N_{t+1}(x,a) \leftarrow  N_t(x,a) + \mathbbm{1}[(x,a) = (X_t, A_t)]$,\\
          \begin{minipage}{0.7\textwidth}
    \begin{align*}
    &p_{t+1}(y \mid x,a) \leftarrow 
    \begin{cases}
    \frac{N_{t}(x, a) p_{t}(y \mid x,a) + \mathbbm{1}[y=X_{t+1}]}{N_{t+1}(x, a)}  & \text{if $(x,a) = (X_t, A_t)$} \\
        p_{t}(y \mid x,a) & \text{otherwise}
	\end{cases}  \\
    &r_{t+1}(x,a) 
    \leftarrow 
    \begin{cases}
    \frac{N_{t}(x, a) r_{t}(x,a) + R_t}{N_{t+1}(x, a)}  & \text{if $(x,a) = (X_t, A_t)$} \\
        r_{t}(x,a) & \text{otherwise}
	\end{cases} 
\end{align*}
          \end{minipage},
           $ \quad \forall x,y \in \set{S}, a \in \set{A}$
   }      
   \ENDFOR
\end{algorithmic}
\end{algorithm}
%\footnotetext{We take convention of $1/0 = \infty$.}





\section{Algorithms}
\label{sec:algo}

In this section, we present DEL (Directed Exploration Learning), an algorithm that achieves the regret limits identified in the previous section. DEL is an adaptation of OSSB \cite{combesnips17}, an asymptotically optimal algorithm for structured bandit. It aims at exploring (state, action) pairs according to the solution of $P(\phi,\set{F}_{\Phi}(\phi))$. Essentially, DEL implements a version of a bandit algorithm in each state.

In each step $t$, DEL first solves the optimization problem $P(\phi_t,\set{F}_{\Phi}(\phi_t))$ where $\phi_t$ is a MDP estimated from the previous observations\footnote{$\phi_t$ may not be communicating. We circumvent this issue by restricting its state space to the set of states communicating with $X_t$ under $\phi_t$, so that $\phi_t$ indeed becomes communicating. We then use $\set{O}(x; \phi_t)$ and $\delta^*(x, a ; \phi_t)$ with arbitrarily chosen stationary optimal policy and its bias function $h^*_{\phi_t}$.  We note that at time $t$, DEL uses only a part of solution related to $X_t$. }. 
Let $\eta^\star(\phi_t)$ denote the solution of this problem, where  
Theorem~1 suggests that $\eta^\star(x, a;\phi_t) \log t$ is the minimum amount of statistics on kernels at $(x,a)$
in order to make sure the current estimation of the optimal policy is indeed optimal. 
%Hence, the algorithm performs the minimal exploration. 
% the number of times (state, action) pair $(x,a)$ is visited exceed $\eta^\star(x,a;\phi_t) \log t$. 
 To ensure that $\phi_t$ estimates $\phi$ well (to apply the certainty equivalence principle), and that the algorithm works as expected, DEL alternates between three phases: exploitation, estimation, and exploration. 
In step $t$, if the system is in state $X_t$, and if $N_T(X_t,a)$ is larger than $\eta^\star(X_t,a;\phi_t) \log t$ for all actions $a$, we play an apparently best action in $X_t$ for $\phi_t$, i.e., we are in the exploitation phase. When this is not the case, we must gather more information about $\phi$ to determine the true optimal actions, and we play an action $a$ such that either $N_t(X_t,a)$ has been visited very little (estimation phase), or $N_T(X_t,a)<\eta^\star(X_t,a;\phi_t) \log t$ (exploration phase). Refer to Algorithm \ref{alg:ORL} for the pseudo-code of DEL.

For simplicity of the presentation and analysis, we assume that the rewards are Bernoulli distributed, although the analysis could be extended to one-parameter sub-gaussian distributions. We further assume that $\phi$ has a unique optimal deterministic policy and that the solution of $\set{P}(\phi, \set{F}_{\Phi} (\phi))$ is unique. Under these assumptions, we have:
\begin{theorem} \label{thm:ORL}
Consider an arbitrary model $\Phi$, and let $\phi \in \Phi$ be ergodic. %correspond to either the unstructured or the Lipschitz model defined in the previous section.
Then, for $\pi = \alg (\varepsilon, \gamma)$, we have:
\begin{align} \label{eq:upper}
\limsup_{T \to \infty}\frac{R^\pi_T(\phi)}{\log T} \le K_{\Phi}(\phi) C(\varepsilon, \gamma, \phi) \;, 
\end{align}
where $C(\varepsilon, \gamma, \phi)  \to 1$ as $\varepsilon\to 0$ and $\gamma \to 0$.

In addition, for Lipschitz $\Phi$ with (L1)-(L2) (resp. unstructured $\Phi$) if $\pi=\alg (\varepsilon, \gamma)$ solves in each step $t$, $\set{P}(\phi_t, \set{F}_{\textnormal{lip}} (\phi_t))$ (resp. $\set{P}(\phi_t, \set{F}_{\textnormal{un}} (\phi_t))$) instead of $\set{P}(\phi_t, \set{F}_{\Phi} (\phi_t))$, its regret is asymptotically smaller than $K_{\textnormal{lip}}(\phi)\log T$ (resp. $K_{\textnormal{un}}(\phi)\log T$).
\end{theorem}

The proof is provided in the supplementary material.
It is worth noting that DEL needs to solve the MDP $\phi_t$ in each step as any algorithm for undiscounted RL problems. It further requires to solve $\set{P}(\phi_t, \set{F}_{\Phi} (\phi_t))$ which can be quite complex. However, for unstructured RL problems, its simplified version, solving $\set{P}(\phi_t, \set{F}_{\textnormal{un}} (\phi_t))$ only, is easy to implement as 
the solution of $\set{P}(\phi_t, \set{F}_{\textnormal{un}} (\phi_t))$ is immediate. % once we obtain $(\delta^*(x,a; \phi_t))_{x,a}$.
DEL then just boils down to solving $\phi_t$, while its regret scales at most as ${(H+1)^2\over \delta_{\min}}SA\log T$ as that of OLP \cite{bartlett08}. Compared to DEL, OLP further needs to solve optimization problems to compute the index of each action. Further observe that the simplified version of DEL for Lipschitz MDPs requires to solve in each step $\set{P}(\phi_t, \set{F}_{\textnormal{lip}} (\phi_t))$ which is a linear programming problem. This simplified version achieves a regret scaling at most as  $K_{\textnormal{lip}}(\phi)\log T$.
In the supplementary material, we demonstrate preliminary numerical experiments that illustrate our theoretical findings. In particular, we study examples of Lipschitz MDPs, for which the regret under DEL with $\set{P}(\phi_t, \set{F}_{\textnormal{lip}} (\phi_t))$ does not seem to scale with $S$ and $A$, whereas it significantly outperforms algorithms that do not exploit the structure.








%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "./main"
%%% End: 


==> upper_old.tex <==
% !TEX root =  main.tex

\section{Algorithms}
\label{sec:algo}

In this section, we present DEL (Directed Exploration Learning), an algorithm that achieves the regret limits identified in the previous section. DEL is an adaptation of OSSB, an asymptotically optimal algorithm for structured bandit \cite{combes17}. It aims at directing exploration so that (state, action) pairs are explored according to the solution of $P(\phi,\set{F}(\phi))$. Essentially, DEL implements the bandit OSSB algorithm at each state.

\note{JS:}
In each step $t$, DEL first solves the optimization problem $P(\phi_t,\set{F}_{\Phi}(\phi_t))$ where $\phi_t$ is a MDP estimated from the previous observations\footnote{We take $\phi_t$ with reduced $\set{S}_t$ communicating to $X_t$, and 
we use $\set{O}(x; \phi_t)$ and $\delta^*(x, a ; \phi_t)$ with an arbitrarily chosen stationary optimal policy and its bias function $h^*_{\phi_t}$. } 
\note{JS: this is non-trivial part. The definition of $\Phi$ seems a bit wired. Hence, I propose to mention $\set{S}^+$ in only definition of $\Delta$...}
and $\set{S}^+_t(x,a)$ of $\Phi$ is taken w.r.t. $\phi_t$. Hence DEL do not require the true $\set{S}^+$ in advance. Let $\eta^\star(\phi_t)$ denote the solution of this problem. The actions are then selected so that the number of times (state, action) pair $(x,a)$ is visited exceed $\eta^\star(x,a;\phi_t)$. To ensure that $\phi_t$ estimates $\phi$ well (to apply the certainty equivalence principle), and that the algorithm works as expected, DEL alternates between three phases: exploitation, estimation, and exploration. In step $t$, if the system is in state $X_t$, and if $N_T(X_t,a)$ is larger than $\eta^\star(X_t,a;\phi_t)$ for all actions $a$, we play an apparent best action in $X_t$ for $\phi_t$, i.e., we are in the exploitation phase. When this is not the case, we must gather more information about $\phi$ to determine the true optimal actions, and we play an action $a$ such that either $N_t(X_t,a)$ has been visited very little (estimation phase), or $N_T(X_t,a)<\eta^\star(X_t,a;\phi_t)$ (exploration phase. Refer to Algorithm \ref{alg:ORL} for the pseudo-code of DEL.


\note{JS: to the general structure and uniqueness assumption}
For simplicity of the presentation and analysis, we assume that the rewards are Bernoulli distributed, although the analysis could be extended to one-parameter sub-gaussian distributions. We further assume that $\phi$ has a unique optimal deterministic policy and that the solution of $\set{P}(\phi, \set{F}_{\Phi} (\phi))$ is unique. Under these assumptions, we have:
\begin{theorem} \label{thm:ORL}
Consider $\Phi$ with Bernoulli reward and ergodic $\phi \in \Phi$.
Then, for $\pi = \alg (\varepsilon, \gamma)$ and $\varepsilon < \frac{1}{|\set{A}|}$we have:
\begin{align} \label{eq:upper}
\limsup_{T \to \infty}\frac{R^\pi_T(\phi)}{\log T} \le K_{\Phi}(\phi) C(\varepsilon, \gamma, \phi) \;, 
\end{align}
where $C(\varepsilon, \gamma, \phi)  \to 1$ as $\varepsilon\to 0$ and $\gamma \to 0$.

In addition, for Lipschitz $\Phi$ with (L1)-(L2) (resp. unstructured $\Phi$) if $\pi=\alg (\varepsilon, \gamma)$ solves in each step $t$, $\set{P}(\phi_t, \set{F}_{\textnormal{lip}} (\phi_t))$ (resp. $\set{P}(\phi_t, \set{F}_{\textnormal{un}} (\phi_t))$) instead of $\set{P}(\phi_t, \set{F}_{\Phi} (\phi_t))$, its regret is asymptotically smaller than $K_{\textnormal{lip}}(\phi)\log(T)$ (resp. $K_{\textnormal{un}}(\phi)\log(T)$).
\end{theorem}

It is worth noting that DEL needs to solve the MDP $\phi_t$ in each step as any algorithm for undiscounted RL problems. It further requires to solve $\set{P}(\phi_t, \set{F}_{\Phi} (\phi_t))$ which can be quite complex. However, for unstructured RL problems, its simplified version (solving $\set{P}(\phi_t, \set{F}_{\textnormal{un}} (\phi_t))$ only) is easy to implement as investigating $\set{P}(\phi_t, \set{F}_{\textnormal{un}} (\phi_t))$ is straightforward. DEL then just boils down to solving $\phi_t$, while it regret scales at most as ${(H+1)^2\over \delta_{\min}}SA\log(T)$ as that of OLP \cite{bartlett08}. Compared to DEL, OLP further needs to solve optimization problems to compute the index of each action. Further observe that the simplified version of DEL for the Lipschitz structure requires to solve in each step $\set{P}(\phi_t, \set{F}_{\textnormal{lip}} (\phi_t))$ which is an LP. Yet this simplified version achieves a regret scaling at most as  $K_{\textnormal{lip}}(\phi)\log(T)$.


\begin{algorithm}[tb]
   \caption{\alg($\varepsilon$,$\gamma$)}
   \label{alg:ORL}
\begin{algorithmic}
\INPUT Model structure $\Phi$
   \STATE Initialize 
   $N_1(x) \leftarrow \mathbbm{1}[x = X_1]$,
   $N_1(x,a) \leftarrow 0$, $s_1(x) \leftarrow 0$, 
$p_1 (y \mid x,a) \leftarrow {1}/{|\set{S}|}$, $r_1 (x,a) \leftarrow 0 $ for each $x,y \in \set{S}$, $ a \in \set{A}$, and $\phi_1$ accordingly.
%   \begin{align*}
%   \hat{p}_0 (y \mid x,a) \leftarrow 
%   \begin{cases}
%   \frac{1}{|\set{S}^+_{x,a}|} & \text{if $y \in \set{S}^+_{x,a}$} \\
%0 & \text{otherwise}
%      \end{cases} \;, ~~ 
%      \text{and} ~~
%         \hat{r}_0 (x,a) \leftarrow 0  \;,
%\end{align*}
%   where $\set{S}^+_{x,a} := \{y \in \set{S} :  p_{\psi}(y \mid  x, a) > 0,  \exists \psi \in \Phi\}$.
%   \STATE{$T_0(x,a) \leftarrow |\set{S}^+(x,a)|, \forall (x,a) \in \set{S} \times \set{A}$}.
%   \STATE{$s_0(x) \leftarrow 0, \forall x \in \set{S}$}.
\FOR{$t=1,...,T$}
\STATE{Obtain a solution $\eta^*(\phi_t)$ of $P(\phi_t, \set{F}_{\Phi}(\phi_t) ) $ and set
  $s_{t+1}(x) \leftarrow s_{t}(x)~\forall x \in \set{S}$.}
\IF{$N_{t} (X_t,a) > \eta^*(X_t, a;\phi_t) (1+\gamma) \log N_{t}(X_t)~\forall a \in  \set{A}$} 
   	\STATE{{\bf Exploit: } $A_t \leftarrow \argmin_{ a\in \set{O}(X_t; \phi_t)} N_t(X_t, a)$} \hfill %\COMMENT{\underline{Exploitation}}
	\ELSE
		\STATE{$s_{t+1}(X_t) \leftarrow s_{t}(X_t) + 1$}
		\IF{$\min_{a \in \set{A}} N_{t}(X_t, a) \le \varepsilon \cdot s_{t}(X_t)$}
			\STATE{{\bf Estimate: }$A_{t} \leftarrow \underline{A}_t := \arg\min_{a \in \set{A}} N_{t}(X_t, a)$}
			%\hfill\COMMENT{\underline{Estimation}}
		\ELSE
			\STATE{{\bf Explore :} $A_{t} \leftarrow \overline{A}_t  := \arg\min_{a \in \set{A}} {N_{t}(X_t, a) \over \eta^*(X_t, a; \phi_t)}$}\footnotemark 
			%\hfill \COMMENT{\underline{Exploration}}
		\ENDIF
\ENDIF
      \STATE{Select action $A_t$, and observe the next state $X_{t+1}$ and the instantaneous reward $R_t$. }
          \STATE{ Update $\phi_{t+1}$: 
          $N_{t+1}(x) \leftarrow  N_t(x,a) + \mathbbm{1}[x = X_{t+1}]$, \\
          $N_{t+1}(x,a) \leftarrow  N_t(x,a) + \mathbbm{1}[(x,a) = (X_t, A_t)]$,\\
          \begin{minipage}{0.7\textwidth}
    \begin{align*}
    &p_{t+1}(y \mid x,a) \leftarrow 
    \begin{cases}
    \frac{N_{t}(x, a) p_{t}(y \mid x,a) + \mathbbm{1}[y=X_{t+1}]}{N_{t+1}(x, a)}  & \text{if $(x,a) = (X_t, A_t)$} \\
        p_{t}(y \mid x,a) & \text{otherwise}
	\end{cases}  \\
    &r_{t+1}(x,a) 
    \leftarrow 
    \begin{cases}
    \frac{N_{t}(x, a) r_{t}(x,a) + R_t}{N_{t+1}(x, a)}  & \text{if $(x,a) = (X_t, A_t)$} \\
        r_{t}(x,a) & \text{otherwise}
	\end{cases} 
\end{align*}
          \end{minipage},
           $ \quad \forall x,y \in \set{S}, a \in \set{A}$
   }      
   \ENDFOR
\end{algorithmic}
\end{algorithm}
\footnotetext{We take convention of $1/0 = \infty$.}









%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "./main"
%%% End: 

